Design of the full-sky scanning strategy and systematic effect control in a cosmic microwave background probe

The quest for primordial $B$-mode polarization signatures in the Cosmic Microwave Background (CMB) is a major goal of contemporary cosmology. Detecting these signatures would confirm primordial gravitational waves and allow precise determination of the tensor-to-scalar ratio, $r$, which is crucial for distinguishing between inflationary models. This requires high-precision, full-sky observations from space-based platforms to avoid atmospheric fluctuations and windows. Since $B$-mode signatures are much fainter than CMB temperature anisotropies, their detection requires well-designed calibration and mitigation strategies. Next-generation space observatories such as LiteBIRD, which use Half-Wave Plate (HWP) modulation technology, represent a significant advance. This technology allows single-detector observations, eliminating the need for pair-differential detection and its associated systematic complexities. The study begins with the optimization of scanning strategy parameters for missions with HWP to improve in-flight calibration, suppress systematic effects, and develop robust null-test methods. In addition, we present a method for calculating the impact of systematic effects on the estimation of $r$ using the SBM (Spin-Based Map-making) software framework, which performs fast map-making in spin space. This method allows the decomposition and elimination of systematic effects in terms of spins, and we demonstrate the elimination of several systematic effects.

==> class/bibliography_bib <==
@article{planck_scanning_strategy,
       author = {{Dupac}, X. and {Tauber}, J.},
        title = "{Scanning strategy for mapping the Cosmic Microwave Background anisotropies with Planck}",
      journal = {\aap},
     keywords = {cosmic microwave background, methods: observational, Astrophysics},
         year = {2005},
        month = {jan},
       volume = {430},
        pages = {363-371},
          doi = {10.1051/0004-6361:20041526},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409405},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...430..363D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mapbased,
    author = {McCallum, Nialh and Thomas, Daniel B and Brown, Michael L},
    title = "{Fast map-based simulations of systematics in CMB surveys including effects of the scanning strategy}",
    journal = {\mnras},
    volume = {513},
    number = {3},
    pages = {3610-3626},
    year = {2022},
    month = {03},
    abstract = "{We present approaches to quickly simulate systematics affecting CMB observations, including the effects of the scanning strategy. Using summary properties of the scan, we capture features of full time ordered data (TOD) simulations, allowing maps and power spectra to be generated at much improved speed for a number of systematics – the cases we present experienced speed ups of 3–4 orders of magnitude when implementing the map-based approaches. We demonstrate the effectiveness of the approaches at capturing the salient features of the scan by directly comparing to full TOD simulations – seeing agreement at sub-percent levels of accuracy. We simulate the effects of differential gain, pointing, and ellipticity to show the effectiveness of the approaches, but note that one could extend these techniques to other systematics. We finally show how to apply these fast map-based simulations of systematic effects to a full focal plane showing their ability to incorporate thousands of detectors as seen in modern CMB experiments.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stac561},
    url = {https://doi.org/10.1093/mnras/stac561},
    eprint = {https://academic.oup.com/mnras/article-pdf/513/3/3610/43687567/stac561.pdf},
}


@article{PhysRevD.77.083003,
  title = {CMB polarization systematics due to beam asymmetry: Impact on inflationary science},
  author = {Shimon, Meir and Keating, Brian and Ponthieu, Nicolas and Hivon, Eric},
  journal = {Phys. Rev. D},
  volume = {77},
  issue = {8},
  pages = {083003},
  numpages = {11},
  year = {2008},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.77.083003},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.77.083003}
}

@article{OptimalScan,
    author = {Wallis, Christopher G. R. and Brown, Michael L. and Battye, Richard A. and Delabrouille, Jacques},
    title = "{Optimal scan strategies for future CMB satellite experiments}",
    journal = {\mnras},
    volume = {466},
    number = {1},
    pages = {425-442},
    year = {2016},
    month = {10},
    abstract = "{The B-mode polarization power spectrum in the cosmic microwave background (CMB) is about four orders of magnitude fainter than the CMB temperature power spectrum. Any instrumental imperfections that couple temperature fluctuations to B-mode polarization must therefore be carefully controlled and/or removed. We investigate the role that a scan strategy can have in mitigating certain common systematics by averaging systematic errors down with many crossing angles. We present approximate analytic forms for the error on the recovered B-mode power spectrum that would result from differential gain, differential pointing and differential ellipticity for the case where two detector pairs are used in a polarization experiment. We use these analytic predictions to search the parameter space of common satellite scan strategies in order to identify those features of a scan strategy that have most impact in mitigating systematic effects. As an example, we go on to identify a scan strategy suitable for the CMB satellite proposed for the European Space Agency M5 call, considering the practical considerations of fuel requirement, data rate and the relative orientation of the telescope to the earth. Having chosen a scan strategy we then go on to investigate the suitability of the scan strategy.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stw2577},
    url = {https://doi.org/10.1093/mnras/stw2577},
    eprint = {https://academic.oup.com/mnras/article-pdf/466/1/425/10864929/stw2577.pdf},
}

@article{spin_characterisation,
    author = {McCallum, Nialh and Thomas, Daniel B and Brown, Michael L and Tessore, Nicolas},
    title = "{Spin characterization of systematics in CMB surveys – a comprehensive formalism}",
    journal = {\mnras},
    volume = {501},
    number = {1},
    pages = {802-832},
    year = {2020},
    month = {11},
    abstract = "{The CMB B-mode polarization signal – both the primordial gravitational wave signature and the signal sourced by lensing – is subject to many contaminants from systematic effects. Of particular concern are systematics that result in mixing of signals of different ‘spin’, particularly leakage from the much larger spin-0 intensity signal to the spin-2 polarization signal. We present a general formalism, which can be applied to arbitrary focal plane setups, that characterizes signals in terms of their spin. We provide general expressions to describe how spin-coupled signals observed by the detectors manifest at map-level, in the harmonic domain, and in the power spectra, focusing on the polarization spectra – the signals of interest for upcoming CMB surveys. We demonstrate the presence of a previously unidentified cross-term between the systematic and the intrinsic sky signal in the power spectrum, which in some cases can be the dominant source of contamination. The formalism is not restricted to intensity to polarization leakage but provides a complete elucidation of all leakage including polarization mixing, and applies to both full and partial (masked) sky surveys, thus covering space-based, balloon-borne, and ground-based experiments. Using a pair-differenced setup, we demonstrate the formalism by using it to completely characterize the effects of differential gain and pointing systematics, incorporating both intensity leakage and polarization mixing. We validate our results with full time ordered data simulations. Finally, we show in an Appendix that an extension of simple binning map-making to include additional spin information is capable of removing spin-coupled systematics during the map-making process.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/staa3609},
    url = {https://doi.org/10.1093/mnras/staa3609},
    eprint = {https://academic.oup.com/mnras/article-pdf/501/1/802/35077383/staa3609.pdf},
}

@ARTICLE{PTEP2023,
      author = {{LiteBIRD Collaboration} and {Allys}, E. and {Arnold}, K. and {Aumont}, J. and {Aurlien}, R. and {Azzoni}, S. and {Baccigalupi}, C. and {Banday}, A.~J. and {Banerji}, R. and {Barreiro}, R.~B. and {Bartolo}, N. and {Bautista}, L. and {Beck}, D. and {Beckman}, S. and {Bersanelli}, M. and {Boulanger}, F. and {Brilenkov}, M. and {Bucher}, M. and {Calabrese}, E. and {Campeti}, P. and {Carones}, A. and {Casas}, F.~J. and {Catalano}, A. and {Chan}, V. and {Cheung}, K. and {Chinone}, Y. and {Clark}, S.~E. and {Columbro}, F. and {D'Alessandro}, G. and {de Bernardis}, P. and {de Haan}, T. and {de la Hoz}, E. and {De Petris}, M. and {Della Torre}, S. and {Diego-Palazuelos}, P. and {Dobbs}, M. and {Dotani}, T. and {Duval}, J.~M. and {Elleflot}, T. and {Eriksen}, H.~K. and {Errard}, J. and {Essinger-Hileman}, T. and {Finelli}, F. and {Flauger}, R. and {Franceschet}, C. and {Fuskeland}, U. and {Galloway}, M. and {Ganga}, K. and {Gerbino}, M. and {Gervasi}, M. and {G{\'e}nova-Santos}, R.~T. and {Ghigna}, T. and {Giardiello}, S. and {Gjerl{\o}w}, E. and {Grain}, J. and {Grupp}, F. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Halverson}, N.~W. and {Hargrave}, P. and {Hasebe}, T. and {Hasegawa}, M. and {Hazumi}, M. and {Henrot-Versill{\'e}}, S. and {Hensley}, B. and {Hergt}, L.~T. and {Herman}, D. and {Hivon}, E. and {Hlozek}, R.~A. and {Hornsby}, A.~L. and {Hoshino}, Y. and {Hubmayr}, J. and {Ichiki}, K. and {Iida}, T. and {Imada}, H. and {Ishino}, H. and {Jaehnig}, G. and {Katayama}, N. and {Kato}, A. and {Keskitalo}, R. and {Kisner}, T. and {Kobayashi}, Y. and {Kogut}, A. and {Kohri}, K. and {Komatsu}, E. and {Komatsu}, K. and {Konishi}, K. and {Krachmalnicoff}, N. and {Kuo}, C.~L. and {Lamagna}, L. and {Lattanzi}, M. and {Lee}, A.~T. and {Leloup}, C. and {Levrier}, F. and {Linder}, E. and {Luzzi}, G. and {Macias-Perez}, J. and {Maciaszek}, T. and {Maffei}, B. and {Maino}, D. and {Mandelli}, S. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Massa}, M. and {Matarrese}, S. and {Matsuda}, F.~T. and {Matsumura}, T. and {Mele}, L. and {Migliaccio}, M. and {Minami}, Y. and {Moggi}, A. and {Montgomery}, J. and {Montier}, L. and {Morgante}, G. and {Mot}, B. and {Nagano}, Y. and {Nagasaki}, T. and {Nagata}, R. and {Nakano}, R. and {Namikawa}, T. and {Nati}, F. and {Natoli}, P. and {Nerval}, S. and {Noviello}, F. and {Odagiri}, K. and {Oguri}, S. and {Ohsaki}, H. and {Pagano}, L. and {Paiella}, A. and {Paoletti}, D. and {Passerini}, A. and {Patanchon}, G. and {Piacentini}, F. and {Piat}, M. and {Pisano}, G. and {Polenta}, G. and {Poletti}, D. and {Prouv{\'e}}, T. and {Puglisi}, G. and {Rambaud}, D. and {Raum}, C. and {Realini}, S. and {Reinecke}, M. and {Remazeilles}, M. and {Ritacco}, A. and {Roudil}, G. and {Rubino-Martin}, J.~A. and {Russell}, M. and {Sakurai}, H. and {Sakurai}, Y. and {Sasaki}, M. and {Scott}, D. and {Sekimoto}, Y. and {Shinozaki}, K. and {Shiraishi}, M. and {Shirron}, P. and {Signorelli}, G. and {Spinella}, F. and {Stever}, S. and {Stompor}, R. and {Sugiyama}, S. and {Sullivan}, R.~M. and {Suzuki}, A. and {Svalheim}, T.~L. and {Switzer}, E. and {Takaku}, R. and {Takakura}, H. and {Takase}, Y. and {Tartari}, A. and {Terao}, Y. and {Thermeau}, J. and {Thommesen}, H. and {Thompson}, K.~L. and {Tomasi}, M. and {Tominaga}, M. and {Tristram}, M. and {Tsuji}, M. and {Tsujimoto}, M. and {Vacher}, L. and {Vielva}, P. and {Vittorio}, N. and {Wang}, W. and {Watanuki}, K. and {Wehus}, I.~K. and {Weller}, J. and {Westbrook}, B. and {Wilms}, J. and {Winter}, B. and {Wollack}, E.~J. and {Yumoto}, J. and {Zannoni}, M.},
        title = "{Probing cosmic inflation with the LiteBIRD cosmic microwave background polarization survey}",
      journal = {\ptep},
         year = 2023,
        month = apr,
       volume = {2023},
       number = {4},
          eid = {042F01},
        pages = {042F01},
          doi = {10.1093/ptep/ptac150},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023PTEP.2023d2F01A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Bock_epic,
  doi = {10.48550/ARXIV.0906.1188},
  url = {https://arxiv.org/abs/0906.1188},
  author = {Bock, James and Aljabri, Abdullah and Amblard, Alex and Baumann, Daniel and Betoule, Marc and Chui, Talso and Colombo, Loris and Cooray, Asantha and Crumb, Dustin and Day, Peter and Dickinson, Clive and Dowell, Darren and Dragovan, Mark and Golwala, Sunil and Gorski, Krzysztof and Hanany, Shaul and Holmes, Warren and Irwin, Kent and Johnson, Brad and Keating, Brian and Kuo, Chao-Lin and Lee, Adrian and Lange, Andrew and Lawrence, Charles and Meyer, Steve and Miller, Nate and Nguyen, Hien and Pierpaoli, Elena and Ponthieu, Nicolas and Puget, Jean-Loup and Raab, Jeff and Richards, Paul and Satter, Celeste and Seiffert, Mike and Shimon, Meir and Tran, Huan and Williams, Brett and Zmuidzinas, Jonas},
  keywords = {Cosmology and Nongalactic Astrophysics (astro-ph.CO), Instrumentation and Methods for Astrophysics (astro-ph.IM), FOS: Physical sciences, FOS: Physical sciences},
  title = {Study of the Experimental Probe of Inflationary Cosmology (EPIC)-Intemediate Mission for NASA's Einstein Inflation Probe},
  publisher = {arXiv},
  year = {2009},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@MISC{healpix.jl,
       author = {{Tomasi}, Maurizio and {Li}, Zack},
        title = "{Healpix.jl: Julia-only port of the HEALPix library}",
     keywords = {Software},
      version = {3.0},
         year = 2021,
        month = sep,
          eid = {ascl:2109.028},
        pages = {ascl:2109.028},
archivePrefix = {ascl},
       eprint = {2109.028},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ascl.soft09028T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{PhysRevD.77.103013,
  title = {Likelihood analysis of CMB temperature and polarization power spectra},
  author = {Hamimeche, Samira and Lewis, Antony},
  journal = {Phys. Rev. D},
  volume = {77},
  issue = {10},
  pages = {103013},
  numpages = {28},
  year = {2008},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.77.103013},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.77.103013}
}

@article{Planck_LFI_beam,
	author = {{Planck Collaboration} and {Ade, P. A. R.} and {Aghanim, N.} and {Ashdown, M.} and {Aumont, J.} and {Baccigalupi, C.} and {Banday, A. J.} and {Barreiro, R. B.} and {Bartolo, N.} and {Battaner, E.} and {Benabed, K.} and {Beno\^{\i}t, A.} and {Benoit-L\'evy, A.} and {Bernard, J.-P.} and {Bersanelli, M.} and {Bielewicz, P.} and {Bock, J. J.} and {Bonaldi, A.} and {Bonavera, L.} and {Bond, J. R.} and {Borrill, J.} and {Bouchet, F. R.} and {Bucher, M.} and {Burigana, C.} and {Butler, R. C.} and {Calabrese, E.} and {Cardoso, J.-F.} and {Catalano, A.} and {Chamballu, A.} and {Christensen, P. R.} and {Colombi, S.} and {Colombo, L. P. L.} and {Crill, B. P.} and {Curto, A.} and {Cuttaia, F.} and {Danese, L.} and {Davies, R. D.} and {Davis, R. J.} and {de Bernardis, P.} and {de Rosa, A.} and {de Zotti, G.} and {Delabrouille, J.} and {Dickinson, C.} and {Diego, J. M.} and {Dole, H.} and {Donzelli, S.} and {Dor\'e, O.} and {Douspis, M.} and {Ducout, A.} and {Dupac, X.} and {Efstathiou, G.} and {Elsner, F.} and {En\ss{}lin, T. A.} and {Eriksen, H. K.} and {Fergusson, J.} and {Finelli, F.} and {Forni, O.} and {Frailis, M.} and {Franceschi, E.} and {Frejsel, A.} and {Galeotta, S.} and {Galli, S.} and {Ganga, K.} and {Giard, M.} and {Giraud-H\'eraud, Y.} and {Gjerl\o{}w, E.} and {Gonz\'alez-Nuevo, J.} and {G\'orski, K. M.} and {Gratton, S.} and {Gregorio, A.} and {Gruppuso, A.} and {Hansen, F. K.} and {Hanson, D.} and {Harrison, D. L.} and {Henrot-Versill\'e, S.} and {Herranz, D.} and {Hildebrandt, S. R.} and {Hivon, E.} and {Hobson, M.} and {Holmes, W. A.} and {Hornstrup, A.} and {Hovest, W.} and {Huffenberger, K. M.} and {Hurier, G.} and {Jaffe, A. H.} and {Jaffe, T. R.} and {Juvela, M.} and {Keih\"anen, E.} and {Keskitalo, R.} and {Kiiveri, K.} and {Kisner, T. S.} and {Knoche, J.} and {Kunz, M.} and {Kurki-Suonio, H.} and {L\"ahteenm\"aki, A.} and {Lamarre, J.-M.} and {Lasenby, A.} and {Lattanzi, M.} and {Lawrence, C. R.} and {Leahy, J. P.} and {Leonardi, R.} and {Lesgourgues, J.} and {Levrier, F.} and {Liguori, M.} and {Lilje, P. B.} and {Linden-V\o{}rnle, M.} and {Lindholm, V.} and {L\'opez-Caniego, M.} and {Lubin, P. M.} and {Mac\'{\i}as-P\'erez, J. F.} and {Maggio, G.} and {Maino, D.} and {Mandolesi, N.} and {Mangilli, A.} and {Maris, M.} and {Martin, P. G.} and {Mart\'{\i}nez-Gonz\'alez, E.} and {Masi, S.} and {Matarrese, S.} and {Mazzotta, P.} and {McGehee, P.} and {Meinhold, P. R.} and {Melchiorri, A.} and {Mendes, L.} and {Mennella, A.} and {Migliaccio, M.} and {Mitra, S.} and {Montier, L.} and {Morgante, G.} and {Mortlock, D.} and {Moss, A.} and {Munshi, D.} and {Murphy, J. A.} and {Naselsky, P.} and {Nati, F.} and {Natoli, P.} and {Netterfield, C. B.} and {N\o{}rgaard-Nielsen, H. U.} and {Novikov, D.} and {Novikov, I.} and {Paci, F.} and {Pagano, L.} and {Paoletti, D.} and {Partridge, B.} and {Pasian, F.} and {Patanchon, G.} and {Pearson, T. J.} and {Perdereau, O.} and {Perotto, L.} and {Perrotta, F.} and {Pettorino, V.} and {Piacentini, F.} and {Pierpaoli, E.} and {Pietrobon, D.} and {Pointecouteau, E.} and {Polenta, G.} and {Pratt, G. W.} and {Pr\'ezeau, G.} and {Prunet, S.} and {Puget, J.-L.} and {Rachen, J. P.} and {Rebolo, R.} and {Reinecke, M.} and {Remazeilles, M.} and {Renzi, A.} and {Rocha, G.} and {Rosset, C.} and {Rossetti, M.} and {Roudier, G.} and {Rubi\~no-Mart\'{\i}n, J. A.} and {Rusholme, B.} and {Sandri, M.} and {Santos, D.} and {Savelainen, M.} and {Scott, D.} and {Seiffert, M. D.} and {Shellard, E. P. S.} and {Spencer, L. D.} and {Stolyarov, V.} and {Sutton, D.} and {Suur-Uski, A.-S.} and {Sygnet, J.-F.} and {Tauber, J. A.} and {Terenzi, L.} and {Toffolatti, L.} and {Tomasi, M.} and {Tristram, M.} and {Tucci, M.} and {Tuovinen, J.} and {Umana, G.} and {Valenziano, L.} and {Valiviita, J.} and {Van Tent, B.} and {Vassallo, T.} and {Vielva, P.} and {Villa, F.} and {Wade, L. A.} and {Wandelt, B. D.} and {Watson, R.} and {Wehus, I. K.} and {Yvon, D.} and {Zacchei, A.} and {Zonca, A.}},
	title = {Planck 2015 results - IV. Low Frequency Instrument beams and window functions},
	DOI= "10.1051/0004-6361/201525809",
	url= "https://doi.org/10.1051/0004-6361/201525809",
	journal = {\aap},
	year = 2016,
	volume = 594,
	pages = "A4",
}

@article{Planck_HFI_beam,
	author = {{Planck Collaboration} and {Adam, R.} and {Ade, P. A. R.} and {Aghanim, N.} and {Arnaud, M.} and {Ashdown, M.} and {Aumont, J.} and {Baccigalupi, C.} and {Banday, A. J.} and {Barreiro, R. B.} and {Bartolo, N.} and {Battaner, E.} and {Benabed, K.} and {Beno\^{\i}t, A.} and {Benoit-L\'evy, A.} and {Bernard, J.-P.} and {Bersanelli, M.} and {Bertincourt, B.} and {Bielewicz, P.} and {Bock, J. J.} and {Bonavera, L.} and {Bond, J. R.} and {Borrill, J.} and {Bouchet, F. R.} and {Boulanger, F.} and {Bucher, M.} and {Burigana, C.} and {Calabrese, E.} and {Cardoso, J.-F.} and {Catalano, A.} and {Challinor, A.} and {Chamballu, A.} and {Chary, R.-R.} and {Chiang, H. C.} and {Christensen, P. R.} and {Clements, D. L.} and {Colombi, S.} and {Colombo, L. P. L.} and {Combet, C.} and {Couchot, F.} and {Coulais, A.} and {Crill, B. P.} and {Curto, A.} and {Cuttaia, F.} and {Danese, L.} and {Davies, R. D.} and {Davis, R. J.} and {de Bernardis, P.} and {de Rosa, A.} and {de Zotti, G.} and {Delabrouille, J.} and {Delouis, J.-M.} and {D\'esert, F.-X.} and {Diego, J. M.} and {Dole, H.} and {Donzelli, S.} and {Dor\'e, O.} and {Douspis, M.} and {Ducout, A.} and {Dupac, X.} and {Efstathiou, G.} and {Elsner, F.} and {En\ss{}lin, T. A.} and {Eriksen, H. K.} and {Falgarone, E.} and {Fergusson, J.} and {Finelli, F.} and {Forni, O.} and {Frailis, M.} and {Fraisse, A. A.} and {Franceschi, E.} and {Frejsel, A.} and {Galeotta, S.} and {Galli, S.} and {Ganga, K.} and {Ghosh, T.} and {Giard, M.} and {Giraud-H\'eraud, Y.} and {Gjerl\o{}w, E.} and {Gonz\'alez-Nuevo, J.} and {G\'orski, K. M.} and {Gratton, S.} and {Gruppuso, A.} and {Gudmundsson, J. E.} and {Hansen, F. K.} and {Hanson, D.} and {Harrison, D. L.} and {Henrot-Versill\'e, S.} and {Herranz, D.} and {Hildebrandt, S. R.} and {Hivon, E.} and {Hobson, M.} and {Holmes, W. A.} and {Hornstrup, A.} and {Hovest, W.} and {Huffenberger, K. M.} and {Hurier, G.} and {Jaffe, A. H.} and {Jaffe, T. R.} and {Jones, W. C.} and {Juvela, M.} and {Keih\"anen, E.} and {Keskitalo, R.} and {Kisner, T. S.} and {Kneissl, R.} and {Knoche, J.} and {Kunz, M.} and {Kurki-Suonio, H.} and {Lagache, G.} and {Lamarre, J.-M.} and {Lasenby, A.} and {Lattanzi, M.} and {Lawrence, C. R.} and {Le Jeune, M.} and {Leahy, J. P.} and {Lellouch, E.} and {Leonardi, R.} and {Lesgourgues, J.} and {Levrier, F.} and {Liguori, M.} and {Lilje, P. B.} and {Linden-V\o{}rnle, M.} and {L\'opez-Caniego, M.} and {Lubin, P. M.} and {Mac\'{\i}as-P\'erez, J. F.} and {Maggio, G.} and {Maino, D.} and {Mandolesi, N.} and {Mangilli, A.} and {Maris, M.} and {Martin, P. G.} and {Mart\'{\i}nez-Gonz\'alez, E.} and {Masi, S.} and {Matarrese, S.} and {McGehee, P.} and {Melchiorri, A.} and {Mendes, L.} and {Mennella, A.} and {Migliaccio, M.} and {Mitra, S.} and {Miville-Desch\^enes, M.-A.} and {Moneti, A.} and {Montier, L.} and {Moreno, R.} and {Morgante, G.} and {Mortlock, D.} and {Moss, A.} and {Mottet, S.} and {Munshi, D.} and {Murphy, J. A.} and {Naselsky, P.} and {Nati, F.} and {Natoli, P.} and {Netterfield, C. B.} and {N\o{}rgaard-Nielsen, H. U.} and {Noviello, F.} and {Novikov, D.} and {Novikov, I.} and {Oxborrow, C. A.} and {Paci, F.} and {Pagano, L.} and {Pajot, F.} and {Paoletti, D.} and {Pasian, F.} and {Patanchon, G.} and {Pearson, T. J.} and {Perdereau, O.} and {Perotto, L.} and {Perrotta, F.} and {Pettorino, V.} and {Piacentini, F.} and {Piat, M.} and {Pierpaoli, E.} and {Pietrobon, D.} and {Plaszczynski, S.} and {Pointecouteau, E.} and {Polenta, G.} and {Pratt, G. W.} and {Pr\'ezeau, G.} and {Prunet, S.} and {Puget, J.-L.} and {Rachen, J. P.} and {Reinecke, M.} and {Remazeilles, M.} and {Renault, C.} and {Renzi, A.} and {Ristorcelli, I.} and {Rocha, G.} and {Rosset, C.} and {Rossetti, M.} and {Roudier, G.} and {Rowan-Robinson, M.} and {Rusholme, B.} and {Sandri, M.} and {Santos, D.} and {Sauv\'e, A.} and {Savelainen, M.} and {Savini, G.} and {Scott, D.} and {Seiffert, M. D.} and {Shellard, E. P. S.} and {Spencer, L. D.} and {Stolyarov, V.} and {Stompor, R.} and {Sudiwala, R.} and {Sutton, D.} and {Suur-Uski, A.-S.} and {Sygnet, J.-F.} and {Tauber, J. A.} and {Terenzi, L.} and {Toffolatti, L.} and {Tomasi, M.} and {Tristram, M.} and {Tucci, M.} and {Tuovinen, J.} and {Valenziano, L.} and {Valiviita, J.} and {Van Tent, B.} and {Vibert, L.} and {Vielva, P.} and {Villa, F.} and {Wade, L. A.} and {Wandelt, B. D.} and {Watson, R.} and {Wehus, I. K.} and {Yvon, D.} and {Zacchei, A.} and {Zonca, A.}},
	title = {Planck 2015 results - VII. High Frequency Instrument data processing: Time-ordered information  and beams},
	DOI= "10.1051/0004-6361/201525844",
	url= "https://doi.org/10.1051/0004-6361/201525844",
	journal = {\aap},
	year = 2016,
	volume = 594,
	pages = "A7",
}

@article{binning_map,
    author = {Brown, Michael L. and Challinor, Anthony and North, Chris E. and Johnson, Bradley R. and O'Dea, Daniel and Sutton, David},
    title = "{Impact of modulation on CMB B-mode polarization experiments}",
    journal = {\mnras},
    volume = {397},
    number = {2},
    pages = {634-656},
    year = {2009},
    month = {07},
    abstract = "{We investigate the impact of both slow and fast polarization modulation strategies on the science return of upcoming ground-based experiments aimed at measuring the B-mode polarization of the cosmic microwave background. Using detailed simulations of the Cℓ OVER experiment, we compare the ability of modulated and un-modulated observations to recover the signature of gravitational waves in the polarized CMB sky in the presence of a number of anticipated systematic effects. The general expectations that fast modulation is helpful in mitigating low-frequency detector noise, and that the additional redundancy in the projection of the instrument's polarization sensitivity directions on to the sky when modulating reduces the impact of instrumental polarization, particularly for fast modulation, are borne out by our simulations. Neither low-frequency polarized atmospheric fluctuations nor systematic errors in the polarization sensitivity directions are mitigated by modulation. Additionally, we find no significant reduction in the effect of pointing errors by modulation. For a Cℓ OVER-like experiment, pointing jitter should be negligible but any systematic miscalibration of the polarization coordinate reference system results in significant E–B mixing on all angular scales and will require careful control. We also stress the importance of combining data from multiple detectors in order to remove the effects of common-mode systematics (such as un-polarized 1/f atmospheric noise) on the measured polarization signal. Finally we compare the performance of our simulated experiment with the predicted performance from a Fisher analysis. We find good agreement between the (optimal) Fisher predictions and the simulated experiment except for the very largest scales where the power spectrum estimator we have used introduces additional variance to the B-mode signal recovered from our simulations. In terms of detecting the total B-mode signal, including lensing, the Fisher analysis and the simulations are in excellent agreement. For a detection of the primordial B-mode signal only, using an input tensor-to-scalar ratio of r= 0.026, the Fisher analysis predictions are ∼20 per cent better than the simulated performance.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2009.14975.x},
    url = {https://doi.org/10.1111/j.1365-2966.2009.14975.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/397/2/634/18195060/mnras0397-0634.pdf},
}

@ARTICLE{planck2018,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Battye}, R. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Challinor}, A. and {Chiang}, H.~C. and {Chluba}, J. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Farhang}, M. and {Fergusson}, J. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Karakci}, A. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Knox}, L. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Lemos}, P. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Lilley}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sirri}, G. and {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. VI. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201833910},
archivePrefix = {arXiv},
       eprint = {1807.06209},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...6P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{wallis_new_map-making,
       author = {{Wallis}, Christopher G.~R. and {Bonaldi}, A. and {Brown}, Michael L. and {Battye}, Richard A.},
        title = "{A new map-making algorithm for CMB polarization experiments}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = oct,
       volume = {453},
       number = {2},
        pages = {2058-2069},
          doi = {10.1093/mnras/stv1689},
archivePrefix = {arXiv},
       eprint = {1503.03285},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453.2058W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{berry1978,
    author = {Berry, M. V.},
    title = "{Regular and irregular motion}",
    journal = {AIP Conference Proceedings},
    volume = {46},
    number = {1},
    pages = {16-120},
    year = {1978},
    month = {09},
    issn = {0094-243X},
    doi = {10.1063/1.31417},
    url = {https://doi.org/10.1063/1.31417},
    eprint = {https://pubs.aip.org/aip/acp/article-pdf/46/1/16/11659773/16\_1\_online.pdf},
}

@ARTICLE{Bennett2003,
       author = {{Bennett}, C.~L. and {Bay}, M. and {Halpern}, M. and {Hinshaw}, G. and {Jackson}, C. and {Jarosik}, N. and {Kogut}, A. and {Limon}, M. and {Meyer}, S.~S. and {Page}, L. and {Spergel}, D.~N. and {Tucker}, G.~S. and {Wilkinson}, D.~T. and {Wollack}, E. and {Wright}, E.~L.},
        title = "{The Microwave Anisotropy Probe Mission}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Cosmology: Dark Matter, Cosmology: Early Universe, Space Vehicles: Instruments, Astrophysics},
         year = 2003,
        month = jan,
       volume = {583},
       number = {1},
        pages = {1-23},
          doi = {10.1086/345346},
archivePrefix = {arXiv},
       eprint = {astro-ph/0301158},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...583....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SO-SAT_HWP,
       author = {{Yamada}, K. and {Bixler}, B. and {Sakurai}, Y. and {Ashton}, P.~C. and {Sugiyama}, J. and {Arnold}, K. and {Begin}, J. and {Corbett}, L. and {Day-Weiss}, S. and {Galitzki}, N. and {Hill}, C.~A. and {Johnson}, B.~R. and {Jost}, B. and {Kusaka}, A. and {Koopman}, B.~J. and {Lashner}, J. and {Lee}, A.~T. and {Mangu}, A. and {Nishino}, H. and {Page}, L.~A. and {Randall}, M.~J. and {Sasaki}, D. and {Song}, X. and {Spisak}, J. and {Tsan}, T. and {Wang}, Y. and {Williams}, P.~A.},
        title = "{The Simons Observatory: Cryogenic Half Wave Plate Rotation Mechanism for the Small Aperture Telescopes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = sep,
          eid = {arXiv:2309.14803},
        pages = {arXiv:2309.14803},
          doi = {10.48550/arXiv.2309.14803},
archivePrefix = {arXiv},
       eprint = {2309.14803},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv230914803Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PB_HWP,
       author = {{Hill}, C.~A. and {Kusaka}, A. and {Ashton}, P. and {Barton}, P. and {Adkins}, T. and {Arnold}, K. and {Bixler}, B. and {Ganjam}, S. and {Lee}, A.~T. and {Matsuda}, F. and {Matsumura}, T. and {Sakurai}, Y. and {Tat}, R. and {Zhou}, Y.},
        title = "{A cryogenic continuously rotating half-wave plate mechanism for the POLARBEAR-2b cosmic microwave background receiver}",
      journal = {Review of Scientific Instruments},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
       volume = {91},
       number = {12},
          eid = {124503},
        pages = {124503},
          doi = {10.1063/5.0029006},
archivePrefix = {arXiv},
       eprint = {2009.03972},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020RScI...91l4503H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{B-mode_Seljak,
       author = {{Seljak}, Uro{\v{s}} and {Zaldarriaga}, Matias},
        title = "{Signature of Gravity Waves in the Polarization of the Microwave Background}",
      journal = {Physical Review Letters},
     keywords = {Astrophysics, General Relativity and Quantum Cosmology},
         year = 1997,
        month = mar,
       volume = {78},
       number = {11},
        pages = {2054-2057},
          doi = {10.1103/PhysRevLett.78.2054},
archivePrefix = {arXiv},
       eprint = {astro-ph/9609169},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvL..78.2054S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{B-mode_Kamionkowski,
       author = {{Kamionkowski}, Marc and {Kosowsky}, Arthur and {Stebbins}, Albert},
        title = "{A Probe of Primordial Gravity Waves and Vorticity}",
      journal = {Physical Review Letters},
     keywords = {Astrophysics, High Energy Physics - Phenomenology},
         year = 1997,
        month = mar,
       volume = {78},
       number = {11},
        pages = {2058-2061},
          doi = {10.1103/PhysRevLett.78.2058},
archivePrefix = {arXiv},
       eprint = {astro-ph/9609132},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvL..78.2058K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{healpix_primer,
       author = {{Gorski}, Krzysztof M. and {Wandelt}, Benjamin D. and {Hansen}, Frode K. and {Hivon}, Eric and {Banday}, Anthony J.},
        title = "{The HEALPix Primer}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = 1999,
        month = may,
          eid = {astro-ph/9905275},
        pages = {astro-ph/9905275},
          doi = {10.48550/arXiv.astro-ph/9905275},
archivePrefix = {arXiv},
       eprint = {astro-ph/9905275},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999astro.ph..5275G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BICEP_syst,
       author = {{Bicep2 Collaboration} and {Ade}, P.~A.~R. and {Aikin}, R.~W. and {Barkats}, D. and {Benton}, S.~J. and {Bischoff}, C.~A. and {Bock}, J.~J. and {Brevik}, J.~A. and {Buder}, I. and {Bullock}, E. and {Dowell}, C.~D. and {Duband}, L. and {Filippini}, J.~P. and {Fliescher}, S. and {Golwala}, S.~R. and {Halpern}, M. and {Hasselfield}, M. and {Hildebrandt}, S.~R. and {Hilton}, G.~C. and {Irwin}, K.~D. and {Karkare}, K.~S. and {Kaufman}, J.~P. and {Keating}, B.~G. and {Kernasovskiy}, S.~A. and {Kovac}, J.~M. and {Kuo}, C.~L. and {Leitch}, E.~M. and {Lueker}, M. and {Netterfield}, C.~B. and {Nguyen}, H.~T. and {O'Brient}, R. and {Ogburn}, R.~W., IV and {Orlando}, A. and {Pryke}, C. and {Richter}, S. and {Schwarz}, R. and {Sheehy}, C.~D. and {Staniszewski}, Z.~K. and {Sudiwala}, R.~V. and {Teply}, G.~P. and {Tolan}, J.~E. and {Turner}, A.~D. and {Vieregg}, A.~G. and {Wong}, C.~L. and {Yoon}, K.~W.},
        title = "{Bicep2 III: Instrumental Systematics}",
      journal = {\apj},
     keywords = {cosmic background radiation, cosmology: observations, gravitational waves, inflation, instrumentation: polarimeters, methods: data analysis, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = dec,
       volume = {814},
       number = {2},
          eid = {110},
        pages = {110},
          doi = {10.1088/0004-637X/814/2/110},
archivePrefix = {arXiv},
       eprint = {1502.00608},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...814..110B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guillaume_HWPIP,
       author = {{Patanchon}, Guillaume and {Imada}, Hiroaki and {Ishino}, Hirokazu and {Matsumura}, Tomotake},
        title = "{Effect of instrumental polarization with a half-wave plate on the B-mode signal: prediction and correction}",
      journal = {\jcap},
     keywords = {CMBR experiments, CMBR polarisation, Statistical sampling techniques, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2024,
        month = apr,
       volume = {2024},
       number = {4},
          eid = {074},
        pages = {074},
          doi = {10.1088/1475-7516/2024/04/074},
archivePrefix = {arXiv},
       eprint = {2308.00967},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024JCAP...04..074P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{planck_prelaunch2010,
       author = {{Tauber}, J.~A. and {Mandolesi}, N. and {Puget}, J. -L. and {Banos}, T. and {Bersanelli}, M. and {Bouchet}, F.~R. and {Butler}, R.~C. and {Charra}, J. and {Crone}, G. and {Dodsworth}, J. and {Efstathiou}, G. and {Gispert}, R. and {Guyot}, G. and {Gregorio}, A. and {Juillet}, J.~J. and {Lamarre}, J. -M. and {Laureijs}, R.~J. and {Lawrence}, C.~R. and {N{\o}rgaard-Nielsen}, H.~U. and {Passvogel}, T. and {Reix}, J.~M. and {Texier}, D. and {Vibert}, L. and {Zacchei}, A. and {Ade}, P.~A.~R. and {Aghanim}, N. and {Aja}, B. and {Alippi}, E. and {Aloy}, L. and {Armand}, P. and {Arnaud}, M. and {Arondel}, A. and {Arreola-Villanueva}, A. and {Artal}, E. and {Artina}, E. and {Arts}, A. and {Ashdown}, M. and {Aumont}, J. and {Azzaro}, M. and {Bacchetta}, A. and {Baccigalupi}, C. and {Baker}, M. and {Balasini}, M. and {Balbi}, A. and {Banday}, A.~J. and {Barbier}, G. and {Barreiro}, R.~B. and {Bartelmann}, M. and {Battaglia}, P. and {Battaner}, E. and {Benabed}, K. and {Beney}, J. -L. and {Beneyton}, R. and {Bennett}, K. and {Benoit}, A. and {Bernard}, J. -P. and {Bhandari}, P. and {Bhatia}, R. and {Biggi}, M. and {Biggins}, R. and {Billig}, G. and {Blanc}, Y. and {Blavot}, H. and {Bock}, J.~J. and {Bonaldi}, A. and {Bond}, R. and {Bonis}, J. and {Borders}, J. and {Borrill}, J. and {Boschini}, L. and {Boulanger}, F. and {Bouvier}, J. and {Bouzit}, M. and {Bowman}, R. and {Br{\'e}elle}, E. and {Bradshaw}, T. and {Braghin}, M. and {Bremer}, M. and {Brienza}, D. and {Broszkiewicz}, D. and {Burigana}, C. and {Burkhalter}, M. and {Cabella}, P. and {Cafferty}, T. and {Cairola}, M. and {Caminade}, S. and {Camus}, P. and {Cantalupo}, C.~M. and {Cappellini}, B. and {Cardoso}, J. -F. and {Carr}, R. and {Catalano}, A. and {Cay{\'o}n}, L. and {Cesa}, M. and {Chaigneau}, M. and {Challinor}, A. and {Chamballu}, A. and {Chambelland}, J.~P. and {Charra}, M. and {Chiang}, L. -Y. and {Chlewicki}, G. and {Christensen}, P.~R. and {Church}, S. and {Ciancietta}, E. and {Cibrario}, M. and {Cizeron}, R. and {Clements}, D. and {Collaudin}, B. and {Colley}, J. -M. and {Colombi}, S. and {Colombo}, A. and {Colombo}, F. and {Corre}, O. and {Couchot}, F. and {Cougrand}, B. and {Coulais}, A. and {Couzin}, P. and {Crane}, B. and {Crill}, B. and {Crook}, M. and {Crumb}, D. and {Cuttaia}, F. and {D{\"o}rl}, U. and {da Silva}, P. and {Daddato}, R. and {Damasio}, C. and {Danese}, L. and {D'Aquino}, G. and {D'Arcangelo}, O. and {Dassas}, K. and {Davies}, R.~D. and {Davies}, W. and {Davis}, R.~J. and {de Bernardis}, P. and {de Chambure}, D. and {de Gasperis}, G. and {de La Fuente}, M.~L. and {de Paco}, P. and {de Rosa}, A. and {de Troia}, G. and {de Zotti}, G. and {Dehamme}, M. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {di Girolamo}, G. and {Dickinson}, C. and {Doelling}, E. and {Dolag}, K. and {Domken}, I. and {Douspis}, M. and {Doyle}, D. and {Du}, S. and {Dubruel}, D. and {Dufour}, C. and {Dumesnil}, C. and {Dupac}, X. and {Duret}, P. and {Eder}, C. and {Elfving}, A. and {En{\ss}lin}, T.~A. and {Eng}, P. and {English}, K. and {Eriksen}, H.~K. and {Estaria}, P. and {Falvella}, M.~C. and {Ferrari}, F. and {Finelli}, F. and {Fishman}, A. and {Fogliani}, S. and {Foley}, S. and {Fonseca}, A. and {Forma}, G. and {Forni}, O. and {Fosalba}, P. and {Fourmond}, J. -J. and {Frailis}, M. and {Franceschet}, C. and {Franceschi}, E. and {Fran{\c{c}}ois}, S. and {Frerking}, M. and {G{\'o}mez-Re{\~n}asco}, M.~F. and {G{\'o}rski}, K.~M. and {Gaier}, T.~C. and {Galeotta}, S. and {Ganga}, K. and {Garc{\'\i}a L{\'a}zaro}, J. and {Garnica}, A. and {Gaspard}, M. and {Gavila}, E. and {Giard}, M. and {Giardino}, G. and {Gienger}, G. and {Giraud-Heraud}, Y. and {Glorian}, J. -M. and {Griffin}, M. and {Gruppuso}, A. and {Guglielmi}, L. and {Guichon}, D. and {Guillaume}, B. and {Guillouet}, P. and {Haissinski}, J. and {Hansen}, F.~K. and {Hardy}, J. and {Harrison}, D. and {Hazell}, A. and {Hechler}, M. and {Heckenauer}, V. and {Heinzer}, D. and {Hell}, R. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Herreros}, J.~M. and {Hervier}, V. and {Heske}, A. and {Heurtel}, A. and {Hildebrandt}, S.~R. and {Hills}, R. and {Hivon}, E. and {Hobson}, M. and {Hollert}, D. and {Holmes}, W. and {Hornstrup}, A. and {Hovest}, W. and {Hoyland}, R.~J. and {Huey}, G. and {Huffenberger}, K.~M. and {Hughes}, N. and {Israelsson}, U. and {Jackson}, B. and {Jaffe}, A. and {Jaffe}, T.~R. and {Jagemann}, T. and {Jessen}, N.~C. and {Jewell}, J. and {Jones}, W. and {Juvela}, M. and {Kaplan}, J. and {Karlman}, P. and {Keck}, F. and {Keih{\"a}nen}, E. and {King}, M. and {Kisner}, T.~S. and {Kletzkine}, P. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Koch}, T. and {Krassenburg}, M. and {Kurki-Suonio}, H. and {L{\"a}hteenm{\"a}ki}, A. and {Lagache}, G. and {Lagorio}, E. and {Lami}, P. and {Lande}, J. and {Lange}, A. and {Langlet}, F. and {Lapini}, R. and {Lapolla}, M. and {Lasenby}, A. and {Le Jeune}, M. and {Leahy}, J.~P. and {Lefebvre}, M. and {Legrand}, F. and {Le Meur}, G. and {Leonardi}, R. and {Leriche}, B. and {Leroy}, C. and {Leutenegger}, P. and {Levin}, S.~M. and {Lilje}, P.~B. and {Lindensmith}, C. and {Linden-V{\o}rnle}, M. and {Loc}, A. and {Longval}, Y. and {Lubin}, P.~M. and {Luchik}, T. and {Luthold}, I. and {Macias-Perez}, J.~F. and {Maciaszek}, T. and {MacTavish}, C. and {Madden}, S. and {Maffei}, B. and {Magneville}, C. and {Maino}, D. and {Mambretti}, A. and {Mansoux}, B. and {Marchioro}, D. and {Maris}, M. and {Marliani}, F. and {Marrucho}, J. -C. and {Mart{\'\i}-Canales}, J. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Mart{\'\i}n-Polegre}, A. and {Martin}, P. and {Marty}, C. and {Marty}, W. and {Masi}, S. and {Massardi}, M. and {Matarrese}, S. and {Matthai}, F. and {Mazzotta}, P. and {McDonald}, A. and {McGrath}, P. and {Mediavilla}, A. and {Meinhold}, P.~R. and {M{\'e}lin}, J. -B. and {Melot}, F. and {Mendes}, L. and {Mennella}, A. and {Mervier}, C. and {Meslier}, L. and {Miccolis}, M. and {Miville-Deschenes}, M. -A. and {Moneti}, A. and {Montet}, D. and {Montier}, L. and {Mora}, J. and {Morgante}, G. and {Morigi}, G. and {Morinaud}, G. and {Morisset}, N. and {Mortlock}, D. and {Mottet}, S. and {Mulder}, J. and {Munshi}, D. and {Murphy}, A. and {Murphy}, P. and {Musi}, P. and {Narbonne}, J. and {Naselsky}, P. and {Nash}, A. and {Nati}, F. and {Natoli}, P. and {Netterfield}, B. and {Newell}, J. and {Nexon}, M. and {Nicolas}, C. and {Nielsen}, P.~H. and {Ninane}, N. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {O'Dwyer}, I.~J. and {Oldeman}, P. and {Olivier}, P. and {Ouchet}, L. and {Oxborrow}, C.~A. and {P{\'e}rez-Cuevas}, L. and {Pagan}, L. and {Paine}, C. and {Pajot}, F. and {Paladini}, R. and {Pancher}, F. and {Panh}, J. and {Parks}, G. and {Parnaudeau}, P. and {Partridge}, B. and {Parvin}, B. and {Pascual}, J.~P. and {Pasian}, F. and {Pearson}, D.~P. and {Pearson}, T. and {Pecora}, M. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Piersanti}, O. and {Plaige}, E. and {Plaszczynski}, S. and {Platania}, P. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Popa}, L. and {Poulleau}, G. and {Poutanen}, T. and {Pr{\'e}zeau}, G. and {Pradell}, L. and {Prina}, M. and {Prunet}, S. and {Rachen}, J.~P. and {Rambaud}, D. and {Rame}, F. and {Rasmussen}, I. and {Rautakoski}, J. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Reiter}, J. and {Renault}, C. and {Ricciardi}, S. and {Rideau}, P. and {Riller}, T. and {Ristorcelli}, I. and {Riti}, J.~B. and {Rocha}, G. and {Roche}, Y. and {Pons}, R. and {Rohlfs}, R. and {Romero}, D. and {Roose}, S. and {Rosset}, C. and {Rouberol}, S. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusconi}, P. and {Rusholme}, B. and {Salama}, M. and {Salerno}, E. and {Sandri}, M. and {Santos}, D. and {Sanz}, J.~L. and {Sauter}, L. and {Sauvage}, F. and {Savini}, G. and {Schmelzel}, M. and {Schnorhk}, A. and {Schwarz}, W. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, P. and {Shih}, C. and {Sias}, M. and {Silk}, J.~I. and {Silvestri}, R. and {Sippel}, R. and {Smoot}, G.~F. and {Starck}, J. -L. and {Stassi}, P. and {Sternberg}, J. and {Stivoli}, F. and {Stolyarov}, V. and {Stompor}, R. and {Stringhetti}, L. and {Strommen}, D. and {Stute}, T. and {Sudiwala}, R. and {Sugimura}, R. and {Sunyaev}, R. and {Sygnet}, J. -F. and {T{\"u}rler}, M. and {Taddei}, E. and {Tallon}, J. and {Tamiatto}, C. and {Taurigna}, M. and {Taylor}, D. and {Terenzi}, L. and {Thuerey}, S. and {Tillis}, J. and {Tofani}, G. and {Toffolatti}, L. and {Tommasi}, E. and {Tomasi}, M. and {Tonazzini}, E. and {Torre}, J. -P. and {Tosti}, S. and {Touze}, F. and {Tristram}, M. and {Tuovinen}, J. and {Tuttlebee}, M. and {Umana}, G. and {Valenziano}, L. and {Vall{\'e}e}, D. and {van der Vlis}, M. and {van Leeuwen}, F. and {Vanel}, J. -C. and {van-Tent}, B. and {Varis}, J. and {Vassallo}, E. and {Vescovi}, C. and {Vezzu}, F. and {Vibert}, D. and {Vielva}, P. and {Vierra}, J. and {Villa}, F. and {Vittorio}, N. and {Vuerli}, C. and {Wade}, L.~A. and {Walker}, A.~R. and {Wandelt}, B.~D. and {Watson}, C. and {Werner}, D. and {White}, M. and {White}, S.~D.~M. and {Wilkinson}, A. and {Wilson}, P. and {Woodcraft}, A. and {Yoffo}, B. and {Yun}, M. and {Yurchenko}, V. and {Yvon}, D. and {Zhang}, B. and {Zimmermann}, O. and {Zonca}, A. and {Zorita}, D.},
        title = "{Planck pre-launch status: The Planck mission}",
      journal = {\aap},
     keywords = {cosmic microwave background, space vehicles: instruments, instrumentation: detectors, instrumentation: polarimeters, submillimeter: general, radio continuum: general},
         year = 2010,
        month = sep,
       volume = {520},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/200912983},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...520A...1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PICO2019,
       author = {{Hanany}, Shaul and {Alvarez}, Marcelo and {Artis}, Emmanuel and {Ashton}, Peter and {Aumont}, Jonathan and {Aurlien}, Ragnhild and {Banerji}, Ranajoy and {Barreiro}, R. Belen and {Bartlett}, James G. and {Basak}, Soumen and {Battaglia}, Nick and {Bock}, Jamie and {Boddy}, Kimberly K. and {Bonato}, Matteo and {Borrill}, Julian and {Bouchet}, Fran{\c{c}}ois and {Boulanger}, Fran{\c{c}}ois and {Burkhart}, Blakesley and {Chluba}, Jens and {Chuss}, David and {Clark}, Susan E. and {Cooperrider}, Joelle and {Crill}, Brendan P. and {De Zotti}, Gianfranco and {Delabrouille}, Jacques and {Di Valentino}, Eleonora and {Didier}, Joy and {Dor{\'e}}, Olivier and {Eriksen}, Hans K. and {Errard}, Josquin and {Essinger-Hileman}, Tom and {Feeney}, Stephen and {Filippini}, Jeffrey and {Fissel}, Laura and {Flauger}, Raphael and {Fuskeland}, Unni and {Gluscevic}, Vera and {Gorski}, Krzysztof M. and {Green}, Dan and {Hensley}, Brandon and {Herranz}, Diego and {Hill}, J. Colin and {Hivon}, Eric and {Hlo{\v{z}}ek}, Ren{\'e}e and {Hubmayr}, Johannes and {Johnson}, Bradley R. and {Jones}, William and {Jones}, Terry and {Knox}, Lloyd and {Kogut}, Al and {L{\'o}pez-Caniego}, Marcos and {Lawrence}, Charles and {Lazarian}, Alex and {Li}, Zack and {Madhavacheril}, Mathew and {Melin}, Jean-Baptiste and {Meyers}, Joel and {Murray}, Calum and {Negrello}, Mattia and {Novak}, Giles and {O'Brient}, Roger and {Paine}, Christopher and {Pearson}, Tim and {Pogosian}, Levon and {Pryke}, Clem and {Puglisi}, Giuseppe and {Remazeilles}, Mathieu and {Rocha}, Graca and {Schmittfull}, Marcel and {Scott}, Douglas and {Shirron}, Peter and {Stephens}, Ian and {Sutin}, Brian and {Tomasi}, Maurizio and {Trangsrud}, Amy and {van Engelen}, Alexander and {Vansyngel}, Flavien and {Wehus}, Ingunn K. and {Wen}, Qi and {Xu}, Siyao and {Young}, Karl and {Zonca}, Andrea},
        title = "{PICO: Probe of Inflation and Cosmic Origins}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
          eid = {arXiv:1902.10541},
        pages = {arXiv:1902.10541},
          doi = {10.48550/arXiv.1902.10541},
archivePrefix = {arXiv},
       eprint = {1902.10541},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190210541H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{planck2016_scanning_beam,
       author = {{Planck Collaboration} and {Adam}, R. and {Ade}, P.~A.~R. and {Aghanim}, N. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Battaner}, E. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bertincourt}, B. and {Bielewicz}, P. and {Bock}, J.~J. and {Bonavera}, L. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {Diego}, J.~M. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fergusson}, J. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frejsel}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gjerl{\o}w}, E. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D.~L. and {Henrot-Versill{\'e}}, S. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Huffenberger}, K.~M. and {Hurier}, G. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Leahy}, J.~P. and {Lellouch}, E. and {Leonardi}, R. and {Lesgourgues}, J. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {McGehee}, P. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Moreno}, R. and {Morgante}, G. and {Mortlock}, D. and {Moss}, A. and {Mottet}, S. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paoletti}, D. and {Pasian}, F. and {Patanchon}, G. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rossetti}, M. and {Roudier}, G. and {Rowan-Robinson}, M. and {Rusholme}, B. and {Sandri}, M. and {Santos}, D. and {Sauv{\'e}}, A. and {Savelainen}, M. and {Savini}, G. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, E.~P.~S. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Tuovinen}, J. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Watson}, R. and {Wehus}, I.~K. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2015 results. VII. High Frequency Instrument data processing: Time-ordered information and beams}",
      journal = {\aap},
     keywords = {methods: data analysis, cosmic background radiation, instrumentation: detectors, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = sep,
       volume = {594},
          eid = {A7},
        pages = {A7},
          doi = {10.1051/0004-6361/201525844},
archivePrefix = {arXiv},
       eprint = {1502.01586},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A...7P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{TES_2022,
    author = "Hubmayr, J. and others",
    collaboration = "LiteBIRD",
    title = "{Optical Characterization of OMT-Coupled TES Bolometers for LiteBIRD}",
    doi = "10.1007/s10909-022-02808-7",
    journal = "J. Low Temp. Phys.",
    volume = "209",
    number = "3-4",
    pages = "396--408",
    year = "2022"
}

@ARTICLE{far_sidelobe,
       author = {{Leloup}, C. and {Patanchon}, G. and {Errard}, J. and {Franceschet}, C. and {Gudmundsson}, J.~E. and {Henrot-Versill{\'e}}, S. and {Imada}, H. and {Ishino}, H. and {Matsumura}, T. and {Puglisi}, G. and {Wang}, W. and {Adler}, A. and {Aumont}, J. and {Aurlien}, R. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basyrov}, A. and {Bersanelli}, M. and {Blinov}, D. and {Bortolami}, M. and {Brinckmann}, T. and {Campeti}, P. and {Carones}, A. and {Carralot}, F. and {Casas}, F.~J. and {Cheung}, K. and {Clermont}, L. and {Columbro}, F. and {Conenna}, G. and {Coppolecchia}, A. and {Cuttaia}, F. and {Dachlythra}, N. and {D'Alessandro}, G. and {de Bernardis}, P. and {de Haan}, T. and {De Petris}, M. and {Della Torre}, S. and {Diego-Palazuelos}, P. and {Eriksen}, H.~K. and {Finelli}, F. and {Fuskeland}, U. and {Galloni}, G. and {Galloway}, M. and {Georges}, M. and {Gerbino}, M. and {Gervasi}, M. and {G{\'e}nova-Santos}, R.~T. and {Ghigna}, T. and {Giardiello}, S. and {Gimeno-Amo}, C. and {Gjerl{\o}w}, E. and {Gruppuso}, A. and {Hazumi}, M. and {Hergt}, L.~T. and {Herranz}, D. and {Hivon}, E. and {Hoang}, T.~D. and {Jost}, B. and {Kohri}, K. and {Krachmalnicoff}, N. and {Lee}, A.~T. and {Lembo}, M. and {Levrier}, F. and {Lonappan}, A.~I. and {L{\'o}pez-Caniego}, M. and {Macias-Perez}, J. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {Micheli}, S. and {Monelli}, M. and {Montier}, L. and {Morgante}, G. and {Mot}, B. and {Mousset}, L. and {Namikawa}, T. and {Natoli}, P. and {Novelli}, A. and {Noviello}, F. and {Obata}, I. and {Odagiri}, K. and {Pagano}, L. and {Paiella}, A. and {Paoletti}, D. and {Pascual-Cisneros}, G. and {Pavlidou}, V. and {Piacentini}, F. and {Piccirilli}, G. and {Pisano}, G. and {Polenta}, G. and {Raffuzzi}, N. and {Remazeilles}, M. and {Ritacco}, A. and {Rizzieri}, A. and {Ruiz-Granda}, M. and {Sakurai}, Y. and {Shiraishi}, M. and {Stever}, S.~L. and {Takase}, Y. and {Tassis}, K. and {Terenzi}, L. and {Thompson}, K.~L. and {Tristram}, M. and {Vacher}, L. and {Vielva}, P. and {Wehus}, I.~K. and {Weymann-Despres}, G. and {Zannoni}, M. and {Zhou}, Y. and {LiteBIRD Collaboration}},
        title = "{Impact of beam far side-lobe knowledge in the presence of foregrounds for LiteBIRD}",
      journal = {\jcap},
     keywords = {CMBR experiments, CMBR polarisation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = jun,
       volume = {2024},
       number = {6},
          eid = {011},
        pages = {011},
          doi = {10.1088/1475-7516/2024/06/011},
archivePrefix = {arXiv},
       eprint = {2312.09001},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024JCAP...06..011L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@software{CAMB,
       author = {{Lewis}, Antony and {Challinor}, Anthony},
        title = "{CAMB: Code for Anisotropies in the Microwave Background}",
 howpublished = {Astrophysics Source Code Library, record ascl:1102.026},
         year = 2011,
        month = feb,
          eid = {ascl:1102.026},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ascl.soft02026L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {759-771},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Julia-2017,
    title={Julia: A fresh approach to numerical computing},
    author={Bezanson, Jeff and Edelman, Alan and Karpinski, Stefan and Shah, Viral B},
    journal={SIAM Review},
    volume={59},
    number={1},
    pages={65--98},
    year={2017},
    publisher={SIAM},
    doi={10.1137/141000671},
    url={https://epubs.siam.org/doi/10.1137/141000671}
}

@ARTICLE{astropy,
       author = {{Astropy Collaboration} and {Price-Whelan}, Adrian M. and {Lim}, Pey Lian and {Earl}, Nicholas and {Starkman}, Nathaniel and {Bradley}, Larry and {Shupe}, David L. and {Patil}, Aarya A. and {Corrales}, Lia and {Brasseur}, C.~E. and {N{\"o}the}, Maximilian and {Donath}, Axel and {Tollerud}, Erik and {Morris}, Brett M. and {Ginsburg}, Adam and {Vaher}, Eero and {Weaver}, Benjamin A. and {Tocknell}, James and {Jamieson}, William and {van Kerkwijk}, Marten H. and {Robitaille}, Thomas P. and {Merry}, Bruce and {Bachetti}, Matteo and {G{\"u}nther}, H. Moritz and {Aldcroft}, Thomas L. and {Alvarado-Montes}, Jaime A. and {Archibald}, Anne M. and {B{\'o}di}, Attila and {Bapat}, Shreyas and {Barentsen}, Geert and {Baz{\'a}n}, Juanjo and {Biswas}, Manish and {Boquien}, M{\'e}d{\'e}ric and {Burke}, D.~J. and {Cara}, Daria and {Cara}, Mihai and {Conroy}, Kyle E. and {Conseil}, Simon and {Craig}, Matthew W. and {Cross}, Robert M. and {Cruz}, Kelle L. and {D'Eugenio}, Francesco and {Dencheva}, Nadia and {Devillepoix}, Hadrien A.~R. and {Dietrich}, J{\"o}rg P. and {Eigenbrot}, Arthur Davis and {Erben}, Thomas and {Ferreira}, Leonardo and {Foreman-Mackey}, Daniel and {Fox}, Ryan and {Freij}, Nabil and {Garg}, Suyog and {Geda}, Robel and {Glattly}, Lauren and {Gondhalekar}, Yash and {Gordon}, Karl D. and {Grant}, David and {Greenfield}, Perry and {Groener}, Austen M. and {Guest}, Steve and {Gurovich}, Sebastian and {Handberg}, Rasmus and {Hart}, Akeem and {Hatfield-Dodds}, Zac and {Homeier}, Derek and {Hosseinzadeh}, Griffin and {Jenness}, Tim and {Jones}, Craig K. and {Joseph}, Prajwel and {Kalmbach}, J. Bryce and {Karamehmetoglu}, Emir and {Ka{\l}uszy{\'n}ski}, Miko{\l}aj and {Kelley}, Michael S.~P. and {Kern}, Nicholas and {Kerzendorf}, Wolfgang E. and {Koch}, Eric W. and {Kulumani}, Shankar and {Lee}, Antony and {Ly}, Chun and {Ma}, Zhiyuan and {MacBride}, Conor and {Maljaars}, Jakob M. and {Muna}, Demitri and {Murphy}, N.~A. and {Norman}, Henrik and {O'Steen}, Richard and {Oman}, Kyle A. and {Pacifici}, Camilla and {Pascual}, Sergio and {Pascual-Granado}, J. and {Patil}, Rohit R. and {Perren}, Gabriel I. and {Pickering}, Timothy E. and {Rastogi}, Tanuj and {Roulston}, Benjamin R. and {Ryan}, Daniel F. and {Rykoff}, Eli S. and {Sabater}, Jose and {Sakurikar}, Parikshit and {Salgado}, Jes{\'u}s and {Sanghi}, Aniket and {Saunders}, Nicholas and {Savchenko}, Volodymyr and {Schwardt}, Ludwig and {Seifert-Eckert}, Michael and {Shih}, Albert Y. and {Jain}, Anany Shrey and {Shukla}, Gyanendra and {Sick}, Jonathan and {Simpson}, Chris and {Singanamalla}, Sudheesh and {Singer}, Leo P. and {Singhal}, Jaladh and {Sinha}, Manodeep and {Sip{\H{o}}cz}, Brigitta M. and {Spitler}, Lee R. and {Stansby}, David and {Streicher}, Ole and {{\v{S}}umak}, Jani and {Swinbank}, John D. and {Taranu}, Dan S. and {Tewary}, Nikita and {Tremblay}, Grant R. and {de Val-Borro}, Miguel and {Van Kooten}, Samuel J. and {Vasovi{\'c}}, Zlatan and {Verma}, Shresth and {de Miranda Cardoso}, Jos{\'e} Vin{\'\i}cius and {Williams}, Peter K.~G. and {Wilson}, Tom J. and {Winkel}, Benjamin and {Wood-Vasey}, W.~M. and {Xue}, Rui and {Yoachim}, Peter and {Zhang}, Chen and {Zonca}, Andrea and {Astropy Project Contributors}},
        title = "{The Astropy Project: Sustaining and Growing a Community-oriented Open-source Project and the Latest Major Release (v5.0) of the Core Package}",
      journal = {\apj},
     keywords = {Astronomy software, Open source software, Astronomy data analysis, 1855, 1866, 1858, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2022,
        month = aug,
       volume = {935},
       number = {2},
          eid = {167},
        pages = {167},
          doi = {10.3847/1538-4357/ac7c74},
archivePrefix = {arXiv},
       eprint = {2206.14220},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...935..167A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{likelihood,
       author = {{Hamimeche}, Samira and {Lewis}, Antony},
        title = "{Likelihood analysis of CMB temperature and polarization power spectra}",
      journal = {Physical Review D},
     keywords = {98.70.Vc, Background radiations, Astrophysics},
         year = 2008,
        month = may,
       volume = {77},
       number = {10},
          eid = {103013},
        pages = {103013},
          doi = {10.1103/PhysRevD.77.103013},
archivePrefix = {arXiv},
       eprint = {0801.0554},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008PhRvD..77j3013H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Odagiri_SPIE,
       author = {{Odagiri}, Kimihide and {Saijo}, Masaru and {Shinozaki}, Keisuke and {Matsuda}, Frederick and {Oguri}, Shugo and {Suzuki}, Toyoaki and {Ogawa}, Hiroyuki and {Sekimoto}, Yutaro and {Dotani}, Tadayasu and {Watanuki}, Kazuya and {Sugimoto}, Ryo and {Yoshihara}, Keisuke and {Narasaki}, Katsuhiro and {Isshiki}, Masahito and {Yoshida}, Seiji and {Prouv{\'e}}, Thomas and {Duval}, Jean-Marc and {Thompson}, Keith L.},
        title = "{Cryogenic thermal design and analysis for LiteBIRD payload module}",
    booktitle = {Space Telescopes and Instrumentation 2022: Optical, Infrared, and Millimeter Wave},
         year = 2022,
       editor = {{Coyle}, Laura E. and {Matsuura}, Shuji and {Perrin}, Marshall D.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {12180},
        month = aug,
          eid = {121801U},
        pages = {121801U},
          doi = {10.1117/12.2629752},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022SPIE12180E..1UO},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{planck_pointing_cal,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Battaner}, E. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bobin}, J. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bowyer}, J.~W. and {Bridges}, M. and {Bucher}, M. and {Burigana}, C. and {Cardoso}, J. -F. and {Catalano}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chen}, X. and {Chiang}, H.~C. and {Chiang}, L. -Y. and {Christensen}, P.~R. and {Church}, S. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {Dickinson}, C. and {Diego}, J.~M. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Galeotta}, S. and {Ganga}, K. and {Giard}, M. and {Giardino}, G. and {Girard}, D. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D. and {Helou}, G. and {Henrot-Versill{\'e}}, S. and {Herent}, O. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hou}, Z. and {Hovest}, W. and {Huffenberger}, K.~M. and {Hurier}, G. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Laureijs}, R.~J. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Leonardi}, R. and {Leroy}, C. and {Lesgourgues}, J. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {MacTavish}, C.~J. and {Maffei}, B. and {Mandolesi}, N. and {Maris}, M. and {Marleau}, F. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Massardi}, M. and {Matarrese}, S. and {Matthai}, F. and {Mazzotta}, P. and {McGehee}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Melot}, F. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Mottet}, S. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {North}, C. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Orieux}, F. and {Osborne}, S. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Paoletti}, D. and {Pasian}, F. and {Patanchon}, G. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Popa}, L. and {Poutanen}, T. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Racine}, B. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rowan-Robinson}, M. and {Rusholme}, B. and {Sanselme}, L. and {Santos}, D. and {Sauv{\'e}}, A. and {Savini}, G. and {Scott}, D. and {Shellard}, E.~P.~S. and {Spencer}, L.~D. and {Starck}, J. -L. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sureau}, F. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Techene}, S. and {Terenzi}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wade}, L.~A. and {Wandelt}, B.~D. and {White}, S.~D.~M. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2013 results. VI. High Frequency Instrument data processing}",
      journal = {\aap},
     keywords = {methods: data analysis, cosmic background radiation, cosmology: observations, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = nov,
       volume = {571},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201321570},
archivePrefix = {arXiv},
       eprint = {1303.5067},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...571A...6P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{binning_brawn,
       author = {{Brown}, Michael L. and {Challinor}, Anthony and {North}, Chris E. and {Johnson}, Bradley R. and {O'Dea}, Daniel and {Sutton}, David},
        title = "{Impact of modulation on CMB B-mode polarization experiments}",
      journal = {\mnras},
     keywords = {methods: analytical, methods: statistical, cosmic microwave background, cosmology: theory, Astrophysics},
         year = 2009,
        month = aug,
       volume = {397},
       number = {2},
        pages = {634-656},
          doi = {10.1111/j.1365-2966.2009.14975.x},
archivePrefix = {arXiv},
       eprint = {0809.4032},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.397..634B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Giorgio_hwp,
    author = {Giorgio Savini and Giampaolo Pisano and Peter A. R. Ade},
    journal = {Appl. Opt.},
    keywords = {Polarimetry; Polarization-selective devices; Ellipsometry and polarimetry; Astronomical optics; Mueller matrices; Optical constants; Optical materials; Optical modulators; Optical properties; Phase shift},
    number = {35},
    pages = {8907--8915},
    publisher = {Optica Publishing Group},
    title = {Achromatic half-wave plate for submillimeter instruments in cosmic microwave background astronomy: modeling and simulation},
    volume = {45},
    month = {Dec},
    year = {2006},
    url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-45-35-8907},
    doi = {10.1364/AO.45.008907},
    abstract = {We adopted an existing formalism and modified it to simulate, with high precision,the transmission, reflection, and absorption of multiple-plate birefringent devices as a function of frequency. To validate the model, we use it to compare the measured properties of an achromatic five-plate device with a broadband antireflection coating to expectations derived from the material optical constants and its geometric configuration. The half-wave plate presented here is observed to perform well with a phase shift variation of\&lt;2{\textdegree} from the ideal 180{\textdegree} over a bandwidth of $\Delta$v/v$\sim$1 at millimeter wavelengths. This formalism represents a powerful design tool for birefringent polarization modulators and enables its optical properties to be specified with high accuracy.},
}

@article{Lorenzo_hwp,
    author = {Moncelsi, Lorenzo and Ade, Peter A. R. and Angilè, Francesco E. and Benton, Steven J. and Devlin, Mark J. and Fissel, Laura M. and Gandilo, Natalie N. and Gundersen, Joshua O. and Matthews, Tristan G. and Netterfield, C. Barth and Novak, Giles and Nutter, David and Pascale, Enzo and Poidevin, Frédérick and Savini, Giorgio and Scott, Douglas and Soler, Juan Diego and Spencer, Locke D. and Truch, Matthew D. P. and Tucker, Gregory S. and Zhang, Jin},
    title = "{Empirical modelling of the BLASTPol achromatic half-wave plate for precision submillimetre polarimetry}",
    journal = {\mnras},
    volume = {437},
    number = {3},
    pages = {2772-2789},
    year = {2013},
    month = {11},
    abstract = "{A cryogenic achromatic half-wave plate (HWP) for submillimetre astronomical polarimetry has been designed, manufactured, tested and deployed in the Balloon-borne Large-Aperture Submillimeter Telescope for Polarimetry (BLASTPol). The design is based on the five-slab Pancharatnam recipe and it works in the wavelength range 200–600 μm, making it the broadest-band HWP built to date at (sub)millimetre wavelengths. The frequency behaviour of the HWP has been fully characterized at room and cryogenic temperatures with incoherent radiation from a polarizing Fourier transform spectrometer. We develop a novel empirical model, complementary to the physical and analytical ones available in the literature, that allows us to recover the HWP Mueller matrix and phase shift as a function of frequency and extrapolated to 4 K. We show that most of the HWP non-idealities can be modelled by quantifying one wavelength-dependent parameter, the position of the HWP equivalent axes, which is then readily implemented in a map-making algorithm. We derive this parameter for a range of spectral signatures of input astronomical sources relevant to BLASTPol, and provide a benchmark example of how our method can yield improved accuracy on measurements of the polarization angle on the sky at submillimetre wavelengths.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stt2090},
    url = {https://doi.org/10.1093/mnras/stt2090},
    eprint = {https://academic.oup.com/mnras/article-pdf/437/3/2772/18466207/stt2090.pdf},
}

@article{Essinger_hwp,
    author = {Essinger-Hileman, T. and Kusaka, A. and Appel, J. W. and Choi, S. K. and Crowley, K. and Ho, S. P. and Jarosik, N. and Page, L. A. and Parker, L. P. and Raghunathan, S. and Simon, S. M. and Staggs, S. T. and Visnjic, K.},
    title = "{Systematic effects from an ambient-temperature, continuously rotating half-wave plate}",
    journal = {Review of Scientific Instruments},
    volume = {87},
    number = {9},
    pages = {094503},
    year = {2016},
    month = {09},
    abstract = "{We present an evaluation of systematic effects associated with a continuously rotating, ambient-temperature half-wave plate (HWP) based on two seasons of data from the Atacama B-Mode Search (ABS) experiment located in the Atacama Desert of Chile. The ABS experiment is a microwave telescope sensitive at 145 GHz. Here we present our in-field evaluation of celestial (Cosmic Microwave Background (CMB) plus galactic foreground) temperature-to-polarization leakage. We decompose the leakage into scalar, dipole, and quadrupole leakage terms. We report a scalar leakage of ∼0.01\\%, consistent with model expectations and an order of magnitude smaller than other CMB experiments have been reported. No significant dipole or quadrupole terms are detected; we constrain each to be \\&lt;0.07\\% (95\\% confidence), limited by statistical uncertainty in our measurement. Dipole and quadrupole leakage at this level lead to systematic error on r ≲ 0.01 before any mitigation due to scan cross-linking or boresight rotation. The measured scalar leakage and the theoretical level of dipole and quadrupole leakage produce systematic error of r \\&lt; 0.001 for the ABS survey and focal-plane layout before any data correction such as so-called deprojection. This demonstrates that ABS achieves significant beam systematic error mitigation from its HWP and shows the promise of continuously rotating HWPs for future experiments.}",
    issn = {0034-6748},
    doi = {10.1063/1.4962023},
    url = {https://doi.org/10.1063/1.4962023},
    eprint = {https://pubs.aip.org/aip/rsi/article-pdf/doi/10.1063/1.4962023/
              15759977/094503\_1\_online.pdf},
}

@ARTICLE{takakura_hwp,
       author = {{Takakura}, Satoru and {Aguilar}, Mario and {Akiba}, Yoshiki and {Arnold}, Kam and {Baccigalupi}, Carlo and {Barron}, Darcy and {Beckman}, Shawn and {Boettger}, David and {Borrill}, Julian and {Chapman}, Scott and {Chinone}, Yuji and {Cukierman}, Ari and {Ducout}, Anne and {Elleflot}, Tucker and {Errard}, Josquin and {Fabbian}, Giulio and {Fujino}, Takuro and {Galitzki}, Nicholas and {Goeckner-Wald}, Neil and {Halverson}, Nils W. and {Hasegawa}, Masaya and {Hattori}, Kaori and {Hazumi}, Masashi and {Hill}, Charles and {Howe}, Logan and {Inoue}, Yuki and {Jaffe}, Andrew H. and {Jeong}, Oliver and {Kaneko}, Daisuke and {Katayama}, Nobuhiko and {Keating}, Brian and {Keskitalo}, Reijo and {Kisner}, Theodore and {Krachmalnicoff}, Nicoletta and {Kusaka}, Akito and {Lee}, Adrian T. and {Leon}, David and {Lowry}, Lindsay and {Matsuda}, Frederick and {Matsumura}, Tomotake and {Navaroli}, Martin and {Nishino}, Haruki and {Paar}, Hans and {Peloton}, Julien and {Poletti}, Davide and {Puglisi}, Giuseppe and {Reichardt}, Christian L. and {Ross}, Colin and {Siritanasak}, Praween and {Suzuki}, Aritoki and {Tajima}, Osamu and {Takatori}, Sayuri and {Teply}, Grant},
        title = "{Performance of a continuously rotating half-wave plate on the POLARBEAR telescope}",
      journal = {\jcap},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Physics - Instrumentation and Detectors},
         year = 2017,
        month = may,
       volume = {2017},
       number = {5},
          eid = {008},
        pages = {008},
          doi = {10.1088/1475-7516/2017/05/008},
archivePrefix = {arXiv},
       eprint = {1702.07111},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017JCAP...05..008T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%to add:

@ARTICLE{Wright1996,
       author = {{Wright}, E.~L. and {Hinshaw}, G. and {Bennett}, C.~L.},
        title = "{Producing Megapixel Cosmic Microwave Background from Differential Radiometer Data}",
      journal = {\apjl},
     keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, METHODS: DATA ANALYSIS, Astrophysics},
         year = 1996,
        month = feb,
       volume = {458},
        pages = {L53},
          doi = {10.1086/309927},
archivePrefix = {arXiv},
       eprint = {astro-ph/9510102},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...458L..53W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Janssen1996,
       author = {{Janssen}, Michael A. and {Scott}, Douglas and {White}, Martin and {Seiffert}, Michael D. and {Lawrence}, Charles R. and {Gorski}, Krzysztof M. and {Dragovan}, Mark and {Gaier}, Todd and {Ganga}, Ken and {Gulkis}, Samuel and {Lange}, Andrew E. and {Levin}, Steven M. and {Lubin}, Philip M. and {Meinhold}, Peter and {Readhead}, Anthony C.~S. and {Richards}, Paul L. and {Ruhl}, John E.},
        title = "{Direct Imaging of the CMB from Space}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = 1996,
        month = feb,
          eid = {astro-ph/9602009},
        pages = {astro-ph/9602009},
          doi = {10.48550/arXiv.astro-ph/9602009},
archivePrefix = {arXiv},
       eprint = {astro-ph/9602009},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996astro.ph..2009J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tegmark1997,
       author = {{Tegmark}, Max},
        title = "{CMB mapping experiments: A designer's guide}",
      journal = {\prd},
     keywords = {98.70.Vc, 98.80.Bp, 98.80.Es, Background radiations, Origin and formation of the Universe, Observational cosmology, Astrophysics},
         year = 1997,
        month = oct,
       volume = {56},
       number = {8},
        pages = {4514-4529},
          doi = {10.1103/PhysRevD.56.4514},
archivePrefix = {arXiv},
       eprint = {astro-ph/9705188},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvD..56.4514T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maino1999,
       author = {{Maino}, D. and {Burigana}, C. and {Maltoni}, M. and {Wandelt}, B.~D. and {G{\'o}rski}, K.~M. and {Malaspina}, M. and {Bersanelli}, M. and {Mandolesi}, N. and {Banday}, A.~J. and {Hivon}, E.},
        title = "{The Planck-LFI instrument: Analysis of the 1/f noise and implications for the scanning strategy}",
      journal = {\aaps},
     keywords = {METHODS: DATA ANALYSIS, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, SPACE VEHICLES, Astrophysics},
         year = 1999,
        month = dec,
       volume = {140},
        pages = {383-391},
          doi = {10.1051/aas:1999429},
archivePrefix = {arXiv},
       eprint = {astro-ph/9906010},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&AS..140..383M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hu2003,
       author = {{Hu}, Wayne and {Hedman}, Matthew M. and {Zaldarriaga}, Matias},
        title = "{Benchmark parameters for CMB polarization experiments}",
      journal = {\prd},
     keywords = {98.70.Vc, Background radiations, Astrophysics},
         year = 2003,
        month = feb,
       volume = {67},
       number = {4},
          eid = {043004},
        pages = {043004},
          doi = {10.1103/PhysRevD.67.043004},
archivePrefix = {arXiv},
       eprint = {astro-ph/0210096},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003PhRvD..67d3004H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{imada2018instrumentally,
  title={Instrumentally induced spurious polarization of a multi-layer half wave plate for a CMB polarization observation},
  author={Imada, Hiroaki and Matsumura, Tomotake and Takaku, Ryota and Patanchon, Guillaume and Ishino, Hirokazu and Sakurai, Yuki and Komatsu, Kunimoto and Katayama, Nobuhiko},
  booktitle={Proc. Twenty-Ninth Int. Symp. Space Terahertz Technol},
  year={2018}
}

@article{takase2024scan,
doi = {10.1088/1475-7516/2024/12/036},
url = {https://dx.doi.org/10.1088/1475-7516/2024/12/036},
year = {2024},
month = {dec},
publisher = {IOP Publishing},
volume = {2024},
number = {12},
pages = {036},
author = {Y. Takase and L. Vacher and H. Ishino and G. Patanchon and L. Montier and S.L. Stever and K. Ishizaka and Y. Nagano and W. Wang and J. Aumont and K. Aizawa and A. Anand and C. Baccigalupi and M. Ballardini and A.J. Banday and R.B. Barreiro and N. Bartolo and S. Basak and M. Bersanelli and M. Bortolami and T. Brinckmann and E. Calabrese and P. Campeti and E. Carinos and A. Carones and F.J. Casas and K. Cheung and L. Clermont and F. Columbro and A. Coppolecchia and F. Cuttaia and G. D'Alessandro and P. de Bernardis and T. de Haan and E. de la Hoz and S. Della Torre and P. Diego-Palazuelos and H.K. Eriksen and J. Errard and F. Finelli and U. Fuskeland and G. Galloni and M. Galloway and M. Gervasi and T. Ghigna and S. Giardiello and C. Gimeno-Amo and E. Gjerløw and R. González González and A. Gruppuso and M. Hazumi and S. Henrot-Versillé and L.T. Hergt and K. Ikuma and K. Kohri and L. Lamagna and M. Lattanzi and C. Leloup and M. Lembo and F. Levrier and A.I. Lonappan and M. López-Caniego and G. Luzzi and B. Maffei and E. Martínez-González and S. Masi and S. Matarrese and F.T. Matsuda and T. Matsumura and S. Micheli and M. Migliaccio and M. Monelli and G. Morgante and B. Mot and R. Nagata and T. Namikawa and A. Novelli and K. Odagiri and S. Oguri and R. Omae and L. Pagano and D. Paoletti and F. Piacentini and M. Pinchera and G. Polenta and L. Porcelli and N. Raffuzzi and M. Remazeilles and A. Ritacco and M. Ruiz-Granda and Y. Sakurai and D. Scott and Y. Sekimoto and M. Shiraishi and G. Signorelli and R.M. Sullivan and H. Takakura and L. Terenzi and M. Tomasi and M. Tristram and B. van Tent and P. Vielva and I.K. Wehus and B. Westbrook and G. Weymann-Despres and E.J. Wollack and M. Zannoni and Y. Zhou and The LiteBIRD collaboration},
title = {Multi-dimensional optimisation of the scanning strategy for the LiteBIRD space mission},
journal = {Journal of Cosmology and Astroparticle Physics},
abstract = {Large angular scale surveys in the absence of atmosphere are essential for measuring the primordial B-mode power spectrum of the Cosmic Microwave Background (CMB). Since this proposed measurement is about three to four orders of magnitude fainter than the temperature anisotropies of the CMB, in-flight calibration of the instruments and active suppression of systematic effects are crucial. We investigate the effect of changing the parameters of the scanning strategy on the in-flight calibration effectiveness, the suppression of the systematic effects themselves, and the ability to distinguish systematic effects by null-tests. Next-generation missions such as LiteBIRD, modulated by a Half-Wave Plate (HWP), will be able to observe polarisation using a single detector, eliminating the need to combine several detectors to measure polarisation, as done in many previous experiments and hence avoiding the consequent systematic effects. While the HWP is expected to suppress many systematic effects, some of them will remain. We use an analytical approach to comprehensively address the mitigation of these systematic effects and identify the characteristics of scanning strategies that are the most effective for implementing a variety of calibration strategies in the multi-dimensional space of common spacecraft scan parameters. We verify that LiteBIRD's standard configuration yields good performance on the metrics we studied. We also present Falcons.jl, a fast spacecraft scanning simulator that we developed to investigate this scanning parameter space.}
}


@ARTICLE{dipole_SRoll,
       author = {{Delouis}, J. -M. and {Puget}, J. -L. and {Vibert}, L.},
        title = "{Improved large-scale interstellar dust foreground model and CMB solar dipole measurement}",
      journal = {\aap},
     keywords = {surveys, cosmic background radiation, diffuse radiation, methods: data analysis, dust, extinction, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jun,
       volume = {650},
          eid = {A82},
        pages = {A82},
          doi = {10.1051/0004-6361/202140616},
archivePrefix = {arXiv},
       eprint = {2102.10004},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...650A..82D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{noise_2000,
       author = {{Ferreira}, P.~G. and {Jaffe}, A.~H.},
        title = "{Simultaneous estimation of noise and signal in cosmic microwave background experiments}",
      journal = {\mnras},
     keywords = {COSMIC MICROWAVE BACKGROUND, Astrophysics},
         year = 2000,
        month = feb,
       volume = {312},
       number = {1},
        pages = {89-102},
          doi = {10.1046/j.1365-8711.2000.03108.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/9909250},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000MNRAS.312...89F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%---------------- For the introduction ---------------------------------

@book{komatsu2019cmb,
  author    = {Komatsu, Eiichiro},
  title     = {Cosmic Microwave Background Radiation},
  series    = {New astronomy library},
  volume    = {6},
  edition   = {First},
  publisher = {NIPPON HYORON SHA CO.,LTD., Japan},
  year      = {2019},
  ISBN      = {978-4-535-60745-3}
}

@article{aghanim2020planck_cosmo,
  title={Planck 2018 results-VI. Cosmological parameters},
  author={Aghanim, Nabila and Akrami, Yashar and Ashdown, Mark and Aumont, J and Baccigalupi, C and Ballardini, M and Banday, AJ and Barreiro, RB and Bartolo, N and Basak, S and others},
  journal={Astronomy \& Astrophysics},
  volume={641},
  pages={A6},
  year={2020},
  publisher={EDP sciences}
}

@ARTICLE{penzias1965measurement,
       author = {{Penzias}, A.~A. and {Wilson}, R.~W.},
        title = "{A Measurement of Excess Antenna Temperature at 4080 Mc/s.}",
      journal = {\apj},
     keywords = {Microwave Background, Cosmic Background Radiation},
         year = 1965,
        month = jul,
       volume = {142},
        pages = {419-421},
          doi = {10.1086/148307},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1965ApJ...142..419P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dicke1965cosmic,
       author = {{Dicke}, R.~H. and {Peebles}, P.~J.~E. and {Roll}, P.~G. and {Wilkinson}, D.~T.},
        title = "{Cosmic Black-Body Radiation.}",
      journal = {\apj},
     keywords = {Big Bang},
         year = 1965,
        month = jul,
       volume = {142},
        pages = {414-419},
          doi = {10.1086/148306},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1965ApJ...142..414D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mather1990preliminary,
  title={A preliminary measurement of the cosmic microwave background spectrum by the Cosmic Background Explorer (COBE) satellite},
  author={Mather, John C and Cheng, ES and Eplee Jr, RE and Isaacman, RB and Meyer, SS and Shafer, RA and Weiss, R and Wright, EL and Bennett, CL and Boggess, NW and others},
  journal={The Astrophysical Journal},
  volume={354},
  pages={L37--L40},
  year={1990},
  doi={10.1086/185717},
  url={https://articles.adsabs.harvard.edu/pdf/1990ApJ...354L..37M}
}


@article{conklin1969velocity,
  title={Velocity of the Earth with respect to the Cosmic Background Radiation},
  author={Conklin, EK},
  journal={Nature},
  volume={222},
  number={5197},
  pages={971--972},
  year={1969},
  publisher={Nature Publishing Group}
}

@article{bennett1996four,
  title={Four-year COBE* DMR cosmic microwave background observations: maps and basic results},
  author={Bennett, Charles L and Banday, Anthony J and G{\'o}rski, Krzysztof M and Hinshaw, G and Jackson, P and Keegstra, P and Kogut, A and Smoot, George F and Wilkinson, David T and Wright, Edward L},
  journal={The Astrophysical Journal Letters},
  volume={464},
  number={1},
  pages={L1},
  year={1996},
  publisher={IOP Publishing}
}

@article{aghanim2020planck_overview,
  title={Planck 2018 results-I. Overview and the cosmological legacy of Planck},
  author={Aghanim, Nabila and Akrami, Yashar and Arroja, Frederico and Ashdown, Mark and Aumont, J and Baccigalupi, Carlo and Ballardini, M and Banday, Anthony J and Barreiro, RB and Bartolo, Nicola and others},
  journal={Astronomy \& Astrophysics},
  volume={641},
  pages={A1},
  year={2020},
  publisher={EDP sciences}
}

@article{Durrer_2015,
	doi = {10.1088/0264-9381/32/12/124007},
	url = {https://doi.org/10.1088/0264-9381/32/12/124007},
	year = 2015,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {32},
	number = {12},
	pages = {124007},
	author = {Ruth Durrer},
	title = {The cosmic microwave background: the history of its experimental investigation and its significance for cosmology},
	journal = {Classical and Quantum Gravity},
	abstract = {This review describes the discovery of the cosmic microwave background (CMB) radiation in 1965 and its impact on cosmology in the 50 years that followed. This discovery established the big bang model of the Universe, and the analysis of its fluctuations has confirmed the idea of inflation and led to the present era of precision cosmology. I discuss the evolution of cosmological perturbations and their imprint on the CMB as temperature fluctuations and polarization. I also show how a phase of inflationary expansion generates fluctuations in the spacetime curvature and primordial gravitational waves. In addition I present the findings of CMB experiments, from the earliest to the most recent ones. The accuracy of these experiments has helped us to estimate the parameters of the cosmological model with unprecedented precision, so that in the future we shall be able to test not only cosmological models but general relativity itself on cosmological scales.}
}

@article{andersen2020beyondplanck,
  title={BeyondPlanck I. Global Bayesian analysis of the Planck Low Frequency Instrument data},
  author={Andersen, KJ and Aurlien, R and Banerji, R and Bersanelli, M and Bertocco, S and Brilenkov, M and Carbone, M and Colombo, LPL and Eriksen, HK and Eskilt, JR and others},
  journal={arXiv preprint arXiv:2011.05609},
  year={2020}
}

@article{tegmark2003high,
  title={High resolution foreground cleaned CMB map from WMAP},
  author={Tegmark, Max and de Oliveira-Costa, Angelica and Hamilton, Andrew JS},
  journal={Physical Review D},
  volume={68},
  number={12},
  pages={123523},
  year={2003},
  publisher={APS}
}

@article{peiris2003first,
  title={First-year Wilkinson microwave anisotropy probe (WMAP)* observations: implications for inflation},
  author={Peiris, Hiranya V and Komatsu, E and Verde, L and Spergel, DN and Bennett, CL and Halpern, M and Hinshaw, G and Jarosik, N and Kogut, A and Limon, M and others},
  journal={The Astrophysical Journal Supplement Series},
  volume={148},
  number={1},
  pages={213},
  year={2003},
  publisher={IOP Publishing}
}


@article{gorski1999healpix,
  title={The healpix primer},
  author={Gorski, Krzysztof M and Wandelt, Benjamin D and Hansen, Frode K and Hivon, Eric and Banday, Anthony J},
  journal={arXiv preprint astro-ph/9905275},
  year={1999}
}


@inproceedings{hazumi2020litebird,
  title={LiteBIRD satellite: JAXA's new strategic L-class mission for all-sky surveys of cosmic microwave background polarization},
  author={Hazumi, Masashi and Ade, Peter AR and Adler, Alexandre and Allys, Erwan and Alonso, David and Arnold, Kam and Auguste, Didier and Aumont, Jonathan and Aurlien, Ragnhild and Austermann, Jason and others},
  booktitle={Space Telescopes and Instrumentation 2020: Optical, Infrared, and Millimeter Wave},
  volume={11443},
  pages={114432F},
  year={2020},
  organization={International Society for Optics and Photonics}
}

@article{tomasi2021healpix,
  title={Healpix. jl: Julia-only port of the HEALPix library},
  author={Tomasi, Maurizio and Li, Zack},
  journal={Astrophysics Source Code Library},
  pages={ascl--2109},
  year={2021}
}

@article{mccallum2021spin,
  title={Spin characterization of systematics in CMB surveys--a comprehensive formalism},
  author={McCallum, Nialh and Thomas, Daniel B and Brown, Michael L and Tessore, Nicolas},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={501},
  number={1},
  pages={802--832},
  year={2021},
  publisher={Oxford University Press}
}

@article{hoang2017bandpass,
  title={Bandpass mismatch error for satellite cmb experiments i: estimating the spurious signal},
  author={Hoang, Duc Thuong and Patanchon, Guillaume and Bucher, Martin and Matsumura, Tomotake and Banerji, Ranajoy and Ishino, Hirokazu and Hazumi, Masashi and Delabrouille, Jacques},
  journal={Journal of Cosmology and Astroparticle Physics},
  volume={2017},
  number={12},
  pages={015},
  year={2017},
  publisher={IOP Publishing}
}

@article{ade2016bicep2,
  title={BICEP2/Keck Array VIII: Measurement of gravitational lensing from large-scale B-mode polarization},
  author={Ade, PAR and Ahmed, Z and Aikin, RW and Alexander, Kate Denham and Barkats, D and Benton, SJ and Bischoff, Colin A and Bock, JJ and Bowens-Rubin, R and Brevik, JA and others},
  journal={The Astrophysical Journal},
  volume={833},
  number={2},
  pages={228},
  year={2016},
  publisher={IOP Publishing}
}

@article{akrami2020planck,
  title={Planck 2018 results-IV. Diffuse component separation},
  author={Akrami, Yashar and Ashdown, M and Aumont, Jonathan and Baccigalupi, Carlo and Ballardini, M and Banday, Anthony J and Barreiro, RB and Bartolo, Nicola and Basak, S and Benabed, K and others},
  journal={Astronomy \& Astrophysics},
  volume={641},
  pages={A4},
  year={2020},
  publisher={EDP sciences}
}

@article{PhysRevD.77.103013,
  title = {Likelihood analysis of CMB temperature and polarization power spectra},
  author = {Hamimeche, Samira and Lewis, Antony},
  journal = {Phys. Rev. D},
  volume = {77},
  issue = {10},
  pages = {103013},
  numpages = {28},
  year = {2008},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.77.103013},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.77.103013}
}

@article{PhysRevLett.112.241101,
  title = {Detection of $B$-Mode Polarization at Degree Angular Scales by BICEP2},
  author = {Ade, P. A. R. and Aikin, R. W. and Barkats, D. and Benton, S. J. and Bischoff, C. A. and Bock, J. J. and Brevik, J. A. and Buder, I. and Bullock, E. and Dowell, C. D. and Duband, L. and Filippini, J. P. and Fliescher, S. and Golwala, S. R. and Halpern, M. and Hasselfield, M. and Hildebrandt, S. R. and Hilton, G. C. and Hristov, V. V. and Irwin, K. D. and Karkare, K. S. and Kaufman, J. P. and Keating, B. G. and Kernasovskiy, S. A. and Kovac, J. M. and Kuo, C. L. and Leitch, E. M. and Lueker, M. and Mason, P. and Netterfield, C. B. and Nguyen, H. T. and O'Brient, R. and Ogburn, R. W. and Orlando, A. and Pryke, C. and Reintsema, C. D. and Richter, S. and Schwarz, R. and Sheehy, C. D. and Staniszewski, Z. K. and Sudiwala, R. V. and Teply, G. P. and Tolan, J. E. and Turner, A. D. and Vieregg, A. G. and Wong, C. L. and Yoon, K. W.},
  collaboration = {BICEP2 Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {24},
  pages = {241101},
  numpages = {25},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.241101},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.241101}
}

@article{lyth1999particle,
  title={Particle physics models of inflation and the cosmological density perturbation},
  author={Lyth, David H and Riotto, Antonio},
  journal={Physics Reports},
  volume={314},
  number={1-2},
  pages={1--146},
  year={1999},
  publisher={Elsevier}
}

@article{guzzetti2016gravitational,
    author = "Guzzetti, M. C. and Bartolo, N. and Liguori, M. and Matarrese, S.",
    title = "{Gravitational waves from inflation}",
    eprint = "1605.01615",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1393/ncr/i2016-10127-1",
    journal = "Riv. Nuovo Cim.",
    volume = "39",
    number = "9",
    pages = "399--495",
    year = "2016"
}


@article{silk1968cosmic,
  title={Cosmic black-body radiation and galaxy formation},
  author={Silk, Joseph},
  journal={The Astrophysical Journal},
  volume={151},
  pages={459},
  year={1968}
}

@inproceedings{sekimoto2020concept,
       author = {{Sekimoto}, Y. and {Ade}, P.~A.~R. and {Adler}, A. and {Allys}, E. and {Arnold}, K. and {Auguste}, D. and {Aumont}, J. and {Aurlien}, R. and {Austermann}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Banerji}, R. and {Barreiro}, R.~B. and {Basak}, S. and {Beall}, J. and {Beck}, D. and {Beckman}, S. and {Bermejo}, J. and {de Bernardis}, P. and {Bersanelli}, M. and {Bonis}, J. and {Borrill}, J. and {Boulanger}, F. and {Bounissou}, S. and {Brilenkov}, M. and {Brown}, M. and {Bucher}, M. and {Calabrese}, E. and {Campeti}, P. and {Carones}, A. and {Casas}, F.~J. and {Challinor}, A. and {Chan}, V. and {Cheung}, K. and {Chinone}, Y. and {Cliche}, J.~F. and {Colombo}, L. and {Columbro}, F. and {Cubas}, J. and {Cukierman}, A. and {Curtis}, D. and {D'Alessandro}, G. and {Dachlythra}, N. and {De Petris}, M. and {Dickinson}, C. and {Diego-Palazuelos}, P. and {Dobbs}, M. and {Dotani}, T. and {Duband}, L. and {Duff}, S. and {Duval}, J.~M. and {Ebisawa}, K. and {Elleflot}, T. and {Eriksen}, H.~K. and {Errard}, J. and {Essinger-Hileman}, T. and {Finelli}, F. and {Flauger}, R. and {Franceschet}, C. and {Fuskeland}, U. and {Galloway}, M. and {Ganga}, K. and {Gao}, J.~R. and {Genova-Santos}, R. and {Gerbino}, M. and {Gervasi}, M. and {Ghigna}, T. and {Gjerl{\o}w}, E. and {Gradziel}, M.~L. and {Grain}, J. and {Grupp}, F. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {de Haan}, T. and {Halverson}, N.~W. and {Hargrave}, P. and {Hasebe}, T. and {Hasegawa}, M. and {Hattori}, M. and {Hazumi}, M. and {Henrot-Versill{\'e}}, S. and {Herman}, D. and {Herranz}, D. and {Hill}, C.~A. and {Hilton}, G. and {Hirota}, Y. and {Hivon}, E. and {Hlozek}, R.~A. and {Hoshino}, Y. and {de la Hoz}, E. and {Hubmayr}, J. and {Ichiki}, K. and {iida}, T. and {Imada}, H. and {Ishimura}, K. and {Ishino}, H. and {Jaehnig}, G. and {Kaga}, T. and {Kashima}, S. and {Katayama}, N. and {Kato}, A. and {Kawasaki}, T. and {Keskitalo}, R. and {Kisner}, T. and {Kobayashi}, Y. and {Kogiso}, N. and {Kogut}, A. and {Kohri}, K. and {Komatsu}, E. and {Komatsu}, K. and {Konishi}, K. and {Krachmalnicoff}, N. and {Kreykenbohm}, I. and {Kuo}, C.~L. and {Kushino}, A. and {Lamagna}, L. and {Lanen}, J.~V. and {Lattanzi}, M. and {Lee}, A.~T. and {Leloup}, C. and {Levrier}, F. and {Linder}, E. and {Louis}, T. and {Luzzi}, G. and {Maciaszek}, T. and {Maffei}, B. and {Maino}, D. and {Maki}, M. and {Mandelli}, S. and {Martinez-Gonzalez}, E. and {Masi}, S. and {Matsumura}, T. and {Mennella}, A. and {Migliaccio}, M. and {Minanmi}, Y. and {Mitsuda}, K. and {Montgomery}, J. and {Montier}, L. and {Morgante}, G. and {Mot}, B. and {Murata}, Y. and {Murphy}, J.~A. and {Nagai}, M. and {Nagano}, Y. and {Nagasaki}, T. and {Nagata}, R. and {Nakamura}, S. and {Namikawa}, T. and {Natoli}, P. and {Nerval}, S. and {Nishibori}, T. and {Nishino}, H. and {O'Sullivan}, C. and {Ogawa}, H. and {Ogawa}, H. and {Oguri}, S. and {Ohsaki}, H. and {Ohta}, I.~S. and {Okada}, N. and {Okada}, N. and {Pagano}, L. and {Paiella}, A. and {Paoletti}, D. and {Patanchon}, G. and {Peloton}, J. and {Piacentini}, F. and {Pisano}, G. and {Polenta}, G. and {Poletti}, D. and {Prouv{\'e}}, T. and {Puglisi}, G. and {Rambaud}, D. and {Raum}, C. and {Realini}, S. and {Reinecke}, M. and {Remazeilles}, M. and {Ritacco}, A. and {Roudil}, G. and {Rubino-Martin}, J.~A. and {Russell}, M. and {Sakurai}, H. and {Sakurai}, Y. and {Sandri}, M. and {Sasaki}, M. and {Savini}, G. and {Scott}, D. and {Seibert}, J. and {Sherwin}, B. and {Shinozaki}, K. and {Shiraishi}, M. and {Shirron}, P. and {Signorelli}, G. and {Smecher}, G. and {Stever}, S. and {Stompor}, R. and {Sugai}, H. and {Sugiyama}, S. and {Suzuki}, A. and {Suzuki}, J. and {Svalheim}, T.~L. and {Switzer}, E. and {Takaku}, R. and {Takakura}, H. and {Takakura}, S. and {Takase}, Y. and {Takeda}, Y. and {Tartari}, A. and {Taylor}, E. and {Terao}, Y. and {Thommesen}, H. and {Thompson}, K.~L. and {Thorne}, B. and {Toda}, T. and {Tomasi}, M. and {Tominaga}, M. and {Trappe}, N. and {Tristram}, M. and {Tsuji}, M. and {Tsujimoto}, M. and {Tucker}, C. and {Ullom}, J. and {Vermeulen}, G. and {Vielva}, P. and {Villa}, F. and {Vissers}, M. and {Vittorio}, N. and {Wehus}, I. and {Weller}, J. and {Westbrook}, B. and {Wilms}, J. and {Winter}, B. and {Wollack}, E.~J. and {Yamasaki}, N.~Y. and {Yoshida}, T. and {Yumoto}, J. and {Zannoni}, M. and {Zonca}, A.},
        title = "{Concept design of low frequency telescope for CMB B-mode polarization satellite LiteBIRD}",
    booktitle = {Millimeter, Submillimeter, and Far-Infrared Detectors and Instrumentation for Astronomy X},
         year = 2020,
       editor = {{Zmuidzinas}, Jonas and {Gao}, Jian-Rong},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {11453},
        month = dec,
          eid = {1145310},
        pages = {1145310},
          doi = {10.1117/12.2561841},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SPIE11453E..10S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@inproceedings{galitzki2018simons,
  title={The Simons observatory: instrument overview},
  author={Galitzki, Nicholas and Ali, Aamir and Arnold, Kam S and Ashton, Peter C and Austermann, Jason E and Baccigalupi, Carlo and Baildon, Taylor and Barron, Darcy and Beall, James A and Beckman, Shawn and others},
  booktitle={Millimeter, Submillimeter, and Far-Infrared Detectors and Instrumentation for Astronomy IX},
  volume={10708},
  pages={1070804},
  year={2018},
  organization={International Society for Optics and Photonics}
}

@article{bock2008experimental,
  title={The Experimental Probe of Inflationary Cosmology (EPIC): a mission concept study for NASA's Einstein inflation probe},
  author={Bock, James and Cooray, Asantha and Hanany, Shaul and Keating, Brian and Lee, Adrian and Matsumura, Tomotake and Milligan, Michael and Ponthieu, Nicolas and Renbarger, Tom and Tran, Huan},
  journal={arXiv preprint arXiv:0805.4207},
  year={2008}
}

@article{CORE2018,
   title={Exploring cosmic origins with CORE: Survey requirements and mission design},
   volume={2018},
   ISSN={1475-7516},
   url={http://dx.doi.org/10.1088/1475-7516/2018/04/014},
   DOI={10.1088/1475-7516/2018/04/014},
   number={04},
   journal={Journal of Cosmology and Astroparticle Physics},
   publisher={IOP Publishing},
   author={Delabrouille, J. and de Bernardis, P. and Bouchet, F.R. and Achúcarro, A. and Ade, P. A. R. and Allison, R. and Arroja, F. and Artal, E. and Ashdown, M. and Baccigalupi, C. and Ballardini, M. and Banday, A.J. and Banerji, R. and et al.},
   year={2018},
   month={Apr},
   pages={014–014} }

@INPROCEEDINGS{sakurai2020breadboard,
       author = {{Sakurai}, Yuki and {Matsumura}, Tomotake and {Katayama}, Nobuhiko and {Komatsu}, Kunimoto and {Takaku}, Ryota and {Sugiyama}, Shinya and {Nomura}, Yoshiki and {Toda}, Takayuki and {Ghigna}, Tommaso and {Iida}, Teruhito and {Sugai}, Hajime and {Imada}, Hiroaki and {Hazumi}, Masashi and {Ishino}, Hirokazu and {Ohsaki}, Hiroyuki and {Terao}, Yutaka and {Enokida}, Hisashi and {Ishida}, Yusuke and {Iwata}, Yosuke and {Ahmad}, Doa and {Konishi}, Kuniaki and {Sakurai}, Haruyuki and {Yumoto}, Junji and {Kuwata-Gonokami}, Makoto and {Kusaka}, Akito and {Hill}, Charles},
        title = "{Breadboard model of the polarization modulator unit based on a continuously rotating half-wave plate for the low-frequency telescope of the LiteBIRD space mission}",
    booktitle = {Millimeter, Submillimeter, and Far-Infrared Detectors and Instrumentation for Astronomy X},
         year = 2020,
       editor = {{Zmuidzinas}, Jonas and {Gao}, Jian-Rong},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {11453},
        month = dec,
          eid = {114534E},
        pages = {114534E},
          doi = {10.1117/12.2560289},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SPIE11453E..4ES},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{columbro2020polarization,
       author = {{Columbro}, Fabio and {de Bernardis}, Paolo and {Lamagna}, Luca and {Masi}, Silvia and {Paiella}, Alessandro and {Piacentini}, Francesco and {Pisano}, Giampaolo},
        title = "{A polarization modulator unit for the mid- and high-frequency telescopes of the LiteBIRD mission}",
    booktitle = {Space Telescopes and Instrumentation 2020: Optical, Infrared, and Millimeter Wave},
         year = 2020,
       editor = {{Lystrup}, Makenzie and {Perrin}, Marshall D.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {11443},
        month = dec,
          eid = {114436Z},
        pages = {114436Z},
          doi = {10.1117/12.2577818},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SPIE11443E..6ZC},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Duivenvoorden2019fullskybeamconv,
   title={Full-sky beam convolution for cosmic microwave background applications},
   volume={486},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stz1143},
   DOI={10.1093/mnras/stz1143},
   number={4},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Duivenvoorden, Adriaan J and Gudmundsson, Jon E and Rahlin, Alexandra S},
   year={2019},
   month={May},
   pages={5448–5467} }

@article{kamionkowski2016quest,
  title={The quest for B modes from inflationary gravitational waves},
  author={Kamionkowski, Marc and Kovetz, Ely D},
  journal={Annual Review of Astronomy and Astrophysics},
  volume={54},
  pages={227--269},
  year={2016},
  publisher={Annual Reviews}
}

@article{planck2018result_inflation,
	author = {{Planck Collaboration} and {Akrami, Y.} and {Arroja, F.} and {Ashdown, M.} and {Aumont, J.} and {Baccigalupi, C.} and {Ballardini, M.} and {Banday, A. J.} and {Barreiro, R. B.} and {Bartolo, N.} and {Basak, S.} and {Benabed, K.} and {Bernard, J.-P.} and {Bersanelli, M.} and {Bielewicz, P.} and {Bock, J. J.} and {Bond, J. R.} and {Borrill, J.} and {Bouchet, F. R.} and {Boulanger, F.} and {Bucher, M.} and {Burigana, C.} and {Butler, R. C.} and {Calabrese, E.} and {Cardoso, J.-F.} and {Carron, J.} and {Challinor, A.} and {Chiang, H. C.} and {Colombo, L. P. L.} and {Combet, C.} and {Contreras, D.} and {Crill, B. P.} and {Cuttaia, F.} and {de Bernardis, P.} and {de Zotti, G.} and {Delabrouille, J.} and {Delouis, J.-M.} and {Di Valentino, E.} and {Diego, J. M.} and {Donzelli, S.} and {Dor\'e, O.} and {Douspis, M.} and {Ducout, A.} and {Dupac, X.} and {Dusini, S.} and {Efstathiou, G.} and {Elsner, F.} and {En\ss{}lin, T. A.} and {Eriksen, H. K.} and {Fantaye, Y.} and {Fergusson, J.} and {Fernandez-Cobos, R.} and {Finelli, F.} and {Forastieri, F.} and {Frailis, M.} and {Franceschi, E.} and {Frolov, A.} and {Galeotta, S.} and {Galli, S.} and {Ganga, K.} and {Gauthier, C.} and {G\'enova-Santos, R. T.} and {Gerbino, M.} and {Ghosh, T.} and {Gonz\'alez-Nuevo, J.} and {G\'orski, K. M.} and {Gratton, S.} and {Gruppuso, A.} and {Gudmundsson, J. E.} and {Hamann, J.} and {Handley, W.} and {Hansen, F. K.} and {Herranz, D.} and {Hivon, E.} and {Hooper, D. C.} and {Huang, Z.} and {Jaffe, A. H.} and {Jones, W. C.} and {Keih\"anen, E.} and {Keskitalo, R.} and {Kiiveri, K.} and {Kim, J.} and {Kisner, T. S.} and {Krachmalnicoff, N.} and {Kunz, M.} and {Kurki-Suonio, H.} and {Lagache, G.} and {Lamarre, J.-M.} and {Lasenby, A.} and {Lattanzi, M.} and {Lawrence, C. R.} and {Le Jeune, M.} and {Lesgourgues, J.} and {Levrier, F.} and {Lewis, A.} and {Liguori, M.} and {Lilje, P. B.} and {Lindholm, V.} and {L\'opez-Caniego, M.} and {Lubin, P. M.} and {Ma, Y.-Z.} and {Mac\'{\i}as-P\'erez, J. F.} and {Maggio, G.} and {Maino, D.} and {Mandolesi, N.} and {Mangilli, A.} and {Marcos-Caballero, A.} and {Maris, M.} and {Martin, P. G.} and {Mart\'{\i}nez-Gonz\'alez, E.} and {Matarrese, S.} and {Mauri, N.} and {McEwen, J. D.} and {Meerburg, P. D.} and {Meinhold, P. R.} and {Melchiorri, A.} and {Mennella, A.} and {Migliaccio, M.} and {Mitra, S.} and {Miville-Desch\^enes, M.-A.} and {Molinari, D.} and {Moneti, A.} and {Montier, L.} and {Morgante, G.} and {Moss, A.} and {M\"unchmeyer, M.} and {Natoli, P.} and {N\o{}rgaard-Nielsen, H. U.} and {Pagano, L.} and {Paoletti, D.} and {Partridge, B.} and {Patanchon, G.} and {Peiris, H. V.} and {Perrotta, F.} and {Pettorino, V.} and {Piacentini, F.} and {Polastri, L.} and {Polenta, G.} and {Puget, J.-L.} and {Rachen, J. P.} and {Reinecke, M.} and {Remazeilles, M.} and {Renzi, A.} and {Rocha, G.} and {Rosset, C.} and {Roudier, G.} and {Rubi\~no-Mart\'{\i}n, J. A.} and {Ruiz-Granados, B.} and {Salvati, L.} and {Sandri, M.} and {Savelainen, M.} and {Scott, D.} and {Shellard, E. P. S.} and {Shiraishi, M.} and {Sirignano, C.} and {Sirri, G.} and {Spencer, L. D.} and {Sunyaev, R.} and {Suur-Uski, A.-S.} and {Tauber, J. A.} and {Tavagnacco, D.} and {Tenti, M.} and {Toffolatti, L.} and {Tomasi, M.} and {Trombetti, T.} and {Valiviita, J.} and {Van Tent, B.} and {Vielva, P.} and {Villa, F.} and {Vittorio, N.} and {Wandelt, B. D.} and {Wehus, I. K.} and {White, S. D. M.} and {Zacchei, A.} and {Zibin, J. P.} and {Zonca, A.}},
	title = {Planck 2018 results - X. Constraints on inflation},
	DOI= "10.1051/0004-6361/201833887",
	url= "https://doi.org/10.1051/0004-6361/201833887",
	journal = {A\&A},
	year = 2020,
	volume = 641,
	pages = "A10",
}

@article{optimalscan2016wallis,
    author = {Wallis, Christopher G. R. and Brown, Michael L. and Battye, Richard A. and Delabrouille, Jacques},
    title = "{Optimal scan strategies for future CMB satellite experiments}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {466},
    number = {1},
    pages = {425-442},
    year = {2016},
    month = {10},
    abstract = "{The B-mode polarization power spectrum in the cosmic microwave background (CMB) is about four orders of magnitude fainter than the CMB temperature power spectrum. Any instrumental imperfections that couple temperature fluctuations to B-mode polarization must therefore be carefully controlled and/or removed. We investigate the role that a scan strategy can have in mitigating certain common systematics by averaging systematic errors down with many crossing angles. We present approximate analytic forms for the error on the recovered B-mode power spectrum that would result from differential gain, differential pointing and differential ellipticity for the case where two detector pairs are used in a polarization experiment. We use these analytic predictions to search the parameter space of common satellite scan strategies in order to identify those features of a scan strategy that have most impact in mitigating systematic effects. As an example, we go on to identify a scan strategy suitable for the CMB satellite proposed for the European Space Agency M5 call, considering the practical considerations of fuel requirement, data rate and the relative orientation of the telescope to the earth. Having chosen a scan strategy we then go on to investigate the suitability of the scan strategy.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stw2577},
    url = {https://doi.org/10.1093/mnras/stw2577},
    eprint = {https://academic.oup.com/mnras/article-pdf/466/1/425/10864929/stw2577.pdf},
}

@misc{litebirdcollaboration2022probing,
      title={Probing Cosmic Inflation with the LiteBIRD Cosmic Microwave Background Polarization Survey},
      author={LiteBIRD Collaboration and E. Allys and K. Arnold and J. Aumont and R. Aurlien and S. Azzoni and C. Baccigalupi and A. J. Banday and R. Banerji and R. B. Barreiro and N. Bartolo and L. Bautista and D. Beck and S. Beckman and M. Bersanelli and F. Boulanger and M. Brilenkov and M. Bucher and E. Calabrese and P. Campeti and A. Carones and F. J. Casas and A. Catalano and V. Chan and K. Cheung and Y. Chinone and S. E. Clark and F. Columbro and G. D'Alessandro and P. de Bernardis and T. de Haan and E. de la Hoz and M. De Petris and S. Della Torre and P. Diego-Palazuelos and T. Dotani and J. M. Duval and T. Elleflot and H. K. Eriksen and J. Errard and T. Essinger-Hileman and F. Finelli and R. Flauger and C. Franceschet and U. Fuskeland and M. Galloway and K. Ganga and M. Gerbino and M. Gervasi and R. T. Génova-Santos and T. Ghigna and S. Giardiello and E. Gjerløw and J. Grain and F. Grupp and A. Gruppuso and J. E. Gudmundsson and N. W. Halverson and P. Hargrave and T. Hasebe and M. Hasegawa and M. Hazumi and S. Henrot-Versillé and B. Hensley and L. T. Hergt and D. Herman and E. Hivon and R. A. Hlozek and A. L. Hornsby and Y. Hoshino and J. Hubmayr and K. Ichiki and T. Iida and H. Imada and H. Ishino and G. Jaehnig and N. Katayama and A. Kato and R. Keskitalo and T. Kisner and Y. Kobayashi and A. Kogut and K. Kohri and E. Komatsu and K. Komatsu and K. Konishi and N. Krachmalnicoff and C. L. Kuo and L. Lamagna and M. Lattanzi and A. T. Lee and C. Leloup and F. Levrier and E. Linder and G. Luzzi and J. Macias-Perez and B. Maffei and D. Maino and S. Mandelli and E. Martínez-González and S. Masi and M. Massa and S. Matarrese and F. T. Matsuda and T. Matsumura and L. Mele and M. Migliaccio and Y. Minami and A. Moggi and J. Montgomery and L. Montier and G. Morgante and B. Mot and Y. Nagano and T. Nagasaki and R. Nagata and R. Nakano and T. Namikawa and F. Nati and P. Natoli and S. Nerval and F. Noviello and K. Odagiri and S. Oguri and H. Ohsaki and L. Pagano and A. Paiella and D. Paoletti and A. Passerini and G. Patanchon and F. Piacentini and M. Piat and G. Polenta and D. Poletti and T. Prouvé and G. Puglisi and D. Rambaud and C. Raum and S. Realini and M. Reinecke and M. Remazeilles and A. Ritacco and G. Roudil and J. A. Rubino-Martin and M. Russell and H. Sakurai and Y. Sakurai and M. Sasaki and D. Scott and Y. Sekimoto and K. Shinozaki and M. Shiraishi and P. Shirron and G. Signorelli and F. Spinella and S. Stever and R. Stompor and S. Sugiyama and R. M. Sullivan and A. Suzuki and T. L. Svalheim and E. Switzer and R. Takaku and H. Takakura and Y. Takase and A. Tartari and Y. Terao and J. Thermeau and H. Thommesen and K. L. Thompson and M. Tomasi and M. Tominaga and M. Tristram and M. Tsuji and M. Tsujimoto and L. Vacher and P. Vielva and N. Vittorio and W. Wang and K. Watanuki and I. K. Wehus and J. Weller and B. Westbrook and J. Wilms and E. J. Wollack and J. Yumoto and M. Zannoni},
      year={2022},
      eprint={2202.02773},
      archivePrefix={arXiv},
      primaryClass={astro-ph.IM}
}

@ARTICLE{dipole_plank2021,
       author = {{Delouis}, J. -M. and {Puget}, J. -L. and {Vibert}, L.},
        title = "{Improved large-scale interstellar dust foreground model and CMB solar dipole measurement}",
      journal = {\aap},
     keywords = {surveys, cosmic background radiation, diffuse radiation, methods: data analysis, dust, extinction, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jun,
       volume = {650},
          eid = {A82},
        pages = {A82},
          doi = {10.1051/0004-6361/202140616},
archivePrefix = {arXiv},
       eprint = {2102.10004},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...650A..82D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SW_effect1967,
       author = {{Sachs}, R.~K. and {Wolfe}, A.~M.},
        title = "{Perturbations of a Cosmological Model and Angular Variations of the Microwave Background}",
      journal = {\apj},
         year = 1967,
        month = jan,
       volume = {147},
        pages = {73},
          doi = {10.1086/148982},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967ApJ...147...73S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seljak1997polarization,
       author = {{Seljak}, Uro{\v{s}}},
        title = "{Measuring Polarization in the Cosmic Microwave Background}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Theory, Methods: Data Analysis, Polarization, Astrophysics},
         year = 1997,
        month = jun,
       volume = {482},
       number = {1},
        pages = {6-16},
          doi = {10.1086/304123},
archivePrefix = {arXiv},
       eprint = {astro-ph/9608131},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...482....6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zaldarriaga1997allsky,
       author = {{Zaldarriaga}, Matias and {Seljak}, Uro{\v{s}}},
        title = "{All-sky analysis of polarization in the microwave background}",
      journal = {\prd},
     keywords = {98.70.Vc, 98.80.Cq, Background radiations, Particle-theory and field-theory models of the early Universe, Astrophysics},
         year = 1997,
        month = feb,
       volume = {55},
       number = {4},
        pages = {1830-1840},
          doi = {10.1103/PhysRevD.55.1830},
archivePrefix = {arXiv},
       eprint = {astro-ph/9609170},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvD..55.1830Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seljak1997signature,
       author = {{Seljak}, Uro{\v{s}} and {Zaldarriaga}, Matias},
        title = "{Signature of Gravity Waves in the Polarization of the Microwave Background}",
      journal = {\prl},
     keywords = {Astrophysics, General Relativity and Quantum Cosmology},
         year = 1997,
        month = mar,
       volume = {78},
       number = {11},
        pages = {2054-2057},
          doi = {10.1103/PhysRevLett.78.2054},
archivePrefix = {arXiv},
       eprint = {astro-ph/9609169},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvL..78.2054S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kamionkowski1997statistics,
       author = {{Kamionkowski}, Marc and {Kosowsky}, Arthur and {Stebbins}, Albert},
        title = "{Statistics of cosmic microwave background polarization}",
      journal = {\prd},
     keywords = {98.70.Vc, 98.80.Cq, Background radiations, Particle-theory and field-theory models of the early Universe, Astrophysics, High Energy Physics - Phenomenology},
         year = 1997,
        month = jun,
       volume = {55},
       number = {12},
        pages = {7368-7388},
          doi = {10.1103/PhysRevD.55.7368},
archivePrefix = {arXiv},
       eprint = {astro-ph/9611125},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvD..55.7368K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{polnarev1985polarization,
       author = {{Polnarev}, A.~G.},
        title = "{Polarization and Anisotropy Induced in the Microwave Background by Cosmological Gravitational Waves}",
      journal = {\sovast},
         year = 1985,
        month = dec,
       volume = {29},
        pages = {607-613},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985SvA....29..607P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hu1997polprimer,
       author = {{Hu}, Wayne and {White}, Martin},
        title = "{A CMB polarization primer}",
      journal = {\na},
     keywords = {Astrophysics},
         year = 1997,
        month = oct,
       volume = {2},
       number = {4},
        pages = {323-344},
          doi = {10.1016/S1384-1076(97)00022-5},
archivePrefix = {arXiv},
       eprint = {astro-ph/9706147},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997NewA....2..323H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ma1995cosmological,
       author = {{Ma}, Chung-Pei and {Bertschinger}, Edmund},
        title = "{Cosmological Perturbation Theory in the Synchronous and Conformal Newtonian Gauges}",
      journal = {\apj},
     keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: THEORY, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE, GRAVITATION, COSMOLOGY: DARK MATTER, ELEMENTARY PARTICLES, Astrophysics, High Energy Physics - Phenomenology},
         year = 1995,
        month = dec,
       volume = {455},
        pages = {7},
          doi = {10.1086/176550},
archivePrefix = {arXiv},
       eprint = {astro-ph/9506072},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...455....7M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{komatsu2022newphysics,
       author = {{Komatsu}, Eiichiro},
        title = "{New physics from the polarized light of the cosmic microwave background}",
      journal = {Nature Reviews Physics},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2022,
        month = jul,
       volume = {4},
       number = {7},
        pages = {452-469},
          doi = {10.1038/s42254-022-00452-4},
archivePrefix = {arXiv},
       eprint = {2202.13919},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022NatRP...4..452K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sato1981firstorder,
       author = {{Sato}, K.},
        title = "{First-order phase transition of a vacuum and the expansion of the Universe}",
      journal = {\mnras},
     keywords = {Cosmology, Expansion, Gauge Theory, Phase Transformations, Universe, Vacuum, Baryons, Bubbles, Fluctuation Theory, Galactic Evolution, Nucleation, Photons, Astrophysics},
         year = 1981,
        month = may,
       volume = {195},
        pages = {467-479},
          doi = {10.1093/mnras/195.3.467},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981MNRAS.195..467S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{guth1981inflationary,
       author = {{Guth}, Alan H.},
        title = "{Inflationary universe: A possible solution to the horizon and flatness problems}",
      journal = {\prd},
         year = 1981,
        month = jan,
       volume = {23},
       number = {2},
        pages = {347-356},
          doi = {10.1103/PhysRevD.23.347},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981PhRvD..23..347G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021BICEP,
       author = {{Ade}, P.~A.~R. and {Ahmed}, Z. and {Amiri}, M. and {Barkats}, D. and {Thakur}, R. Basu and {Bischoff}, C.~A. and {Beck}, D. and {Bock}, J.~J. and {Boenish}, H. and {Bullock}, E. and {Buza}, V. and {Cheshire}, J.~R. and {Connors}, J. and {Cornelison}, J. and {Crumrine}, M. and {Cukierman}, A. and {Denison}, E.~V. and {Dierickx}, M. and {Duband}, L. and {Eiben}, M. and {Fatigoni}, S. and {Filippini}, J.~P. and {Fliescher}, S. and {Goeckner-Wald}, N. and {Goldfinger}, D.~C. and {Grayson}, J. and {Grimes}, P. and {Hall}, G. and {Halal}, G. and {Halpern}, M. and {Hand}, E. and {Harrison}, S. and {Henderson}, S. and {Hildebrandt}, S.~R. and {Hilton}, G.~C. and {Hubmayr}, J. and {Hui}, H. and {Irwin}, K.~D. and {Kang}, J. and {Karkare}, K.~S. and {Karpel}, E. and {Kefeli}, S. and {Kernasovskiy}, S.~A. and {Kovac}, J.~M. and {Kuo}, C.~L. and {Lau}, K. and {Leitch}, E.~M. and {Lennox}, A. and {Megerian}, K.~G. and {Minutolo}, L. and {Moncelsi}, L. and {Nakato}, Y. and {Namikawa}, T. and {Nguyen}, H.~T. and {O'Brient}, R. and {Ogburn}, R.~W. and {Palladino}, S. and {Prouve}, T. and {Pryke}, C. and {Racine}, B. and {Reintsema}, C.~D. and {Richter}, S. and {Schillaci}, A. and {Schwarz}, R. and {Schmitt}, B.~L. and {Sheehy}, C.~D. and {Soliman}, A. and {Germaine}, T. St. and {Steinbach}, B. and {Sudiwala}, R.~V. and {Teply}, G.~P. and {Thompson}, K.~L. and {Tolan}, J.~E. and {Tucker}, C. and {Turner}, A.~D. and {Umilt{\`a}}, C. and {Verg{\`e}s}, C. and {Vieregg}, A.~G. and {Wandui}, A. and {Weber}, A.~C. and {Wiebe}, D.~V. and {Willmert}, J. and {Wong}, C.~L. and {Wu}, W.~L.~K. and {Yang}, H. and {Yoon}, K.~W. and {Young}, E. and {Yu}, C. and {Zeng}, L. and {Zhang}, C. and {Zhang}, S. and {Bicep/Keck Collaboration}},
        title = "{Improved Constraints on Primordial Gravitational Waves using Planck, WMAP, and BICEP/Keck Observations through the 2018 Observing Season}",
      journal = {\prl},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = oct,
       volume = {127},
       number = {15},
          eid = {151301},
        pages = {151301},
          doi = {10.1103/PhysRevLett.127.151301},
archivePrefix = {arXiv},
       eprint = {2110.00483},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PhRvL.127o1301A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{achucarro2022inflation,
       author = {{Ach{\'u}carro}, Ana and {Biagetti}, Matteo and {Braglia}, Matteo and {Cabass}, Giovanni and {Caldwell}, Robert and {Castorina}, Emanuele and {Chen}, Xingang and {Coulton}, William and {Flauger}, Raphael and {Fumagalli}, Jacopo and {Ivanov}, Mikhail M. and {Lee}, Hayden and {Maleknejad}, Azadeh and {Meerburg}, P. Daniel and {Moradinezhad Dizgah}, Azadeh and {Palma}, Gonzalo A. and {Pimentel}, Guilherme L. and {Renaux-Petel}, S{\'e}bastien and {Wallisch}, Benjamin and {Wandelt}, Benjamin D. and {Witkowski}, Lukas T. and {Kimmy Wu}, W.~L.},
        title = "{Inflation: Theory and Observations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology, High Energy Physics - Theory},
         year = 2022,
        month = mar,
          eid = {arXiv:2203.08128},
        pages = {arXiv:2203.08128},
          doi = {10.48550/arXiv.2203.08128},
archivePrefix = {arXiv},
       eprint = {2203.08128},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220308128A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{hinshaw2013nineyear,
       author = {{Hinshaw}, G. and {Larson}, D. and {Komatsu}, E. and {Spergel}, D.~N. and {Bennett}, C.~L. and {Dunkley}, J. and {Nolta}, M.~R. and {Halpern}, M. and {Hill}, R.~S. and {Odegard}, N. and {Page}, L. and {Smith}, K.~M. and {Weiland}, J.~L. and {Gold}, B. and {Jarosik}, N. and {Kogut}, A. and {Limon}, M. and {Meyer}, S.~S. and {Tucker}, G.~S. and {Wollack}, E. and {Wright}, E.~L.},
        title = "{Nine-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results}",
      journal = {\apjs},
     keywords = {cosmic background radiation, cosmology: observations, dark matter, early universe, instrumentation: detectors, space vehicles, space vehicles: instruments, telescopes, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = oct,
       volume = {208},
       number = {2},
          eid = {19},
        pages = {19},
          doi = {10.1088/0067-0049/208/2/19},
archivePrefix = {arXiv},
       eprint = {1212.5226},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..208...19H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{planck2013cosmological,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and et al.},
        title = "{Planck 2013 results. XVI. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmological parameters, early Universe, inflation, primordial nucleosynthesis, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = nov,
       volume = {571},
          eid = {A16},
        pages = {A16},
          doi = {10.1051/0004-6361/201321591},
archivePrefix = {arXiv},
       eprint = {1303.5076},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...571A..16P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{starobinsky1980newtype,
       author = {{Starobinsky}, A.~A.},
        title = "{A new type of isotropic cosmological models without singularity}",
      journal = {Physics Letters B},
         year = 1980,
        month = mar,
       volume = {91},
       number = {1},
        pages = {99-102},
          doi = {10.1016/0370-2693(80)90670-X},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980PhLB...91...99S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{bond1997theoretical,
       author = {{Bond}, J.~R.},
        title = "{The theoretical agenda in CMB research.}",
     keywords = {Cosmic Microwave Background: Anisotropy, Cosmic Microwave Background: Early Universe, Astrophysics},
    booktitle = {Microwave Background Anisotropies},
         year = 1997,
       editor = {{Bouchet}, Francois R. and {Gispert}, Richard and {Guiderdoni}, Bruno and {Tr{\^a}n Thanh V{\^a}n}, Jean},
       volume = {16},
        month = jan,
        pages = {15-22},
          doi = {10.48550/arXiv.astro-ph/9610119},
archivePrefix = {arXiv},
       eprint = {astro-ph/9610119},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997mba..conf...15B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bond1987statistics,
       author = {{Bond}, J.~R. and {Efstathiou}, G.},
        title = "{The statistics of cosmic background radiation fluctuations}",
      journal = {\mnras},
     keywords = {Computational Astrophysics, Cosmology, Radiation Distribution, Relic Radiation, Statistical Analysis, Angular Correlation, Anisotropy, Correlation, Dark Matter, Power Spectra, Space Radiation},
         year = 1987,
        month = jun,
       volume = {226},
        pages = {655-687},
          doi = {10.1093/mnras/226.3.655},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987MNRAS.226..655B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{antony2000efficient,
       author = {{Lewis}, Antony and {Challinor}, Anthony and {Lasenby}, Anthony},
        title = "{Efficient Computation of Cosmic Microwave Background Anisotropies in Closed Friedmann-Robertson-Walker Models}",
      journal = {\apj},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Theory, Astrophysics},
         year = 2000,
        month = aug,
       volume = {538},
       number = {2},
        pages = {473-476},
          doi = {10.1086/309179},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911177},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...538..473L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{antony2013efficient,
       author = {{Lewis}, Antony},
        title = "{Efficient sampling of fast and slow cosmological parameters}",
      journal = {\prd},
     keywords = {98.80.-k, 98.70.Vc, 98.80.Es, Cosmology, Background radiations, Observational cosmology, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2013,
        month = may,
       volume = {87},
       number = {10},
          eid = {103529},
        pages = {103529},
          doi = {10.1103/PhysRevD.87.103529},
archivePrefix = {arXiv},
       eprint = {1304.4473},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PhRvD..87j3529L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{howlett2012cmb,
       author = {{Howlett}, Cullan and {Lewis}, Antony and {Hall}, Alex and {Challinor}, Anthony},
        title = "{CMB power spectrum parameter degeneracies in the era of precision cosmology}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2012,
        month = apr,
       volume = {2012},
       number = {4},
          eid = {027},
        pages = {027},
          doi = {10.1088/1475-7516/2012/04/027},
archivePrefix = {arXiv},
       eprint = {1201.3654},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012JCAP...04..027H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bernardis2000boomerang,
       author = {{de Bernardis}, P. and {Ade}, P.~A.~R. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Boscaleri}, A. and {Coble}, K. and {Crill}, B.~P. and {De Gasperis}, G. and {Farese}, P.~C. and {Ferreira}, P.~G. and {Ganga}, K. and {Giacometti}, M. and {Hivon}, E. and {Hristov}, V.~V. and {Iacoangeli}, A. and {Jaffe}, A.~H. and {Lange}, A.~E. and {Martinis}, L. and {Masi}, S. and {Mason}, P.~V. and {Mauskopf}, P.~D. and {Melchiorri}, A. and {Miglio}, L. and {Montroy}, T. and {Netterfield}, C.~B. and {Pascale}, E. and {Piacentini}, F. and {Pogosyan}, D. and {Prunet}, S. and {Rao}, S. and {Romeo}, G. and {Ruhl}, J.~E. and {Scaramuzzi}, F. and {Sforna}, D. and {Vittorio}, N.},
        title = "{A flat Universe from high-resolution maps of the cosmic microwave background radiation}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2000,
        month = apr,
       volume = {404},
       number = {6781},
        pages = {955-959},
          doi = {10.1038/35010035},
archivePrefix = {arXiv},
       eprint = {astro-ph/0004404},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000Natur.404..955D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hanany2000maxima,
       author = {{Hanany}, S. and {Ade}, P. and {Balbi}, A. and {Bock}, J. and {Borrill}, J. and {Boscaleri}, A. and {de Bernardis}, P. and {Ferreira}, P.~G. and {Hristov}, V.~V. and {Jaffe}, A.~H. and {Lange}, A.~E. and {Lee}, A.~T. and {Mauskopf}, P.~D. and {Netterfield}, C.~B. and {Oh}, S. and {Pascale}, E. and {Rabii}, B. and {Richards}, P.~L. and {Smoot}, G.~F. and {Stompor}, R. and {Winant}, C.~D. and {Wu}, J.~H.~P.},
        title = "{MAXIMA-1: A Measurement of the Cosmic Microwave Background Anisotropy on Angular Scales of 10'-5{\textdegree}}",
      journal = {\apjl},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Astrophysics},
         year = 2000,
        month = dec,
       volume = {545},
       number = {1},
        pages = {L5-L9},
          doi = {10.1086/317322},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005123},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...545L...5H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{grishchuk1974amplification,
       author = {{Grishchuk}, L.~P.},
        title = "{Amplification of gravitational waves in an isotropic universe.}",
      journal = {Zhurnal Eksperimentalnoi i Teoreticheskoi Fiziki},
         year = 1974,
        month = jan,
       volume = {67},
        pages = {825-838},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ZhETF..67..825G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{peebles1970primeval,
       author = {{Peebles}, P.~J.~E. and {Yu}, J.~T.},
        title = "{Primeval Adiabatic Perturbation in an Expanding Universe}",
      journal = {\apj},
         year = 1970,
        month = dec,
       volume = {162},
        pages = {815},
          doi = {10.1086/150713},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970ApJ...162..815P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hu1996acoustic,
       author = {{Hu}, Wayne and {White}, Martin},
        title = "{Acoustic Signatures in the Cosmic Microwave Background}",
      journal = {\apj},
     keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: THEORY, Astrophysics},
         year = 1996,
        month = nov,
       volume = {471},
        pages = {30},
          doi = {10.1086/177951},
archivePrefix = {arXiv},
       eprint = {astro-ph/9602019},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...471...30H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hu1997cmbanisotropies,
       author = {{Hu}, Wayne and {White}, Martin},
        title = "{CMB anisotropies: Total angular momentum method}",
      journal = {\prd},
     keywords = {98.70.Vc, 98.80.Es, Background radiations, Observational cosmology, Astrophysics},
         year = 1997,
        month = jul,
       volume = {56},
       number = {2},
        pages = {596-615},
          doi = {10.1103/PhysRevD.56.596},
archivePrefix = {arXiv},
       eprint = {astro-ph/9702170},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997PhRvD..56..596H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{einstein1911einfluss,
  title={{\"U}ber den Einflu{\ss} der Schwerkraft auf die Ausbreitung des Lichtes},
  author={Einstein, Albert and others},
  journal={Annalen der Physik},
  volume={35},
  number={10},
  pages={898--908},
  year={1911},
  publisher={Springer}
}

@ARTICLE{seljak1996gravitational,
       author = {{Seljak}, Uros},
        title = "{Gravitational Lensing Effect on Cosmic Microwave Background Anisotropies: A Power Spectrum Approach}",
      journal = {\apj},
     keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE, COSMOLOGY: GRAVITATIONAL LENSING, Astrophysics, General Relativity and Quantum Cosmology},
         year = 1996,
        month = may,
       volume = {463},
        pages = {1},
          doi = {10.1086/177218},
archivePrefix = {arXiv},
       eprint = {astro-ph/9505109},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...463....1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{keisler2011measurement,
       author = {{Keisler}, R. and {Reichardt}, C.~L. and {Aird}, K.~A. and {Benson}, B.~A. and {Bleem}, L.~E. and {Carlstrom}, J.~E. and {Chang}, C.~L. and {Cho}, H.~M. and {Crawford}, T.~M. and {Crites}, A.~T. and {de Haan}, T. and {Dobbs}, M.~A. and {Dudley}, J. and {George}, E.~M. and {Halverson}, N.~W. and {Holder}, G.~P. and {Holzapfel}, W.~L. and {Hoover}, S. and {Hou}, Z. and {Hrubes}, J.~D. and {Joy}, M. and {Knox}, L. and {Lee}, A.~T. and {Leitch}, E.~M. and {Lueker}, M. and {Luong-Van}, D. and {McMahon}, J.~J. and {Mehl}, J. and {Meyer}, S.~S. and {Millea}, M. and {Mohr}, J.~J. and {Montroy}, T.~E. and {Natoli}, T. and {Padin}, S. and {Plagge}, T. and {Pryke}, C. and {Ruhl}, J.~E. and {Schaffer}, K.~K. and {Shaw}, L. and {Shirokoff}, E. and {Spieler}, H.~G. and {Staniszewski}, Z. and {Stark}, A.~A. and {Story}, K. and {van Engelen}, A. and {Vanderlinde}, K. and {Vieira}, J.~D. and {Williamson}, R. and {Zahn}, O.},
        title = "{A Measurement of the Damping Tail of the Cosmic Microwave Background Power Spectrum with the South Pole Telescope}",
      journal = {\apj},
     keywords = {cosmic background radiation, cosmological parameters, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = dec,
       volume = {743},
       number = {1},
          eid = {28},
        pages = {28},
          doi = {10.1088/0004-637X/743/1/28},
archivePrefix = {arXiv},
       eprint = {1105.3182},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...743...28K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boggess1992cobe,
       author = {{Boggess}, N.~W. and {Mather}, J.~C. and {Weiss}, R. and {Bennett}, C.~L. and {Cheng}, E.~S. and {Dwek}, E. and {Gulkis}, S. and {Hauser}, M.~G. and {Janssen}, M.~A. and {Kelsall}, T. and {Meyer}, S.~S. and {Moseley}, S.~H. and {Murdock}, T.~L. and {Shafer}, R.~A. and {Silverberg}, R.~F. and {Smoot}, G.~F. and {Wilkinson}, D.~T. and {Wright}, E.~L.},
        title = "{The COBE Mission: Its Design and Performance Two Years after Launch}",
      journal = {\apj},
     keywords = {Cosmic Background Explorer Satellite, Infrared Radiation, Microwaves, Relic Radiation, Spaceborne Astronomy, Astronomical Satellites, Radiation Measurement, Satellite Instruments, Astrophysics, ARTIFICIAL SATELLITES, SPACE PROBES, COSMOLOGY: COSMIC MICROWAVE BACKGROUND},
         year = 1992,
        month = oct,
       volume = {397},
        pages = {420},
          doi = {10.1086/171797},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992ApJ...397..420B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wright1996scanning,
       author = {{Wright}, Edward L.},
        title = "{Scanning and Mapping Strategies for CMB Experiments}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = 1996,
        month = nov,
          eid = {astro-ph/9612006},
        pages = {astro-ph/9612006},
          doi = {10.48550/arXiv.astro-ph/9612006},
archivePrefix = {arXiv},
       eprint = {astro-ph/9612006},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996astro.ph.12006W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{delabrouille1998scanning,
       author = {{Delabrouille}, J. and {Puget}, J. -L. and {Gispert}, R. and {Lamarre}, J. -M.},
        title = "{Scanning strategies for the Planck mission}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = 1998,
        month = oct,
          eid = {astro-ph/9810478},
        pages = {astro-ph/9810478},
          doi = {10.48550/arXiv.astro-ph/9810478},
archivePrefix = {arXiv},
       eprint = {astro-ph/9810478},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998astro.ph.10478D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maris2006flexible,
       author = {{Maris}, M. and {Bersanelli}, M. and {Burigana}, C. and {Cappellini}, B. and {Dupac}, X. and {Morgante}, G. and {Pasian}, F. and {Sandri}, M. and {Sinigaglia}, A. and {Terenzi}, L. and {PLANCK Collaboration}},
        title = "{The Flexible Planck Scanning Strategy}",
      journal = {Memorie della Societa Astronomica Italiana Supplementi},
     keywords = {Cosmology: diffuse radiation, cosmic microwave background, Space vehicles: instruments.},
         year = 2006,
        month = jan,
       volume = {9},
        pages = {460},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MSAIS...9..460M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{planck_prelaunch,
       author = {{Tauber}, J.~A. and {Mandolesi}, N. and {Puget}, J. -L. and {Banos}, T. and {Bersanelli}, M. and {Bouchet}, F.~R. and {Butler}, R.~C. and {Charra}, J. and {Crone}, G. and {Dodsworth}, J. and {Efstathiou}, G. and {Gispert}, R. and {Guyot}, G. and {Gregorio}, A. and {Juillet}, J.~J. and {Lamarre}, J. -M. and {Laureijs}, R.~J. and {Lawrence}, C.~R. and {N{\o}rgaard-Nielsen}, H.~U. and {Passvogel}, T. and {Reix}, J.~M. and {Texier}, D. and {Vibert}, L. and {Zacchei}, A. and {Ade}, P.~A.~R. and {Aghanim}, N. and {Aja}, B. and {Alippi}, E. and {Aloy}, L. and {Armand}, P. and {Arnaud}, M. and {Arondel}, A. and {Arreola-Villanueva}, A. and {Artal}, E. and {Artina}, E. and {Arts}, A. and {Ashdown}, M. and {Aumont}, J. and {Azzaro}, M. and {Bacchetta}, A. and {Baccigalupi}, C. and {Baker}, M. and {Balasini}, M. and {Balbi}, A. and {Banday}, A.~J. and {Barbier}, G. and {Barreiro}, R.~B. and {Bartelmann}, M. and {Battaglia}, P. and {Battaner}, E. and {Benabed}, K. and {Beney}, J. -L. and {Beneyton}, R. and {Bennett}, K. and {Benoit}, A. and {Bernard}, J. -P. and {Bhandari}, P. and {Bhatia}, R. and {Biggi}, M. and {Biggins}, R. and {Billig}, G. and {Blanc}, Y. and {Blavot}, H. and {Bock}, J.~J. and {Bonaldi}, A. and {Bond}, R. and {Bonis}, J. and {Borders}, J. and {Borrill}, J. and {Boschini}, L. and {Boulanger}, F. and {Bouvier}, J. and {Bouzit}, M. and {Bowman}, R. and {Br{\'e}elle}, E. and {Bradshaw}, T. and {Braghin}, M. and {Bremer}, M. and {Brienza}, D. and {Broszkiewicz}, D. and {Burigana}, C. and {Burkhalter}, M. and {Cabella}, P. and {Cafferty}, T. and {Cairola}, M. and {Caminade}, S. and {Camus}, P. and {Cantalupo}, C.~M. and {Cappellini}, B. and {Cardoso}, J. -F. and {Carr}, R. and {Catalano}, A. and {Cay{\'o}n}, L. and {Cesa}, M. and {Chaigneau}, M. and {Challinor}, A. and {Chamballu}, A. and {Chambelland}, J.~P. and {Charra}, M. and {Chiang}, L. -Y. and {Chlewicki}, G. and {Christensen}, P.~R. and {Church}, S. and {Ciancietta}, E. and {Cibrario}, M. and {Cizeron}, R. and {Clements}, D. and {Collaudin}, B. and {Colley}, J. -M. and {Colombi}, S. and {Colombo}, A. and {Colombo}, F. and {Corre}, O. and {Couchot}, F. and {Cougrand}, B. and {Coulais}, A. and {Couzin}, P. and {Crane}, B. and {Crill}, B. and {Crook}, M. and {Crumb}, D. and {Cuttaia}, F. and {D{\"o}rl}, U. and {da Silva}, P. and {Daddato}, R. and {Damasio}, C. and {Danese}, L. and {D'Aquino}, G. and {D'Arcangelo}, O. and {Dassas}, K. and {Davies}, R.~D. and {Davies}, W. and {Davis}, R.~J. and {de Bernardis}, P. and {de Chambure}, D. and {de Gasperis}, G. and {de La Fuente}, M.~L. and {de Paco}, P. and {de Rosa}, A. and {de Troia}, G. and {de Zotti}, G. and {Dehamme}, M. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {di Girolamo}, G. and {Dickinson}, C. and {Doelling}, E. and {Dolag}, K. and {Domken}, I. and {Douspis}, M. and {Doyle}, D. and {Du}, S. and {Dubruel}, D. and {Dufour}, C. and {Dumesnil}, C. and {Dupac}, X. and {Duret}, P. and {Eder}, C. and {Elfving}, A. and {En{\ss}lin}, T.~A. and {Eng}, P. and {English}, K. and {Eriksen}, H.~K. and {Estaria}, P. and {Falvella}, M.~C. and {Ferrari}, F. and {Finelli}, F. and {Fishman}, A. and {Fogliani}, S. and {Foley}, S. and {Fonseca}, A. and {Forma}, G. and {Forni}, O. and {Fosalba}, P. and {Fourmond}, J. -J. and {Frailis}, M. and {Franceschet}, C. and {Franceschi}, E. and {Fran{\c{c}}ois}, S. and {Frerking}, M. and {G{\'o}mez-Re{\~n}asco}, M.~F. and {G{\'o}rski}, K.~M. and {Gaier}, T.~C. and {Galeotta}, S. and {Ganga}, K. and {Garc{\'\i}a L{\'a}zaro}, J. and {Garnica}, A. and {Gaspard}, M. and {Gavila}, E. and {Giard}, M. and {Giardino}, G. and {Gienger}, G. and {Giraud-Heraud}, Y. and {Glorian}, J. -M. and {Griffin}, M. and {Gruppuso}, A. and {Guglielmi}, L. and {Guichon}, D. and {Guillaume}, B. and {Guillouet}, P. and {Haissinski}, J. and {Hansen}, F.~K. and {Hardy}, J. and {Harrison}, D. and {Hazell}, A. and {Hechler}, M. and {Heckenauer}, V. and {Heinzer}, D. and {Hell}, R. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Herreros}, J.~M. and {Hervier}, V. and {Heske}, A. and {Heurtel}, A. and {Hildebrandt}, S.~R. and {Hills}, R. and {Hivon}, E. and {Hobson}, M. and {Hollert}, D. and {Holmes}, W. and {Hornstrup}, A. and {Hovest}, W. and {Hoyland}, R.~J. and {Huey}, G. and {Huffenberger}, K.~M. and {Hughes}, N. and {Israelsson}, U. and {Jackson}, B. and {Jaffe}, A. and {Jaffe}, T.~R. and {Jagemann}, T. and {Jessen}, N.~C. and {Jewell}, J. and {Jones}, W. and {Juvela}, M. and {Kaplan}, J. and {Karlman}, P. and {Keck}, F. and {Keih{\"a}nen}, E. and {King}, M. and {Kisner}, T.~S. and {Kletzkine}, P. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Koch}, T. and {Krassenburg}, M. and {Kurki-Suonio}, H. and {L{\"a}hteenm{\"a}ki}, A. and {Lagache}, G. and {Lagorio}, E. and {Lami}, P. and {Lande}, J. and {Lange}, A. and {Langlet}, F. and {Lapini}, R. and {Lapolla}, M. and {Lasenby}, A. and {Le Jeune}, M. and {Leahy}, J.~P. and {Lefebvre}, M. and {Legrand}, F. and {Le Meur}, G. and {Leonardi}, R. and {Leriche}, B. and {Leroy}, C. and {Leutenegger}, P. and {Levin}, S.~M. and {Lilje}, P.~B. and {Lindensmith}, C. and {Linden-V{\o}rnle}, M. and {Loc}, A. and {Longval}, Y. and {Lubin}, P.~M. and {Luchik}, T. and {Luthold}, I. and {Macias-Perez}, J.~F. and {Maciaszek}, T. and {MacTavish}, C. and {Madden}, S. and {Maffei}, B. and {Magneville}, C. and {Maino}, D. and {Mambretti}, A. and {Mansoux}, B. and {Marchioro}, D. and {Maris}, M. and {Marliani}, F. and {Marrucho}, J. -C. and {Mart{\'\i}-Canales}, J. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Mart{\'\i}n-Polegre}, A. and {Martin}, P. and {Marty}, C. and {Marty}, W. and {Masi}, S. and {Massardi}, M. and {Matarrese}, S. and {Matthai}, F. and {Mazzotta}, P. and {McDonald}, A. and {McGrath}, P. and {Mediavilla}, A. and {Meinhold}, P.~R. and {M{\'e}lin}, J. -B. and {Melot}, F. and {Mendes}, L. and {Mennella}, A. and {Mervier}, C. and {Meslier}, L. and {Miccolis}, M. and {Miville-Deschenes}, M. -A. and {Moneti}, A. and {Montet}, D. and {Montier}, L. and {Mora}, J. and {Morgante}, G. and {Morigi}, G. and {Morinaud}, G. and {Morisset}, N. and {Mortlock}, D. and {Mottet}, S. and {Mulder}, J. and {Munshi}, D. and {Murphy}, A. and {Murphy}, P. and {Musi}, P. and {Narbonne}, J. and {Naselsky}, P. and {Nash}, A. and {Nati}, F. and {Natoli}, P. and {Netterfield}, B. and {Newell}, J. and {Nexon}, M. and {Nicolas}, C. and {Nielsen}, P.~H. and {Ninane}, N. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {O'Dwyer}, I.~J. and {Oldeman}, P. and {Olivier}, P. and {Ouchet}, L. and {Oxborrow}, C.~A. and {P{\'e}rez-Cuevas}, L. and {Pagan}, L. and {Paine}, C. and {Pajot}, F. and {Paladini}, R. and {Pancher}, F. and {Panh}, J. and {Parks}, G. and {Parnaudeau}, P. and {Partridge}, B. and {Parvin}, B. and {Pascual}, J.~P. and {Pasian}, F. and {Pearson}, D.~P. and {Pearson}, T. and {Pecora}, M. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Piersanti}, O. and {Plaige}, E. and {Plaszczynski}, S. and {Platania}, P. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Popa}, L. and {Poulleau}, G. and {Poutanen}, T. and {Pr{\'e}zeau}, G. and {Pradell}, L. and {Prina}, M. and {Prunet}, S. and {Rachen}, J.~P. and {Rambaud}, D. and {Rame}, F. and {Rasmussen}, I. and {Rautakoski}, J. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Reiter}, J. and {Renault}, C. and {Ricciardi}, S. and {Rideau}, P. and {Riller}, T. and {Ristorcelli}, I. and {Riti}, J.~B. and {Rocha}, G. and {Roche}, Y. and {Pons}, R. and {Rohlfs}, R. and {Romero}, D. and {Roose}, S. and {Rosset}, C. and {Rouberol}, S. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusconi}, P. and {Rusholme}, B. and {Salama}, M. and {Salerno}, E. and {Sandri}, M. and {Santos}, D. and {Sanz}, J.~L. and {Sauter}, L. and {Sauvage}, F. and {Savini}, G. and {Schmelzel}, M. and {Schnorhk}, A. and {Schwarz}, W. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, P. and {Shih}, C. and {Sias}, M. and {Silk}, J.~I. and {Silvestri}, R. and {Sippel}, R. and {Smoot}, G.~F. and {Starck}, J. -L. and {Stassi}, P. and {Sternberg}, J. and {Stivoli}, F. and {Stolyarov}, V. and {Stompor}, R. and {Stringhetti}, L. and {Strommen}, D. and {Stute}, T. and {Sudiwala}, R. and {Sugimura}, R. and {Sunyaev}, R. and {Sygnet}, J. -F. and {T{\"u}rler}, M. and {Taddei}, E. and {Tallon}, J. and {Tamiatto}, C. and {Taurigna}, M. and {Taylor}, D. and {Terenzi}, L. and {Thuerey}, S. and {Tillis}, J. and {Tofani}, G. and {Toffolatti}, L. and {Tommasi}, E. and {Tomasi}, M. and {Tonazzini}, E. and {Torre}, J. -P. and {Tosti}, S. and {Touze}, F. and {Tristram}, M. and {Tuovinen}, J. and {Tuttlebee}, M. and {Umana}, G. and {Valenziano}, L. and {Vall{\'e}e}, D. and {van der Vlis}, M. and {van Leeuwen}, F. and {Vanel}, J. -C. and {van-Tent}, B. and {Varis}, J. and {Vassallo}, E. and {Vescovi}, C. and {Vezzu}, F. and {Vibert}, D. and {Vielva}, P. and {Vierra}, J. and {Villa}, F. and {Vittorio}, N. and {Vuerli}, C. and {Wade}, L.~A. and {Walker}, A.~R. and {Wandelt}, B.~D. and {Watson}, C. and {Werner}, D. and {White}, M. and {White}, S.~D.~M. and {Wilkinson}, A. and {Wilson}, P. and {Woodcraft}, A. and {Yoffo}, B. and {Yun}, M. and {Yurchenko}, V. and {Yvon}, D. and {Zhang}, B. and {Zimmermann}, O. and {Zonca}, A. and {Zorita}, D.},
        title = "{Planck pre-launch status: The Planck mission}",
      journal = {\aap},
     keywords = {cosmic microwave background, space vehicles: instruments, instrumentation: detectors, instrumentation: polarimeters, submillimeter: general, radio continuum: general},
         year = 2010,
        month = sep,
       volume = {520},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/200912983},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...520A...1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{planck2014planck_mission,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Baker}, M. and {Balbi}, A. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartlett}, J.~G. and {Battaner}, E. and {Benabed}, K. and {Bennett}, K. and {Beno{\^\i}t}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bhatia}, R. and {Bock}, J.~J. and {Bonaldi}, A. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Bradshaw}, T. and {Bremer}, M. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Cabella}, P. and {Cantalupo}, C.~M. and {Cappellini}, B. and {Cardoso}, J. -F. and {Carr}, R. and {Casale}, M. and {Catalano}, A. and {Cay{\'o}n}, L. and {Challinor}, A. and {Chamballu}, A. and {Charra}, J. and {Chary}, R. -R. and {Chiang}, L. -Y. and {Chiang}, C. and {Christensen}, P.~R. and {Clements}, D.~L. and {Colombi}, S. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Crone}, G. and {Crook}, M. and {Cuttaia}, F. and {Danese}, L. and {D'Arcangelo}, O. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Bruin}, J. and {de Gasperis}, G. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {Dick}, J. and {Dickinson}, C. and {Dolag}, K. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {D{\"o}rl}, U. and {Douspis}, M. and {Dupac}, X. and {Efstathiou}, G. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Finelli}, F. and {Foley}, S. and {Forni}, O. and {Fosalba}, P. and {Frailis}, M. and {Franceschi}, E. and {Freschi}, M. and {Gaier}, T.~C. and {Galeotta}, S. and {Gallegos}, J. and {Gandolfo}, B. and {Ganga}, K. and {Giard}, M. and {Giardino}, G. and {Gienger}, G. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez}, J. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Guyot}, G. and {Haissinski}, J. and {Hansen}, F.~K. and {Harrison}, D. and {Helou}, G. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Hoyland}, R.~J. and {Huffenberger}, K.~M. and {Jaffe}, A.~H. and {Jagemann}, T. and {Jones}, W.~C. and {Juillet}, J.~J. and {Juvela}, M. and {Kangaslahti}, P. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knox}, L. and {Krassenburg}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lange}, A.~E. and {Lasenby}, A. and {Laureijs}, R.~J. and {Lawrence}, C.~R. and {Leach}, S. and {Leahy}, J.~P. and {Leonardi}, R. and {Leroy}, C. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lowe}, S. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maciaszek}, T. and {MacTavish}, C.~J. and {Maffei}, B. and {Maino}, D. and {Mandolesi}, N. and {Mann}, R. and {Maris}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Massardi}, M. and {Matarrese}, S. and {Matthai}, F. and {Mazzotta}, P. and {McDonald}, A. and {McGehee}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Melin}, J. -B. and {Mendes}, L. and {Mennella}, A. and {Mevi}, C. and {Miniscalco}, R. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Morisset}, N. and {Mortlock}, D. and {Munshi}, D. and {Murphy}, A. and {Naselsky}, P. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {O'Dwyer}, I.~J. and {Ortiz}, I. and {Osborne}, S. and {Osuna}, P. and {Oxborrow}, C.~A. and {Pajot}, F. and {Paladini}, R. and {Partridge}, B. and {Pasian}, F. and {Passvogel}, T. and {Patanchon}, G. and {Pearson}, D. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Plaszczynski}, S. and {Platania}, P. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Popa}, L. and {Poutanen}, T. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Reix}, J. -M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Salerno}, E. and {Sandri}, M. and {Santos}, D. and {Savini}, G. and {Schaefer}, B.~M. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, P. and {Simonetto}, A. and {Smoot}, G.~F. and {Sozzi}, C. and {Starck}, J. -L. and {Sternberg}, J. and {Stivoli}, F. and {Stolyarov}, V. and {Stompor}, R. and {Stringhetti}, L. and {Sudiwala}, R. and {Sunyaev}, R. and {Sygnet}, J. -F. and {Tapiador}, D. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Taylor}, D. and {Terenzi}, L. and {Texier}, D. and {Toffolatti}, L. and {Tomasi}, M. and {Torre}, J. -P. and {Tristram}, M. and {Tuovinen}, J. and {T{\"u}rler}, M. and {Tuttlebee}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Varis}, J. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Watson}, C. and {White}, S.~D.~M. and {White}, M. and {Wilkinson}, A. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck early results. I. The Planck mission}",
      journal = {\aap},
     keywords = {cosmology: observations, cosmic background radiation, surveys, space vehicles: instruments, instrumentation: detectors, catalogs, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = dec,
       volume = {536},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201116464},
archivePrefix = {arXiv},
       eprint = {1101.2022},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...536A...1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{freese1990natural,
    author = "Freese, Katherine and Frieman, Joshua A. and Olinto, Angela V.",
    title = "{Natural inflation with pseudo - Nambu-Goldstone bosons}",
    reportNumber = "FERMILAB-PUB-90-177-A",
    doi = "10.1103/PhysRevLett.65.3233",
    journal = "Phys. Rev. Lett.",
    volume = "65",
    pages = "3233--3236",
    year = "1990"
}

@ARTICLE{linder2003chaotic,
       author = {{Linde}, A.~D.},
        title = "{Chaotic inflation}",
      journal = {Physics Letters B},
         year = 1983,
        month = sep,
       volume = {129},
       number = {3-4},
        pages = {177-181},
          doi = {10.1016/0370-2693(83)90837-7},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983PhLB..129..177L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kazanas1980dynamics,
       author = {{Kazanas}, D.},
        title = "{Dynamics of the universe and spontaneous symmetry breaking}",
      journal = {\apjl},
     keywords = {Cosmology, Symmetry, Universe, Dynamic Models, Expansion, Gravitation, Astrophysics},
         year = 1980,
        month = oct,
       volume = {241},
        pages = {L59-L63},
          doi = {10.1086/183361},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980ApJ...241L..59K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{finelli2018core,
       author = {{Finelli}, F. and {Bucher}, M. and {Ach{\'u}carro}, A. and {Ballardini}, M. and {Bartolo}, N. and {Baumann}, D. and {Clesse}, S. and {Errard}, J. and {Handley}, W. and {Hindmarsh}, M. and {Kiiveri}, K. and {Kunz}, M. and {Lasenby}, A. and {Liguori}, M. and {Paoletti}, D. and {Ringeval}, C. and {V{\"a}liviita}, J. and {van Tent}, B. and {Vennin}, V. and {Ade}, P. and {Allison}, R. and {Arroja}, F. and {Ashdown}, M. and {Banday}, A.~J. and {Banerji}, R. and {Bartlett}, J.~G. and {Basak}, S. and {de Bernardis}, P. and {Bersanelli}, M. and {Bonaldi}, A. and {Borril}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Brinckmann}, T. and {Burigana}, C. and {Buzzelli}, A. and {Cai}, Z. -Y. and {Calvo}, M. and {Carvalho}, C.~S. and {Castellano}, G. and {Challinor}, A. and {Chluba}, J. and {Colantoni}, I. and {Coppolecchia}, A. and {Crook}, M. and {D'Alessandro}, G. and {D'Amico}, G. and {Delabrouille}, J. and {Desjacques}, V. and {De Zotti}, G. and {Diego}, J.~M. and {Di Valentino}, E. and {Feeney}, S. and {Fergusson}, J.~R. and {Fernandez-Cobos}, R. and {Ferraro}, S. and {Forastieri}, F. and {Galli}, S. and {Garc{\'\i}a-Bellido}, J. and {de Gasperis}, G. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Gonz{\'a}lez-Nuevo}, J. and {Grandis}, S. and {Greenslade}, J. and {Hagstotz}, S. and {Hanany}, S. and {Hazra}, D.~K. and {Hern{\'a}ndez-Monteagudo}, C. and {Hervias-Caimapo}, C. and {Hills}, M. and {Hivon}, E. and {Hu}, B. and {Kisner}, T. and {Kitching}, T. and {Kovetz}, E.~D. and {Kurki-Suonio}, H. and {Lamagna}, L. and {Lattanzi}, M. and {Lesgourgues}, J. and {Lewis}, A. and {Lindholm}, V. and {Lizarraga}, J. and {L{\'o}pez-Caniego}, M. and {Luzzi}, G. and {Maffei}, B. and {Mandolesi}, N. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Martins}, C.~J.~A.~P. and {Masi}, S. and {McCarthy}, D. and {Matarrese}, S. and {Melchiorri}, A. and {Melin}, J. -B. and {Molinari}, D. and {Monfardini}, A. and {Natoli}, P. and {Negrello}, M. and {Notari}, A. and {Oppizzi}, F. and {Paiella}, A. and {Pajer}, E. and {Patanchon}, G. and {Patil}, S.~P. and {Piat}, M. and {Pisano}, G. and {Polastri}, L. and {Polenta}, G. and {Pollo}, A. and {Poulin}, V. and {Quartin}, M. and {Ravenni}, A. and {Remazeilles}, M. and {Renzi}, A. and {Roest}, D. and {Roman}, M. and {Rubi{\~n}o-Martin}, J.~A. and {Salvati}, L. and {Starobinsky}, A.~A. and {Tartari}, A. and {Tasinato}, G. and {Tomasi}, M. and {Torrado}, J. and {Trappe}, N. and {Trombetti}, T. and {Tucci}, M. and {Tucker}, C. and {Urrestilla}, J. and {van de Weygaert}, R. and {Vielva}, P. and {Vittorio}, N. and {Young}, K. and {Zannoni}, M.},
        title = "{Exploring cosmic origins with CORE: Inflation}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = apr,
       volume = {2018},
       number = {4},
          eid = {016},
        pages = {016},
          doi = {10.1088/1475-7516/2018/04/016},
archivePrefix = {arXiv},
       eprint = {1612.08270},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018JCAP...04..016F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{ghigna2024litebird,
author = {T. Ghigna and A. Adler and K. Aizawa and H. Akamatsu and R. Akizawa and E. Allys and A. Anand and J. Aumont and J. Austermann and S. Azzoni and C. Baccigalupi and M. Ballardini and A. Banday and R. Barreiro and N. Bartolo and S. Basak and A. Basyrov and S. Beckman and M. Bersanelli and M. Bortolami and F. Bouchet and T. Brinckmann and P. Campeti and E. Carinos and A. Carones and F. J. Casas and K. Cheung and Y. Chinone and L. Clermont and F. Columbro and A. Coppolecchia and D. Curtis and P. de Bernardis and T. de Haan and E. de la Hoz and M. De Petris and S. Della Torre and G. Delle Monache and E. Di Giorgi and C. Dickinson and P. Diego-Palazuelos and J. J. D{\'i}az Garc{\'i}a and M. Dobbs and T. Dotani and H. K. Eriksen and J. Errard and T. Essinger-Hileman and N. Farias and E. Ferreira and C. Franceschet and U. Fuskeland and G. Galloni and M. Galloway and K. Ganga and M. Gerbino and M. Gervasi and R. T. G{\'e}nova-Santos and S. Giardiello and C. Gimeno-Amo and E. Gjerl{\o}w and R. Gonz{\'a}lez Gonz{\'a}lez and L. Grandsire and A. Gruppuso and N. Halverson and P. Hargrave and S. E. Harper and M. Hazumi and S. Henrot-Versill{\'e} and L. T. Hergt and D. Herranz and E. Hivon and R. Hlozek and T. D. Hoang and J. Hubmayr and K. Ichiki and K. Ikuma and H. Ishino and G. Jaehnig and B. Jost and K. Kohri and K. Konishi and L. Lamagna and M. Lattanzi and C. Leloup and F. Levrier and A. Lanoppan and G. Luzzi and J. Macias-Perez and B. Maffei and E. Marchitelli and E. Mart{\'i}nez-Gonz{\'a}lez and S. Masi and S. Matarrese and T. Matsumura and S. Micheli and M. Migliaccio and M. Monelli and L. Montier and G. Morgante and L. Mousset and Y. Nagano and R. Nagata and P. Natoli and A. Novelli and F. Noviello and I. Obata and A. Occhiuzzi and K. Odagiri and R. Omae and L. Pagano and A. Paiella and D. Paoletti and G. Pascual-Cisneros and G. Patanchon and V. Pavlidou and F. Piacentini and M. Piat and G. Piccirilli and M. Pinchera and G. Pisano and L. Porcelli and N. Raffuzzi and C. Raum and M. Remazeilles and A. Ritacco and J. Rubino-Martin and M. Ruiz-Granda and Y. Sakurai and G. Savini and D. Scott and Y. Sekimoto and M. Shiraishi and G. Signorelli and S. L. Stever and R. Sullivan and A. Suzuki and R. Takaku and H. Takakura and S. Takakura and Y. Takase and A. Tartari and K. Tassis and K. L. Thompson and M. Tomasi and M. Tristram and C. Tucker and L. Vacher and B. van Tent and P. Vielva and K. Watanuki and I. K. Wehus and B. Westbrook and G. Weymann-Despres and B. Winter and E. J. Wollack and A. Zacchei and M. Zannoni and Y. Zhou},
title = {{The LiteBIRD mission to explore cosmic inflation}},
volume = {13092},
booktitle = {Space Telescopes and Instrumentation 2024: Optical, Infrared, and Millimeter Wave},
editor = {Laura E. Coyle and Shuji Matsuura and Marshall D. Perrin},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {1309228},
keywords = {LiteBIRD, CMB, TES, Cosmic Inflation, JAXA, B-mode, Polarization},
year = {2024},
doi = {10.1117/12.3021377},
URL = {https://doi.org/10.1117/12.3021377}
}

@INPROCEEDINGS{montier2018mhft,
       author = {{Montier}, L. and {Mot}, B. and {de Bernardis}, P. and {Maffei}, B. and {Pisano}, G. and {Columbro}, F. and {Gudmundsson}, J.~E. and {Henrot-Versill{\'e}}, S. and {Lamagna}, L. and {Montgomery}, J. and {Prouv{\'e}}, T. and {Russell}, M. and {Savini}, G. and {Stever}, S. and {Thompson}, K.~L. and {Tsujimoto}, M. and {Tucker}, C. and {Westbrook}, B. and {Ade}, P.~A.~R. and {Adler}, A. and {Allys}, E. and {Arnold}, K. and {Auguste}, D. and {Aumont}, J. and {Aurlien}, R. and {Austermann}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Banerji}, R. and {Barreiro}, R.~B. and {Basak}, S. and {Beall}, J. and {Beck}, D. and {Beckman}, S. and {Bermejo}, J. and {Bersanelli}, M. and {Bonis}, J. and {Borrill}, J. and {Boulanger}, F. and {Bounissou}, S. and {Brilenkov}, M. and {Brown}, M. and {Bucher}, M. and {Calabrese}, E. and {Campeti}, P. and {Carones}, A. and {Casas}, F.~J. and {Challinor}, A. and {Chan}, V. and {Cheung}, K. and {Chinone}, Y. and {Cliche}, J.~F. and {Colombo}, L. and {Cubas}, J. and {Cukierman}, A. and {Curtis}, D. and {D'Alessandro}, G. and {Dachlythra}, N. and {De Petris}, M. and {Dickinson}, C. and {Diego-Palazuelos}, P. and {Dobbs}, M. and {Dotani}, T. and {Duband}, L. and {Duff}, S. and {Duval}, J.~M. and {Ebisawa}, K. and {Elleflot}, T. and {Eriksen}, H.~K. and {Errard}, J. and {Essinger-Hileman}, T. and {Finelli}, F. and {Flauger}, R. and {Franceschet}, C. and {Fuskeland}, U. and {Galloway}, M. and {Ganga}, K. and {Gao}, J.~R. and {Genova-Santos}, R. and {Gerbino}, M. and {Gervasi}, M. and {Ghigna}, T. and {Gjerl{\o}w}, E. and {Gradziel}, M.~L. and {Grain}, J. and {Grupp}, F. and {Gruppuso}, A. and {de Haan}, T. and {Halverson}, N.~W. and {Hargrave}, P. and {Hasebe}, T. and {Hasegawa}, M. and {Hattori}, M. and {Hazumi}, M. and {Herman}, D. and {Herranz}, D. and {Hill}, C.~A. and {Hilton}, G. and {Hirota}, Y. and {Hivon}, E. and {Hlozek}, R.~A. and {Hoshino}, Y. and {de la Hoz}, E. and {Hubmayr}, J. and {Ichiki}, K. and {Iida}, T. and {Imada}, H. and {Ishimura}, K. and {Ishino}, H. and {Jaehnig}, G. and {Kaga}, T. and {Kashima}, S. and {Katayama}, N. and {Kato}, A. and {Kawasaki}, T. and {Keskitalo}, R. and {Kisner}, T. and {Kobayashi}, Y. and {Kogiso}, N. and {Kogut}, A. and {Kohri}, K. and {Komatsu}, E. and {Komatsu}, K. and {Konishi}, K. and {Krachmalnicoff}, N. and {Kreykenbohm}, I. and {Kuo}, C.~L. and {Kushino}, A. and {Lanen}, J.~V. and {Lattanzi}, M. and {Lee}, A.~T. and {Leloup}, C. and {Levrier}, F. and {Linder}, E. and {Louis}, T. and {Luzzi}, G. and {Maciaszek}, T. and {Maino}, D. and {Maki}, M. and {Mandelli}, S. and {Martinez-Gonzalez}, E. and {Masi}, S. and {Matsumura}, T. and {Mennella}, A. and {Migliaccio}, M. and {Minami}, Y. and {Mitsuda}, K. and {Morgante}, G. and {Murata}, Y. and {Murphy}, J.~A. and {Nagai}, M. and {Nagano}, Y. and {Nagasaki}, T. and {Nagata}, R. and {Nakamura}, S. and {Namikawa}, T. and {Natoli}, P. and {Nerval}, S. and {Nishibori}, T. and {Nishino}, H. and {O'Sullivan}, C. and {Ogawa}, H. and {Ogawa}, H. and {Oguri}, S. and {Ohsaki}, H. and {Ohta}, I.~S. and {Okada}, N. and {Okada}, N. and {Pagano}, L. and {Paiella}, A. and {Paoletti}, D. and {Patanchon}, G. and {Peloton}, J. and {Piacentini}, F. and {Polenta}, G. and {Poletti}, D. and {Puglisi}, G. and {Rambaud}, D. and {Raum}, C. and {Realini}, S. and {Reinecke}, M. and {Remazeilles}, M. and {Ritacco}, A. and {Roudil}, G. and {Rubino-Martin}, J.~A. and {Sakurai}, H. and {Sakurai}, Y. and {Sandri}, M. and {Sasaki}, M. and {Scott}, D. and {Seibert}, J. and {Sekimoto}, Y. and {Sherwin}, B. and {Shinozaki}, K. and {Shiraishi}, M. and {Shirron}, P. and {Signorelli}, G. and {Smecher}, G. and {Stompor}, R. and {Sugai}, H. and {Sugiyama}, S. and {Suzuki}, A. and {Suzuki}, J. and {Svalheim}, T.~L. and {Switzer}, E. and {Takaku}, R. and {Takakura}, H. and {Takakura}, S. and {Takase}, Y. and {Takeda}, Y. and {Tartari}, A. and {Taylor}, E. and {Terao}, Y. and {Thommesen}, H. and {Thorne}, B. and {Toda}, T. and {Tomasi}, M. and {Tominaga}, M. and {Trappe}, N. and {Tristram}, M. and {Tsuji}, M. and {Ullom}, J. and {Vermeulen}, G. and {Vielva}, P. and {Villa}, F. and {Vissers}, M. and {Vittorio}, N. and {Wehus}, I. and {Weller}, J. and {Wilms}, J. and {Winter}, B. and {Wollack}, E.~J. and {Yamasaki}, N.~Y. and {Yoshida}, T. and {Yumoto}, J. and {Zannoni}, M. and {Zonca}, A.},
        title = "{Overview of the medium and high frequency telescopes of the LiteBIRD space mission}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
    booktitle = {Space Telescopes and Instrumentation 2020: Optical, Infrared, and Millimeter Wave},
         year = 2020,
       editor = {{Lystrup}, Makenzie and {Perrin}, Marshall D.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {11443},
        month = dec,
          eid = {114432G},
        pages = {114432G},
          doi = {10.1117/12.2562243},
archivePrefix = {arXiv},
       eprint = {2102.00809},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SPIE11443E..2GM},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ade2021improved,
       author = {{Ade}, P.~A.~R. and {Ahmed}, Z. and {Amiri}, M. and {Barkats}, D. and {Thakur}, R. Basu and {Bischoff}, C.~A. and {Beck}, D. and {Bock}, J.~J. and {Boenish}, H. and {Bullock}, E. and {Buza}, V. and {Cheshire}, J.~R. and {Connors}, J. and {Cornelison}, J. and {Crumrine}, M. and {Cukierman}, A. and {Denison}, E.~V. and {Dierickx}, M. and {Duband}, L. and {Eiben}, M. and {Fatigoni}, S. and {Filippini}, J.~P. and {Fliescher}, S. and {Goeckner-Wald}, N. and {Goldfinger}, D.~C. and {Grayson}, J. and {Grimes}, P. and {Hall}, G. and {Halal}, G. and {Halpern}, M. and {Hand}, E. and {Harrison}, S. and {Henderson}, S. and {Hildebrandt}, S.~R. and {Hilton}, G.~C. and {Hubmayr}, J. and {Hui}, H. and {Irwin}, K.~D. and {Kang}, J. and {Karkare}, K.~S. and {Karpel}, E. and {Kefeli}, S. and {Kernasovskiy}, S.~A. and {Kovac}, J.~M. and {Kuo}, C.~L. and {Lau}, K. and {Leitch}, E.~M. and {Lennox}, A. and {Megerian}, K.~G. and {Minutolo}, L. and {Moncelsi}, L. and {Nakato}, Y. and {Namikawa}, T. and {Nguyen}, H.~T. and {O'Brient}, R. and {Ogburn}, R.~W. and {Palladino}, S. and {Prouve}, T. and {Pryke}, C. and {Racine}, B. and {Reintsema}, C.~D. and {Richter}, S. and {Schillaci}, A. and {Schwarz}, R. and {Schmitt}, B.~L. and {Sheehy}, C.~D. and {Soliman}, A. and {Germaine}, T. St. and {Steinbach}, B. and {Sudiwala}, R.~V. and {Teply}, G.~P. and {Thompson}, K.~L. and {Tolan}, J.~E. and {Tucker}, C. and {Turner}, A.~D. and {Umilt{\`a}}, C. and {Verg{\`e}s}, C. and {Vieregg}, A.~G. and {Wandui}, A. and {Weber}, A.~C. and {Wiebe}, D.~V. and {Willmert}, J. and {Wong}, C.~L. and {Wu}, W.~L.~K. and {Yang}, H. and {Yoon}, K.~W. and {Young}, E. and {Yu}, C. and {Zeng}, L. and {Zhang}, C. and {Zhang}, S. and {Bicep/Keck Collaboration}},
        title = "{Improved Constraints on Primordial Gravitational Waves using Planck, WMAP, and BICEP/Keck Observations through the 2018 Observing Season}",
      journal = {\prl},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = oct,
       volume = {127},
       number = {15},
          eid = {151301},
        pages = {151301},
          doi = {10.1103/PhysRevLett.127.151301},
archivePrefix = {arXiv},
       eprint = {2110.00483},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PhRvL.127o1301A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{adachi2016measurement,
       author = {{Adachi}, S. and {Aguilar Fa{\'u}ndez}, M.~A.~O. and {Arnold}, K. and {Baccigalupi}, C. and {Barron}, D. and {Beck}, D. and {Bianchini}, F. and {Chapman}, S. and {Cheung}, K. and {Chinone}, Y. and {Crowley}, K. and {Dobbs}, M. and {El Bouhargani}, H. and {Elleflot}, T. and {Errard}, J. and {Fabbian}, G. and {Feng}, C. and {Fujino}, T. and {Galitzki}, N. and {Goeckner-Wald}, N. and {Groh}, J. and {Hall}, G. and {Hasegawa}, M. and {Hazumi}, M. and {Hirose}, H. and {Jaffe}, A.~H. and {Jeong}, O. and {Kaneko}, D. and {Katayama}, N. and {Keating}, B. and {Kikuchi}, S. and {Kisner}, T. and {Kusaka}, A. and {Lee}, A.~T. and {Leon}, D. and {Linder}, E. and {Lowry}, L.~N. and {Matsuda}, F. and {Matsumura}, T. and {Minami}, Y. and {Navaroli}, M. and {Nishino}, H. and {Pham}, A.~T.~P. and {Poletti}, D. and {Reichardt}, C.~L. and {Segawa}, Y. and {Siritanasak}, P. and {Tajima}, O. and {Takakura}, S. and {Takatori}, S. and {Tanabe}, D. and {Teply}, G.~P. and {Tsai}, C. and {Verg{\`e}s}, C. and {Westbrook}, B. and {Zhou}, Y. and {Polarbear Collaboration}},
        title = "{A Measurement of the CMB E-mode Angular Power Spectrum at Subdegree Scales from 670 Square Degrees of POLARBEAR Data}",
      journal = {\apj},
     keywords = {Cosmic microwave background radiation, 322, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = nov,
       volume = {904},
       number = {1},
          eid = {65},
        pages = {65},
          doi = {10.3847/1538-4357/abbacd},
archivePrefix = {arXiv},
       eprint = {2005.06168},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...904...65A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{sayre2020measurements,
       author = {{Sayre}, J.~T. and {Reichardt}, C.~L. and {Henning}, J.~W. and {Ade}, P.~A.~R. and {Anderson}, A.~J. and {Austermann}, J.~E. and {Avva}, J.~S. and {Beall}, J.~A. and {Bender}, A.~N. and {Benson}, B.~A. and {Bianchini}, F. and {Bleem}, L.~E. and {Carlstrom}, J.~E. and {Chang}, C.~L. and {Chaubal}, P. and {Chiang}, H.~C. and {Citron}, R. and {Corbett Moran}, C. and {Crawford}, T.~M. and {Crites}, A.~T. and {de Haan}, T. and {Dobbs}, M.~A. and {Everett}, W. and {Gallicchio}, J. and {George}, E.~M. and {Gilbert}, A. and {Gupta}, N. and {Halverson}, N.~W. and {Harrington}, N. and {Hilton}, G.~C. and {Holder}, G.~P. and {Holzapfel}, W.~L. and {Hrubes}, J.~D. and {Huang}, N. and {Hubmayr}, J. and {Irwin}, K.~D. and {Knox}, L. and {Lee}, A.~T. and {Li}, D. and {Lowitz}, A. and {McMahon}, J.~J. and {Meyer}, S.~S. and {Mocanu}, L.~M. and {Montgomery}, J. and {Nadolski}, A. and {Natoli}, T. and {Nibarger}, J.~P. and {Noble}, G. and {Novosad}, V. and {Padin}, S. and {Patil}, S. and {Pryke}, C. and {Ruhl}, J.~E. and {Saliwanchik}, B.~R. and {Schaffer}, K.~K. and {Sievers}, C. and {Smecher}, G. and {Stark}, A.~A. and {Tucker}, C. and {Vanderlinde}, K. and {Veach}, T. and {Vieira}, J.~D. and {Wang}, G. and {Whitehorn}, N. and {Wu}, W.~L.~K. and {Yefremenko}, V. and {SPTpol Collaboration}},
        title = "{Measurements of B -mode polarization of the cosmic microwave background from 500 square degrees of SPTpol data}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jun,
       volume = {101},
       number = {12},
          eid = {122003},
        pages = {122003},
          doi = {10.1103/PhysRevD.101.122003},
archivePrefix = {arXiv},
       eprint = {1910.05748},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PhRvD.101l2003S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bicep2_2018,
       author = {{BICEP2 Collaboration} and {Keck Array Collaboration} and {Ade}, P.~A.~R. and {Ahmed}, Z. and {Aikin}, R.~W. and {Alexander}, K.~D. and {Barkats}, D. and {Benton}, S.~J. and {Bischoff}, C.~A. and {Bock}, J.~J. and {Bowens-Rubin}, R. and {Brevik}, J.~A. and {Buder}, I. and {Bullock}, E. and {Buza}, V. and {Connors}, J. and {Cornelison}, J. and {Crill}, B.~P. and {Crumrine}, M. and {Dierickx}, M. and {Duband}, L. and {Dvorkin}, C. and {Filippini}, J.~P. and {Fliescher}, S. and {Grayson}, J. and {Hall}, G. and {Halpern}, M. and {Harrison}, S. and {Hildebrandt}, S.~R. and {Hilton}, G.~C. and {Hui}, H. and {Irwin}, K.~D. and {Kang}, J. and {Karkare}, K.~S. and {Karpel}, E. and {Kaufman}, J.~P. and {Keating}, B.~G. and {Kefeli}, S. and {Kernasovskiy}, S.~A. and {Kovac}, J.~M. and {Kuo}, C.~L. and {Larsen}, N.~A. and {Lau}, K. and {Leitch}, E.~M. and {Lueker}, M. and {Megerian}, K.~G. and {Moncelsi}, L. and {Namikawa}, T. and {Netterfield}, C.~B. and {Nguyen}, H.~T. and {O'Brient}, R. and {Ogburn}, R.~W. and {Palladino}, S. and {Pryke}, C. and {Racine}, B. and {Richter}, S. and {Schillaci}, A. and {Schwarz}, R. and {Sheehy}, C.~D. and {Soliman}, A. and {St. Germaine}, T. and {Staniszewski}, Z.~K. and {Steinbach}, B. and {Sudiwala}, R.~V. and {Teply}, G.~P. and {Thompson}, K.~L. and {Tolan}, J.~E. and {Tucker}, C. and {Turner}, A.~D. and {Umilt{\`a}}, C. and {Vieregg}, A.~G. and {Wandui}, A. and {Weber}, A.~C. and {Wiebe}, D.~V. and {Willmert}, J. and {Wong}, C.~L. and {Wu}, W.~L.~K. and {Yang}, H. and {Yoon}, K.~W. and {Zhang}, C.},
        title = "{Constraints on Primordial Gravitational Waves Using Planck, WMAP, and New BICEP2/Keck Observations through the 2015 Season}",
      journal = {\prl},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = nov,
       volume = {121},
       number = {22},
          eid = {221301},
        pages = {221301},
          doi = {10.1103/PhysRevLett.121.221301},
archivePrefix = {arXiv},
       eprint = {1810.05216},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PhRvL.121v1301B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{benett2013finalmaps,
       author = {{Bennett}, C.~L. and {Larson}, D. and {Weiland}, J.~L. and {Jarosik}, N. and {Hinshaw}, G. and {Odegard}, N. and {Smith}, K.~M. and {Hill}, R.~S. and {Gold}, B. and {Halpern}, M. and {Komatsu}, E. and {Nolta}, M.~R. and {Page}, L. and {Spergel}, D.~N. and {Wollack}, E. and {Dunkley}, J. and {Kogut}, A. and {Limon}, M. and {Meyer}, S.~S. and {Tucker}, G.~S. and {Wright}, E.~L.},
        title = "{Nine-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Final Maps and Results}",
      journal = {\apjs},
     keywords = {cosmic background radiation, cosmology: observations, dark matter, early universe, instrumentation: detectors, space vehicles, space vehicles: instruments, telescopes, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = oct,
       volume = {208},
       number = {2},
          eid = {20},
        pages = {20},
          doi = {10.1088/0067-0049/208/2/20},
archivePrefix = {arXiv},
       eprint = {1212.5225},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..208...20B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{polarbear2017measurement,
       author = {{POLARBEAR Collaboration} and {Ade}, P.~A.~R. and {Aguilar}, M. and {Akiba}, Y. and {Arnold}, K. and {Baccigalupi}, C. and {Barron}, D. and {Beck}, D. and {Bianchini}, F. and {Boettger}, D. and {Borrill}, J. and {Chapman}, S. and {Chinone}, Y. and {Crowley}, K. and {Cukierman}, A. and {D{\"u}nner}, R. and {Dobbs}, M. and {Ducout}, A. and {Elleflot}, T. and {Errard}, J. and {Fabbian}, G. and {Feeney}, S.~M. and {Feng}, C. and {Fujino}, T. and {Galitzki}, N. and {Gilbert}, A. and {Goeckner-Wald}, N. and {Groh}, J.~C. and {Hall}, G. and {Halverson}, N. and {Hamada}, T. and {Hasegawa}, M. and {Hazumi}, M. and {Hill}, C.~A. and {Howe}, L. and {Inoue}, Y. and {Jaehnig}, G. and {Jaffe}, A.~H. and {Jeong}, O. and {Kaneko}, D. and {Katayama}, N. and {Keating}, B. and {Keskitalo}, R. and {Kisner}, T. and {Krachmalnicoff}, N. and {Kusaka}, A. and {Le Jeune}, M. and {Lee}, A.~T. and {Leitch}, E.~M. and {Leon}, D. and {Linder}, E. and {Lowry}, L. and {Matsuda}, F. and {Matsumura}, T. and {Minami}, Y. and {Montgomery}, J. and {Navaroli}, M. and {Nishino}, H. and {Paar}, H. and {Peloton}, J. and {Pham}, A.~T.~P. and {Poletti}, D. and {Puglisi}, G. and {Reichardt}, C.~L. and {Richards}, P.~L. and {Ross}, C. and {Segawa}, Y. and {Sherwin}, B.~D. and {Silva-Feaver}, M. and {Siritanasak}, P. and {Stebor}, N. and {Stompor}, R. and {Suzuki}, A. and {Tajima}, O. and {Takakura}, S. and {Takatori}, S. and {Tanabe}, D. and {Teply}, G.~P. and {Tomaru}, T. and {Tucker}, C. and {Whitehorn}, N. and {Zahn}, A.},
        title = "{A Measurement of the Cosmic Microwave Background B-mode Polarization Power Spectrum at Subdegree Scales from Two Years of polarbear Data}",
      journal = {\apj},
     keywords = {cosmic background radiation, cosmology: observations, large-scale structure of universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = oct,
       volume = {848},
       number = {2},
          eid = {121},
        pages = {121},
          doi = {10.3847/1538-4357/aa8e9f},
archivePrefix = {arXiv},
       eprint = {1705.02907},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...848..121P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{henning2018measurements,
       author = {{Henning}, J.~W. and {Sayre}, J.~T. and {Reichardt}, C.~L. and {Ade}, P.~A.~R. and {Anderson}, A.~J. and {Austermann}, J.~E. and {Beall}, J.~A. and {Bender}, A.~N. and {Benson}, B.~A. and {Bleem}, L.~E. and {Carlstrom}, J.~E. and {Chang}, C.~L. and {Chiang}, H.~C. and {Cho}, H. -M. and {Citron}, R. and {Corbett Moran}, C. and {Crawford}, T.~M. and {Crites}, A.~T. and {de Haan}, T. and {Dobbs}, M.~A. and {Everett}, W. and {Gallicchio}, J. and {George}, E.~M. and {Gilbert}, A. and {Halverson}, N.~W. and {Harrington}, N. and {Hilton}, G.~C. and {Holder}, G.~P. and {Holzapfel}, W.~L. and {Hoover}, S. and {Hou}, Z. and {Hrubes}, J.~D. and {Huang}, N. and {Hubmayr}, J. and {Irwin}, K.~D. and {Keisler}, R. and {Knox}, L. and {Lee}, A.~T. and {Leitch}, E.~M. and {Li}, D. and {Lowitz}, A. and {Manzotti}, A. and {McMahon}, J.~J. and {Meyer}, S.~S. and {Mocanu}, L. and {Montgomery}, J. and {Nadolski}, A. and {Natoli}, T. and {Nibarger}, J.~P. and {Novosad}, V. and {Padin}, S. and {Pryke}, C. and {Ruhl}, J.~E. and {Saliwanchik}, B.~R. and {Schaffer}, K.~K. and {Sievers}, C. and {Smecher}, G. and {Stark}, A.~A. and {Story}, K.~T. and {Tucker}, C. and {Vanderlinde}, K. and {Veach}, T. and {Vieira}, J.~D. and {Wang}, G. and {Whitehorn}, N. and {Wu}, W.~L.~K. and {Yefremenko}, V.},
        title = "{Measurements of the Temperature and E-mode Polarization of the CMB from 500 Square Degrees of SPTpol Data}",
      journal = {\apj},
     keywords = {cosmic background radiation, cosmological parameters, cosmology: observations, polarization, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = jan,
       volume = {852},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/aa9ff4},
archivePrefix = {arXiv},
       eprint = {1707.09353},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...852...97H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{planck2018power_spectra,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Casaponsa}, B. and {Challinor}, A. and {Chiang}, H.~C. and {Colombo}, L.~P.~L. and {Combet}, C. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Lilley}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sirri}, G. and {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. V. CMB power spectra and likelihoods}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmology: observations, cosmological parameters, methods: data analysis, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A5},
        pages = {A5},
          doi = {10.1051/0004-6361/201936386},
archivePrefix = {arXiv},
       eprint = {1907.12875},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...5P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{choi2020atacama,
       author = {{Choi}, Steve K. and {Hasselfield}, Matthew and {Ho}, Shuay-Pwu Patty and {Koopman}, Brian and {Lungu}, Marius and {Abitbol}, Maximilian H. and {Addison}, Graeme E. and {Ade}, Peter A.~R. and {Aiola}, Simone and {Alonso}, David and {Amiri}, Mandana and {Amodeo}, Stefania and {Angile}, Elio and {Austermann}, Jason E. and {Baildon}, Taylor and {Battaglia}, Nick and {Beall}, James A. and {Bean}, Rachel and {Becker}, Daniel T. and {Bond}, J. Richard and {Bruno}, Sarah Marie and {Calabrese}, Erminia and {Calafut}, Victoria and {Campusano}, Luis E. and {Carrero}, Felipe and {Chesmore}, Grace E. and {Cho}, Hsiao-mei and {Clark}, Susan E. and {Cothard}, Nicholas F. and {Crichton}, Devin and {Crowley}, Kevin T. and {Darwish}, Omar and {Datta}, Rahul and {Denison}, Edward V. and {Devlin}, Mark J. and {Duell}, Cody J. and {Duff}, Shannon M. and {Duivenvoorden}, Adriaan J. and {Dunkley}, Jo and {D{\"u}nner}, Rolando and {Essinger-Hileman}, Thomas and {Fankhanel}, Max and {Ferraro}, Simone and {Fox}, Anna E. and {Fuzia}, Brittany and {Gallardo}, Patricio A. and {Gluscevic}, Vera and {Golec}, Joseph E. and {Grace}, Emily and {Gralla}, Megan and {Guan}, Yilun and {Hall}, Kirsten and {Halpern}, Mark and {Han}, Dongwon and {Hargrave}, Peter and {Henderson}, Shawn and {Hensley}, Brandon and {Hill}, J. Colin and {Hilton}, Gene C. and {Hilton}, Matt and {Hincks}, Adam D. and {Hlo{\v{z}}ek}, Ren{\'e}e and {Hubmayr}, Johannes and {Huffenberger}, Kevin M. and {Hughes}, John P. and {Infante}, Leopoldo and {Irwin}, Kent and {Jackson}, Rebecca and {Klein}, Jeff and {Knowles}, Kenda and {Kosowsky}, Arthur and {Lakey}, Vincent and {Li}, Dale and {Li}, Yaqiong and {Li}, Zack and {Lokken}, Martine and {Louis}, Thibaut and {MacInnis}, Amanda and {Madhavacheril}, Mathew and {Maldonado}, Felipe and {Mallaby-Kay}, Maya and {Marsden}, Danica and {Maurin}, Lo{\"\i}c and {McMahon}, Jeff and {Menanteau}, Felipe and {Moodley}, Kavilan and {Morton}, Tim and {Naess}, Sigurd and {Namikawa}, Toshiya and {Nati}, Federico and {Newburgh}, Laura and {Nibarger}, John P. and {Nicola}, Andrina and {Niemack}, Michael D. and {Nolta}, Michael R. and {Orlowski-Sherer}, John and {Page}, Lyman A. and {Pappas}, Christine G. and {Partridge}, Bruce and {Phakathi}, Phumlani and {Prince}, Heather and {Puddu}, Roberto and {Qu}, Frank J. and {Rivera}, Jesus and {Robertson}, Naomi and {Rojas}, Felipe and {Salatino}, Maria and {Schaan}, Emmanuel and {Schillaci}, Alessandro and {Schmitt}, Benjamin L. and {Sehgal}, Neelima and {Sherwin}, Blake D. and {Sierra}, Carlos and {Sievers}, Jon and {Sifon}, Cristobal and {Sikhosana}, Precious and {Simon}, Sara and {Spergel}, David N. and {Staggs}, Suzanne T. and {Stevens}, Jason and {Storer}, Emilie and {Sunder}, Dhaneshwar D. and {Switzer}, Eric R. and {Thorne}, Ben and {Thornton}, Robert and {Trac}, Hy and {Treu}, Jesse and {Tucker}, Carole and {Vale}, Leila R. and {Van Engelen}, Alexander and {Van Lanen}, Jeff and {Vavagiakis}, Eve M. and {Wagoner}, Kasey and {Wang}, Yuhan and {Ward}, Jonathan T. and {Wollack}, Edward J. and {Xu}, Zhilei and {Zago}, Fernando and {Zhu}, Ningfeng},
        title = "{The Atacama Cosmology Telescope: a measurement of the Cosmic Microwave Background power spectra at 98 and 150 GHz}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
       volume = {2020},
       number = {12},
          eid = {045},
        pages = {045},
          doi = {10.1088/1475-7516/2020/12/045},
archivePrefix = {arXiv},
       eprint = {2007.07289},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JCAP...12..045C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{allison2015towards,
       author = {{Allison}, R. and {Caucal}, P. and {Calabrese}, E. and {Dunkley}, J. and {Louis}, T.},
        title = "{Towards a cosmological neutrino mass detection}",
      journal = {\prd},
     keywords = {98.80.-k, 14.60.Pq, 95.85.Ry, Cosmology, Neutrino mass and mixing, Neutrino muon pion and other elementary particles, cosmic rays, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = dec,
       volume = {92},
       number = {12},
          eid = {123535},
        pages = {123535},
          doi = {10.1103/PhysRevD.92.123535},
archivePrefix = {arXiv},
       eprint = {1509.07471},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PhRvD..92l3535A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{divalentino2016cosmological,
       author = {{Di Valentino}, Eleonora and {Giusarma}, Elena and {Mena}, Olga and {Melchiorri}, Alessandro and {Silk}, Joseph},
        title = "{Cosmological limits on neutrino unknowns versus low redshift priors}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2016,
        month = apr,
       volume = {93},
       number = {8},
          eid = {083527},
        pages = {083527},
          doi = {10.1103/PhysRevD.93.083527},
archivePrefix = {arXiv},
       eprint = {1511.00975},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PhRvD..93h3527D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{giusarma2016improvement,
       author = {{Giusarma}, Elena and {Gerbino}, Martina and {Mena}, Olga and {Vagnozzi}, Sunny and {Ho}, Shirley and {Freese}, Katherine},
        title = "{Improvement of cosmological neutrino mass bounds}",
      journal = {\prd},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = oct,
       volume = {94},
       number = {8},
          eid = {083522},
        pages = {083522},
          doi = {10.1103/PhysRevD.94.083522},
archivePrefix = {arXiv},
       eprint = {1605.04320},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PhRvD..94h3522G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boyle2018deconstructing,
       author = {{Boyle}, Aoife and {Komatsu}, Eiichiro},
        title = "{Deconstructing the neutrino mass constraint from galaxy redshift surveys}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = mar,
       volume = {2018},
       number = {3},
          eid = {035},
        pages = {035},
          doi = {10.1088/1475-7516/2018/03/035},
archivePrefix = {arXiv},
       eprint = {1712.01857},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018JCAP...03..035B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{archidiacono2017physical,
       author = {{Archidiacono}, Maria and {Brinckmann}, Thejs and {Lesgourgues}, Julien and {Poulin}, Vivian},
        title = "{Physical effects involved in the measurements of neutrino masses with future cosmological data}",
      journal = {\jcap},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
         year = 2017,
        month = feb,
       volume = {2017},
       number = {2},
          eid = {052},
        pages = {052},
          doi = {10.1088/1475-7516/2017/02/052},
archivePrefix = {arXiv},
       eprint = {1610.09852},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017JCAP...02..052A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bennett1996fouryear,
       author = {{Bennett}, C.~L. and {Banday}, A.~J. and {Gorski}, K.~M. and {Hinshaw}, G. and {Jackson}, P. and {Keegstra}, P. and {Kogut}, A. and {Smoot}, G.~F. and {Wilkinson}, D.~T. and {Wright}, E.~L.},
        title = "{Four-Year COBE DMR Cosmic Microwave Background Observations: Maps and Basic Results}",
      journal = {\apjl},
     keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: OBSERVATIONS, Astrophysics},
         year = 1996,
        month = jun,
       volume = {464},
        pages = {L1},
          doi = {10.1086/310075},
archivePrefix = {arXiv},
       eprint = {astro-ph/9601067},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...464L...1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gamow1946expanding,
       author = {{Gamow}, G.},
        title = "{Expanding Universe and the Origin of Elements}",
      journal = {Physical Review},
         year = 1946,
        month = oct,
       volume = {70},
       number = {7-8},
        pages = {572-573},
          doi = {10.1103/PhysRev.70.572.2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1946PhRv...70..572G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{irwin1995TES,
       author = {{Irwin}, K.~D.},
        title = "{An application of electrothermal feedback for high resolution cryogenic particle detection}",
      journal = {Applied Physics Letters},
         year = 1995,
        month = apr,
       volume = {66},
       number = {15},
        pages = {1998-2000},
          doi = {10.1063/1.113674},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApPhL..66.1998I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{polarbear2010new,
       author = {{The Polarbear Collaboration} and {Errard}, J. and {Ade}, P.~A.~R. and {Anthony}, A. and {Arnold}, K. and {Aubin}, F. and {Boettger}, D. and {Borrill}, J. and {Cantalupo}, C. and {Dobbs}, M.~A. and {Flanigan}, D. and {Ghribi}, A. and {Halverson}, N. and {Hazumi}, M. and {Holzapfel}, W.~L. and {Howard}, J. and {Hyland}, P. and {Jaffe}, A. and {Keating}, B. and {Kisner}, T. and {Kermish}, Z. and {Lee}, A.~T. and {Linder}, E. and {Lungu}, M. and {Matsumura}, T. and {Miller}, N. and {Meng}, X. and {Myers}, M. and {Nishino}, H. and {O'Brient}, R. and {O'Dea}, D. and {Reichardt}, C. and {Schanning}, I. and {Shimizu}, A. and {Shimmin}, C. and {Shimon}, M. and {Spieler}, H. and {Steinbach}, B. and {Stompor}, R. and {Suzuki}, A. and {Tomaru}, T. and {Tran}, H.~T. and {Tucker}, C. and {Quealy}, E. and {Richards}, P.~L. and {Zahn}, O.},
        title = "{The new generation CMB B-mode polarization experiment: POLARBEAR}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2010,
        month = nov,
          eid = {arXiv:1011.0763},
        pages = {arXiv:1011.0763},
          doi = {10.48550/arXiv.1011.0763},
archivePrefix = {arXiv},
       eprint = {1011.0763},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010arXiv1011.0763T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kusaka2014modulation,
       author = {{Kusaka}, A. and {Essinger-Hileman}, T. and {Appel}, J.~W. and {Gallardo}, P. and {Irwin}, K.~D. and {Jarosik}, N. and {Nolta}, M.~R. and {Page}, L.~A. and {Parker}, L.~P. and {Raghunathan}, S. and {Sievers}, J.~L. and {Simon}, S.~M. and {Staggs}, S.~T. and {Visnjic}, K.},
        title = "{Publisher's Note: ``Modulation of cosmic microwave background polarization with a warm rapidly rotating half-wave plate on the Atacama B-Mode Search instrument'' [Rev. Sci. Instrum. 85, 024501 (2014)]}",
      journal = {Review of Scientific Instruments},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2014,
        month = mar,
       volume = {85},
       number = {3},
          eid = {039901},
        pages = {039901},
          doi = {10.1063/1.4867655},
archivePrefix = {arXiv},
       eprint = {1310.3711},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014RScI...85c9901K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{errard2015atomospheric,
       author = {{Errard}, J. and {Ade}, P.~A.~R. and {Akiba}, Y. and {Arnold}, K. and {Atlas}, M. and {Baccigalupi}, C. and {Barron}, D. and {Boettger}, D. and {Borrill}, J. and {Chapman}, S. and {Chinone}, Y. and {Cukierman}, A. and {Delabrouille}, J. and {Dobbs}, M. and {Ducout}, A. and {Elleflot}, T. and {Fabbian}, G. and {Feng}, C. and {Feeney}, S. and {Gilbert}, A. and {Goeckner-Wald}, N. and {Halverson}, N.~W. and {Hasegawa}, M. and {Hattori}, K. and {Hazumi}, M. and {Hill}, C. and {Holzapfel}, W.~L. and {Hori}, Y. and {Inoue}, Y. and {Jaehnig}, G.~C. and {Jaffe}, A.~H. and {Jeong}, O. and {Katayama}, N. and {Kaufman}, J. and {Keating}, B. and {Kermish}, Z. and {Keskitalo}, R. and {Kisner}, T. and {Le Jeune}, M. and {Lee}, A.~T. and {Leitch}, E.~M. and {Leon}, D. and {Linder}, E. and {Matsuda}, F. and {Matsumura}, T. and {Miller}, N.~J. and {Myers}, M.~J. and {Navaroli}, M. and {Nishino}, H. and {Okamura}, T. and {Paar}, H. and {Peloton}, J. and {Poletti}, D. and {Puglisi}, G. and {Rebeiz}, G. and {Reichardt}, C.~L. and {Richards}, P.~L. and {Ross}, C. and {Rotermund}, K.~M. and {Schenck}, D.~E. and {Sherwin}, B.~D. and {Siritanasak}, P. and {Smecher}, G. and {Stebor}, N. and {Steinbach}, B. and {Stompor}, R. and {Suzuki}, A. and {Tajima}, O. and {Takakura}, S. and {Tikhomirov}, A. and {Tomaru}, T. and {Whitehorn}, N. and {Wilson}, B. and {Yadav}, A. and {Zahn}, O.},
        title = "{Modeling Atmospheric Emission for CMB Ground-based Observations}",
      journal = {\apj},
     keywords = {atmospheric effects, methods: data analysis, methods: observational, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = aug,
       volume = {809},
       number = {1},
          eid = {63},
        pages = {63},
          doi = {10.1088/0004-637X/809/1/63},
archivePrefix = {arXiv},
       eprint = {1501.07911},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...809...63E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{thomas1990atomwindow,
       author = {{Thomas}, Michael E.},
        title = "{Infared- and millimeter-wavelength continuum absorption in the atmospheric windows: measurements and models.}",
      journal = {Infrared Physics},
     keywords = {Atmospheric Attenuation, Atmospheric Models, Atmospheric Windows, Electromagnetic Wave Transmission, Infrared Windows, Continuous Spectra, Infrared Absorption, Millimeter Waves, Water Vapor, Geophysics, Earth Atmosphere: Infrared Absorption, Earth Atmosphere: Microwave Absorption},
         year = 1990,
        month = jan,
       volume = {30},
       number = {2},
        pages = {161-174},
          doi = {10.1016/0020-0891(90)90027-S},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990InfPh..30..161T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{friedmann1924freadmanneq,
       author = {{Friedmann}, A.},
        title = "{{\"U}ber die M{\"o}glichkeit einer Welt mit konstanter negativer Kr{\"u}mmung des Raumes}",
      journal = {Zeitschrift fur Physik},
         year = 1924,
        month = dec,
       volume = {21},
       number = {1},
        pages = {326-332},
          doi = {10.1007/BF01328280},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ZPhy...21..326F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kovac2002poldetection,
       author = {{Kovac}, J.~M. and {Leitch}, E.~M. and {Pryke}, C. and {Carlstrom}, J.~E. and {Halverson}, N.~W. and {Holzapfel}, W.~L.},
        title = "{Detection of polarization in the cosmic microwave background using DASI}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2002,
        month = dec,
       volume = {420},
       number = {6917},
        pages = {772-787},
          doi = {10.1038/nature01269},
archivePrefix = {arXiv},
       eprint = {astro-ph/0209478},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002Natur.420..772K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


